Multi-Constraint Shortest Path using Forest Hop Labeling

The \textit{Multi-Constraint Shortest Path (MCSP)} problem aims to find the shortest path between two nodes in a network subject to a given constraint set. It is typically processed as a \textit{skyline path} problem. However, the number of intermediate skyline paths becomes larger as the network size increases and the constraint number grows, which brings about the dramatical growth of computational cost and further makes the existing index-based methods hardly capable of obtaining the complete exact results. In this paper, we propose a novel high-dimensional skyline path concatenation method to avoid the expensive skyline path search, which then supports the efficient construction of hop labeling index for \textit{MCSP} queries. Specifically, a set of insightful observations and techniques are proposed to improve the efficiency of concatenating two skyline path set, a \textit{n-Cube} technique is designed to prune the concatenation space among multiple hops, and a \textit{constraint pruning} method is used to avoid the unnecessary computation. Furthermore, to scale up to larger networks, we propose a novel \textit{forest hop labeling} which enables the parallel label construction from different network partitions. Our approach is the first method that can achieve both accuracy and efficiency for \textit{MCSP} query answering. Extensive experiments on real-life road networks demonstrate the superiority of our method over the state-of-the-art solutions.

==> CSP-H2H (VLDBJ)/CSP2Hop.tex <==
\section{CSP-2Hop Labeling}
\label{sec:CSP2Hop}
%In our case, except computing weighs, the 2 hop labeling have to consider another criterion which is cost. Therefore, the definition of constrained 2 hop labeling (CSP-2Hop) as follows:
%Unlike the 2-hop labeling in the single-criteria scenario whose label is only a distance value, the 
\textit{CSP-2Hop}'s label is a set of skyline paths. Specifically, for each vertex $u \in V$, it has a label set \mycolor{$L(u)=\{(v,P(u,v))\}$}, where $v$ is the hop vertex (\mycolor{$\{v\}$ is $u$'s hop set}) and $P(u,v)$ is the skyline path set. We use $L=\{(L(u)|\forall u \in V\}$ to denote the set of all the labels. If $L$ can answer all the \textit{CSP} queries in $G$, then we say $L$ is a \textit{CSP-2Hop} cover. Given a \textit{CSP} query $q(s,t,C)$, we first determine the common intermediate hop set \mycolor{$H=L(s) \cap L(t)$}. Then, we can find a set of candidate paths from $s$ to $t$ for validation by concatenating the skyline paths:
\begin{equation*}
\begin{aligned}
    P_c(H) &= \{P_c(h_i)|
    \{P(s,h_i)\oplus P(h_i,t)\}\}, \forall h_i\in H\\
    &=\{\{ p_j(w_j(s,h_i)+w_k(h_i,t),c_j(s,h_i)+c_k(h_i,t))\}\}\\
    &\forall p_j\in p(s,h_i) \wedge p_k\in p(h_i,t) 
\end{aligned}
\end{equation*}
where $\oplus$ is \textit{path concatenation} operator. Each $P_c(h_i)$ contains all the pairwise skyline concatenation results, and $P_c(H)$ is their union.
For instance, suppose the out-label of $s$ to $h$ has two skyline paths $p_1$ and $p_2$ and the in-label of $h$ to $t$ contains $p_3$ and $p_4$. Then we can obtain four paths from $s$ to $t$ by concatenating $p_1$ and $p_2$ interchangeably with $p_3$ and $p_4$, and obtain $P_c(h)=\{p_1\oplus p_3, p_1\oplus p_4, p_2\oplus p_3, p_2\oplus p_4\}$. 
%P_{candi}{\{i|p_i(w(s,h)+w(h,t),c(s,h)+c(h, t))|h \in H\}}$.

%\begin{definition}[Skyline Path Candidate]
%Suppose $h_i$ is an intermediate hop in $H$, we define $P(h_i)$ is the set of skyline paths from $s$ to $h_i$, $P’(h_i)$ is the set of skyline paths from $h_i$ to $s$. We denote $p_n.h_i$ is an arbitrary skyline path in $P(h_i)$, $p_m.h_i$ is an arbitrary skyline path in $P’(h_i)$. $p$ is a stitching path using a path in $P(h_i)$ and another path $P’(h_i)$. A set $P_{candi}$ has all the pair-wise connecting paths by paths in $P(h_i)$ and  $P’(h_i)$.
%\end{definition}


%the definition above need to be edited later. 

%In detail, for an arbitrary vertex $v$, we create its in-label set by storing skyline paths from other vertices to $v$, and also create its out-label set by storing skyline paths from $v$ to other vertices. To answer a query $q(s, t, C)$, we should first find the intermediate hop set $H$ by $L_{out}(s)$ and $L_{in}(t)$. For each intermediate hop $h$ in $H$, we combine the skyline paths from $s$ to $h$ with the skyline paths from $h$ to $t$.  We then generate a set of candidate path $P_{candi}$ for all intermediate hop in $H$. 

%We then identify the paths in candidate paths set $P_{candi}$ and ensure the set $P_{candi}$ must contain the result of the CSP query. To prove the existence of CSP in $P_{candi}$, the question can transfer to identify that $P_{candi}$ can contain all the skyline paths from $s$ to $t$. If all the skyline paths can be found in the set, the CSP also can be identified in the set of skyline paths.

As proved in Theorem \ref{the:Skyline}, the skyline paths between $s$ and $t$ are enough to answer any \textit{CSP} query, so we only need to prove the candidate set $P_c(H)$ covers all the skyline paths between $s$ and $t$. Firstly, we introduce the following lemma:  
%Due to each path in $P_{candi}$ is generated by two sub-skyline paths, we provide the theorem on the existence and corresponding proof as follows:

\begin{lemma}
\label{lemma:SkylineSubpath}
If a path $p$ is a skyline path, the sub-paths on $p$ are all skyline paths.
\end{lemma}
\begin{proof}
The proof of it can be found in \cite{storandt2012route}.
\end{proof}


\begin{theorem}
\label{the:HopSkyline}
$P_c(h)$ covers all the skyline paths from $s$ to $t$ that travel via hop $h$.
%Given an intermediate hop set $H$, let a set $P_1$ has all the skyline paths from vertex $s \in V$ to each vertex $h \in H$, and a set $P_2$ has all the skyline paths from $h$ to vertex $t \in V$. $P_{candi}$ has all the matching paths by $P_1$ and $P_2$. We ensure that all the paths in $P_{candi}$ must cover all the skyline paths from $s$ to $t$. 
\end{theorem}
\begin{proof}
Suppose $p^*$ is a skyline path from $s$ to $t$ via $h$ and $p^*\notin P_c(h)$. According to Lemma \ref{lemma:SkylineSubpath}, $p^*$'s sub-paths $p^*(s,h)$ and $p^*(h,t)$ are also skyline paths from $s$ to $h$ and from $h$ to $t$. If $p^*(s,h)\notin P(s,h)$ or $p^*(h,t)\notin P(h,t)$, it contradicts the definition that $P(s,h)$ contains all the skyline paths from $s$ to $h$, and similar for $P(h,t)$. Therefore, $P_c(h)$ covers all the skyline paths from $s$ to $t$ via $h$.
 %Initially, we ensure that if a path $p$ is a skyline path, all the sub-paths on $p$ are skyline paths{\cite{storandt2012route}}. For this reason, if we have a path $p$ from $s$ to $t$, and select a intermediate hop $h$ on $p$, $s-h$ path $p_1$  and $h-t$ path $p_2$ will also be the skyline paths. By the definition of 2 hop labeling in CSP, $L_{out}(s)$ can cover all the skyline paths from $s$ to $h$, $L_{in}(t)$ also have all the skyline paths from $h$ to $t$. Hence, we can conclude that $p_1$ and $p_2$ must exist in the labels of $s$ and $t$. This is, if $s$ to $t$ has skyline paths, the two sub-paths of each skyline path can be found in the labels of $s$ and $t$. We can identify that the combination set $P_{candi}$ must include all the skyline paths from $s$ to $t$.
\end{proof}


\iffalse
\begin{table*}
\centering
\caption{CSP-2Hop Labels}
\label{talbe:CSP-2Hop}
\scriptsize
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{} & \textbf{$v_3$} & \textbf{$v_7$} & \textbf{$v_{11}$} & \textbf{$v_{10}$} & \textbf{$v_9$}                                                 & \textbf{$v_4$}                                                        & \textbf{$v_1$}                                                                    & \textbf{$v_5$}                                                                   & \textbf{$v_8$}                                                        & \textbf{$v_{12}$}                                              \\ \hline
\textbf{$v_2$}     & (1, 1)         &                &                   &                   & (2, 5),(4, 3)                                                  & (1, 2)                                                                & (1, 2)                                                                            & (2, 4),(4, 3)                                                                    & (2, 4)                                                                & (3, 5),(7, 4)                                                  \\ \hline
\textbf{$v_3$}     &                &                &                   &                   & (1, 4),(6, 3)                                                  & (2, 3),(3, 2)                                                         & (2, 3)                                                                            & (3, 5),(4, 4)                                                                    & \begin{tabular}[c]{@{}l@{}}(2, 6),(3, 5)\\ (4, 4)\end{tabular}        & \begin{tabular}[c]{@{}l@{}}(3, 7),(4, 6)\\ (5, 5)\end{tabular} \\ \hline
\textbf{$v_6$}     &                & (2, 0)         &                   &                   &                                                                &                                                                       & (2, 0)                                                                            & (1, 1)                                                                           & \begin{tabular}[c]{@{}l@{}}(3, 5),(4, 4)\\ (5, 3)\end{tabular}        & (4, 2)                                                         \\ \hline
\textbf{$v_7$}     &                &                &                   &                   &                                                                &                                                                       & (3, 5),(4, 0)                                                                     & (1, 3),(3, 1)                                                                           & (3, 3)                                                                & (2, 2)                                                         \\ \hline
\textbf{$v_{13}$}  &                &                & \begin{tabular}[c]{@{}c@{}}(2, 3)\\(5, 2)\end{tabular}     & \begin{tabular}[c]{@{}c@{}}(3, 5)\\(4, 0)\end{tabular}     & \begin{tabular}[c]{@{}c@{}}(4, 9),(5, 6)\\ (6, 1)\end{tabular} & \begin{tabular}[c]{@{}c@{}}(4, 9),(5, 7)\\ (6, 4),(9, 2)\end{tabular} & \begin{tabular}[c]{@{}l@{}}(6, 13),(7, 11)\\ (8, 8),(9, 6)\\ (12, 5)\end{tabular} & \begin{tabular}[c]{@{}l@{}}(5, 11),(6, 9)\\ (7, 6),(8, 5)\\ (10, 4)\end{tabular} & \begin{tabular}[c]{@{}l@{}}(3, 7),(4, 5)\\ (5, 2)\end{tabular}        & \begin{tabular}[c]{@{}l@{}}(2, 6),(3, 4)\\ (6, 3)\end{tabular} \\ \hline
\textbf{$v_{11}$}  &                &                &                   & (1, 2)            & (3, 3)                                                         & (3, 4)                                                                & \begin{tabular}[c]{@{}l@{}}(5, 8)\\ (7, 3)\end{tabular}                           & \begin{tabular}[c]{@{}l@{}}(4, 6),(5, 5)\\ (6, 4)\end{tabular}                   & (2, 2)                                                                & (1, 1)                                                         \\ \hline
\textbf{$v_{10}$}  &                &                &                   &                   & (2, 1)                                                         & (2, 4),(5, 2)                                                         & \begin{tabular}[c]{@{}l@{}}(4, 8),(6, 7)\\ (7, 6),(8, 5)\end{tabular}             & \begin{tabular}[c]{@{}l@{}}(3, 6),(4, 5)\\ (6, 4)\end{tabular}                   & (1, 2)                                                                & (2, 3)                                                         \\ \hline
\textbf{$v_9$}     &                &                &                   &                   &                                                                & (2, 4),(3, 1)                                                         & (3, 7),(5, 5)                                                                     & (3, 6),(4, 5)                                                                    & (1, 2)                                                                & (2, 3)                                                         \\ \hline
\textbf{$v_4$}     &                &                &                   &                   &                                                                &                                                                       & (2, 4),(4, 3)                                                                     & (1, 2)                                                                           & (1, 2)                                                                & (2, 3)                                                         \\ \hline
\textbf{$v_1$}     &                &                &                   &                   &                                                                &                                                                       &                                                                                   & (2, 2),(3, 1)                                                                    & \begin{tabular}[c]{@{}l@{}}(3, 6),(5, 5)\\ (6, 4),(7, 3)\end{tabular} & (4, 7),(6, 2)                                                  \\ \hline
\textbf{$v_5$}     &                &                &                   &                   &                                                                &                                                                       &                                                                                   &                                                                                  & (2, 4),(3, 3)                                                         & \begin{tabular}[c]{@{}l@{}}(3, 5),(4, 4)\\ (5, 3)\end{tabular} \\ \hline
\textbf{$v_8$}     &                &                &                   &                   &                                                                &                                                                       &                                                                                   &                                                                                  &                                                                       & (1, 1)                                                         \\ \hline
\textbf{$v_{12}$}  &                &                &                   &                   &                                                                &                                                                       &                                                                                   &                                                                                  & (1, 1)                                                                &                                                                \\ \hline
\end{tabular}
\end{table*}
\fi

\begin{table}[]
\centering
\caption{Partial CSP-2Hop Labels}
\label{talbe:CSP-2Hop}
\scriptsize
\scalebox{0.75}{
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Ancestors} & \textbf{$v_4$} & \textbf{$v_1$} & \textbf{$v_5$} & \textbf{$v_8$}                                                        & \textbf{$v_{12}$}                                              \\ \hline
\textbf{$v_7$}     & -              & (3, 5),(4, 0)  & (1, 3),(3, 1)         & (3, 3)                                                                & (2, 2)                                                         \\ \hline
\textbf{$v_9$}     & (2, 4),(3, 1)  & (3, 7),(5, 5)  & (3, 6),(4, 3)  & (1, 2)                                                                & (2, 3)                                                         \\ \hline
\textbf{$v_4$}     & -              & (2, 4),(4, 3)  & (1, 2)         & (1, 2)                                                                & (2, 3)                                                         \\ \hline
\textbf{$v_1$}     & -              & -              & (2, 2),(3, 1)  & (3, 6),(5, 5) (6, 4),(7, 3) & (4, 7),(6, 2)                                                  \\ \hline
\textbf{$v_5$}     & -              & -              & -              & (2, 4),(3, 3)                                                         & (3, 5),(4, 4) (5, 3) \\ \hline
\textbf{$v_8$}     & -              & -              & -              & -                                                                     & (1, 1)                                                         \\ \hline
%\textbf{$v_{12}$}  & -              & -              & -              & (1, 1)                                                                & -                                                              \\ \hline
\end{tabular}}
\end{table}


Next we need to prove the union of all the hops $h\in H$ covers all the skyline paths between $s$ and $t$. Because our 2-hop labeling is based on the graph cut, we only need to prove the following theorem:
\begin{theorem}
\label{the:CSP-2Hop}
If the hop set $H$ is the set of cuts between $s$ and $t$, then $P_c(H)=\bigcup_{h_i\in H} P_c(h_i)$ covers all the skyline paths from $s$ to $t$.
\end{theorem}
\begin{proof}
Similar to Theorem \ref{the:HopSkyline}, we also prove it with contradiction. Suppose $p^*$ is a skyline path and $p^*\notin P_c(H)$. Because $H$ is the graph cut set, $p^*$ has to travel through one of the cut vertex $h_i\in H$, which has a candidate set $P_c(h_i)$. However, $p^*\notin P_c(h_i)$ contradicts with Theorem \ref{the:HopSkyline}. So every skyline path from $s$ to $t$ exists in $P_c(H)$.
\end{proof}

In summary, our \textit{CSP-2Hop} is able to answer any \textit{CSP} query with label concatenation. 


\subsection{Index Structure}
\label{subsec:CSP2Hop_Index}
Our \textit{CSP-2Hop} is based on the \textit{Tree Decomposition} \cite{robertson1986graph,ouyang2018hierarchy}, which maps a graph into a tree structure with each tree node corresponding to a vertex and the graph cut information is captured by its ancestors:

\begin{definition}[Tree Decomposition]
\label{def:TreeDecomposition}
Given a graph $G$, its tree decomposition $T$ is a rooted tree in which each node $X\in V$ is a subset of $V$. $T$ has the following tree properties:
\begin{enumerate}
\item $\bigcup_{X_i\in V}X_i=V$;
\item $\forall (u, v)\in E, \exists X_i$ such that $\{u, v\}\subseteq X_i$;
\item $\forall v\in V$, the set $\{X|v\in X\}$ forms a subtree of $T$.
\end{enumerate}
\end{definition}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=2in]{Tree.pdf}
    \caption{Tree Decomposition Example}
    \label{fig:Tree Decomposition}
\end{figure}

For instance, Figure \ref{fig:Tree Decomposition} shows the tree decomposition of the example graph in Figure \ref{fig:ExampleGraph}. The first vertex in each tree node is its representative vertex. %Depending on if the tree nodes have an ancestor/descendent relation not, 
This structure has a \textit{Cut Property} that can be used to assign labels: $\forall s,t\in V$ and $X_s,X_t$ are their corresponding tree nodes without an ancestor/descendent relation, their cuts are in their \textit{lowest common ancestor (LCA)} node \cite{chang2012exact}, \mycolor{which is the lowest tree node that has both $X_s$ and $X_t$}. For example, the tree nodes of $v_2$ and $v_7$ are $X_2$ and $X_7$, and their \textit{LCA} is $X_{1}=\{v_{1},v_5,v_8,v_{12}\}$. Then these four vertices form a cut between $v_2$ and $v_7$. If $s$ is $t$'s descendant, then $t$ can be viewed as a cut between itself and $s$. Therefore, the \textit{LCA} of a vertex pair contains all the cuts between them. 
%2) \textit{Ancestor Property}: $\forall X_v\in T_G, X_u(u\in X_v\{v\})$ is an ancestor of $X_v$ in $T_G$. This can also be easily checked in Figure \ref{fig:Tree Decomposition}. The ancestor property 
Accordingly, we assign labels to a vertex with all its ancestors in $T_G$. It should be noted that the vertices in each tree node are also in its label because of the \textit{Ancestor Property}: $\forall X_v\in T_G, X_u(u\in X_v\backslash\{v\})$ is an ancestor of $X_v$ in $T_G$. For example, $v_6$ has labels of $\{v_7,v_1,v_5,v_8,v_{12}\}\supseteq \{v_1,v_5,v_7\}$. The detailed labels are shown in Table \ref{talbe:CSP-2Hop}, with the rows being the vertices and columns being the hops. Some cells have several values because they are skyline paths. \mycolor{The details of the index computation will be discussed in Section \ref{subsec:Construction}}. The following theorem proves the correctness of the labels:
\begin{theorem}
\label{the:LabelCorrectness}
The above procedure creates a \textit{CSP-2Hop}.
\end{theorem}
\begin{proof}
Because the labels assigned by the above procedure contains all the cuts between every vertex pair, it is a \textit{CSP-2Hop} according to Theorem \ref{the:CSP-2Hop}.
\end{proof}

\subsection{Query Processing}
\label{subsec:CSP2Hop_Query}
%To  solve the CSP queries using the CSP-2hop index, the naive solution for the CSP from $s$ to $t$ as follows: First, we generate the set $P_{candi}$ by connecting the skyline paths in the out label of $s$ to $h$ and the skyline paths in the in label of $h$ to $t$. Afterward, we screen out the paths with costs less than $C$ from $P_{candi}$. Then, we select the path with minimum weight as our output. 

Given a \textit{CSP} query $q(s,t,C)$, we can answer it with the \textit{CSP-2Hop} in the same way like the single-criteria scenario: Firstly, we generate the hop set $H=L(s) \cap L(t)=\{h|h\in X(LCA(s,t)\}$ by retrieving the vertices in the \textit{LCA} of $s$ and $t$, \mycolor{where \textit{LCA}$(s,t)$ returns the \textit{LCA} of $s$ and $t$}. Then for each $h_i\in H$, we compute $P_c(h_i)$ by $P(s,h_i)\oplus P(h_i,t)$. By taking the union of all $P_c(h_i)$, we obtain the candidate set $P_c(H)$. During the concatenation, we maintain the current optimal result (i.e., the shortest one satisfying the constraint $C$) and keep updating it. Finally, after all the candidates are generated and validated, we return the optimal one as the \textit{CSP} result.

However, unlike the 2-hop labeling of the single-criteria case where only $|H|$ times of adding is needed, the concatenation of the skyline paths makes hop computation much more time-consuming. Suppose the label of $s$ to $h$ has $m$ skyline paths and the label of $h$ to $t$ has $n$ skyline paths. Then for each intermediate hop, we have to compute $mn$ times, and the total time complexity grows to $O(mn|H|)$ instead of $O(|H|)$. 

For example, given a query $q(v_9,v_7,6)$, the \textit{LCA} of $v_9$ and $v_7$ in the tree is $X_1$, and it contains vertices $H=\{v_1,v_5,v_8,v_{12}\}$. For hop $v_1$, $L(v_9)[v_1]=\{(3,7),(5,5)\}$ and $L(v_7)[v_1]=\{(3,5),(4,0)\}$. Therefore, we can get four candidates $P_c(v_1)=\{(6,12),(7,7),(8,10),(9,5)\}$. Only $(9,5)$ has a cost smaller than $6$, so $(9,5)$ is the current best result. For hop $v_5$, we can get candidates $P_c(v_5)=\{(4,9),(5,6),(6,7),\\(7,4)\}$. Then $(5,6)$ replaces $(9,5)$ as it has smaller weight and meet the constraint condition as well. For hop $v_8$, we can get candidates $P_c(v_8)=\{(4,5)\}$, and the current best result is updated to $(4,5)$. Finally, for hop $v_{12}$, we obtain the candidate $P_c(v_{12})=\{(4,5)\}$, which is equal to the current best result. The final result is $(4,5)$. As shown in this example, although only 4 hops are needed, we actually run 10 path concatenation operations. Therefore, pruning over this large amount of computation is crucial to the query performance and we will elaborate it in Section \ref{sec:Skyline}.

\subsection{CSP-2Hop Construction}
\label{subsec:Construction}
The index construction is made up of two phases: a bottom-up \textit{Skyline Tree Decomposition} that gathers the skyline shortcuts, creates the tree nodes and forms the tree, and a top-down \textit{Skyline Label Assignment} that populates the labels with query answering, \mycolor{as shown in Algorithm \ref{Algorithm:Construction}}. It should be noted that both of these two phases do not involve the expensive skyline path search and only use the skyline path concatenation.

\begin{algorithm}[ht]
	\caption{\mycolor{CSP-2Hop Construction}}
	\label{Algorithm:Construction}
	\scriptsize
	\LinesNumbered
	\KwIn{Graph $G(V,E)$}
	\KwOut{CSP-2Hop Labeling $L$}
	\mycolor{
	\While{$v\in V$ has the minimum degree and $V\neq \phi$}
	{
		$X_v=N(v)$, $r(v)\leftarrow$ Iteration Number\Comment{Tree Node Contraction}\\
		\For{$(u,w)\leftarrow N(v)\times N(v)$}
		{
			$P(u,w)\leftarrow Skyline(p(u,v)\oplus p(v,u), (u,w))$\;
			$E\leftarrow E\cup (P(u,w))$, $V\leftarrow V-v$, 	$E\leftarrow E-(u,v)-(v,w)$\;
		}
	}
	\For{$v$ in $r(v)$ increasing order}
	{
		$u\leftarrow min\{r(u)|u\in X(v)\}, X_v.Parent\leftarrow X_u$\Comment{Tree Formation}
	}
	$X_v\leftarrow$ Tree Root, $Q.insert(X_v)$\Comment{Label Assignment}\\
	\While{$X_v\leftarrow Q.pop()$}
	{
		\For{$u\in \{u|X_u$ is ancestor of $X_v\}$}
		{
			$P(v,u))\leftarrow Skyline(P(v,w)\oplus P(w,u)), \forall w\in X_v$\;
			$L(v)\leftarrow{(u,P(v,u))}$\;
		}
		$Q.insert(X_u.children)$, $L\leftarrow L\cup L(v)$\;
	}	
	}
	
\end{algorithm}

%\subsubsection{Skyline Tree Decomposition}
%\label{subsec::Construction_TD}
%The skyline tree decomposition is made up of two steps: \textit{node contraction} that forms the tree nodes and \textit{tree construction} that organizes these nodes into a tree.

\subsubsection{Skyline Tree Node Contraction}
\label{subsubsec::CSP2Hop_TD_Contraction}
We contract the vertices in the degree-increasing order. For each $v\in V$, we add a skyline shortcut $p'(u,w)$ to all of its neighbor pairs $(u,w)$ by $p(u,v)\oplus p(v,w)$. If $(u,w)$ does not exist, then we use $p'_s(u,w)$ as its skyline path $p(u,w)$ directly. Otherwise, we compute the skyline of $p(u,w)$ and $p'(u,w)$ in a linear time sort-merge way, \mycolor{which sorts the two path sets based on $w$ first and obtain the new skyline paths by comparing them in the distance-increasing order}. After that, a tree node $X(v)$ is formed with $v$ and its neighbors $N(v)$, and all their corresponding skyline paths from $v$ to $N(v)$. The tree node $X(v)$ is assigned an order $r(v)$ according to the order when $v$ is contracted. After contracting $v$, $v$ and its edges are removed from $G$ and the remaining vertices' degree are updated. Then we contract the remaining vertices in this way until none remains. \mycolor{The time complexity of the contraction phase is $O(|V|(max(|X_i|)^2\times w^2_{max}\log w^2_{max}+\log |V|))$, where $max(|X_i|)$ is the tree width, $w_{max}$ is the longest edge distance that determines the worst case of skyline number, and $w^2_{max}\log w^2_{max}$ is concatenation.}

We use the graph in Figure \ref{fig:ExampleGraph} as the example. Firstly, we contract $v_2$ with $N(v_2)=\{v_1,v_3,v_4\}$. Because there is no edge between $v_1$ and $v_3$, we add a shortcut $(v_1,v_3)$ with  by $w=w(v_1,v_2)+w(v_2,v_3)=2$ and $c=c(v_1,v_2)+c(v_2,v_3)=3$. Similarly, there is no edge between $v_1$ and $v_4$, so we add a new edge $(v_1,v_4)$ with $w=w(v_1,v_2)+w(v_2,v_4)=2$ and $c=c(v_1,v_2)+c(v_2,v_4)=4$. As for $v_4$ and $v_3$, we first generate a shortcut by $p(v_4,v_2)\oplus p(v_2,v_3)=(2,3)$. Then because there already exists an edge $(3,2)$ from $v_4$ to $v_3$, we compute the new skyline paths between the shortcut and the edge, and get the new skyline paths $p(v_4,v_3)=\{(3,2),(2,3)\}$. After that, we remove $v_2$ from the graph, leaving $v_1$'s degree changed to 4, $v_4$'s degree remaining 5, and $v_3$'s degree remaining 3. We also obtained a tree node $X(v_2,v_3,v_1,v_4)$ with the skyline paths from $v_2$ to $N(v_2)$ and order $r(v_2)=1$. This procedure runs on with the next vertex with the smallest degree. When all the vertices finished contraction, we have an order of $\left<v_2,v_3,v_6,v_7,v_{13},v_{11},v_{10},v_9,v_4,v_1,v_5,v_8,v_{12}\right>$.


%We can have the following in sights in terms of the properties above: First, every node in $T_G$ must have at least one vertex, and every vertex in G can exist in more than one tree node. Moreover, arbitrary edge $(u, v)$  can embed in one or more tree nodes, but it is not means any two vertices u, v in a tree node must be an edge. In addition, the node $X$ can acts as separator, if we remove vertices in X from its subtree resulting in the remaining vertices in the subtree are independent.

%We can describe a tree decomposition by its treewidth and treeheight. The definition is:

%\begin{definition}[Treewidth and Treeheight]
%Given a tree decomposition $T_G$, The treewidth of $T_G$ is $max_{X\in T_G} |X|-1$. The treeheight of $T_G$ is the maximum depth from the leaves to the root of $T_G$. 
%\end{definition}

\subsubsection{Skyline Label Assignment}
\label{subsubsec::CSP2Hop_TD_Label}
It should be noted the obtained tree preserves all the skyline path information of the original graph because every edge's information are preserved in the shortcuts. In fact, we can view it as a \textit{superset} of the \textit{CSP-CH} result. Therefore, we can assign the labels with skyline search on this tree directly. However, it would be very time-consuming as the \textit{Sky-Dijk} is much slower than \textit{Dijkstra}'s. To this end, we use the top-down label cascading method that takes advantages the existing labels with query answering to assign labels to the new nodes.

Specifically, a label $L(u)$ stores all the skyline paths from $u$ to its ancestors. Therefore, we start from the root of the tree to fill all the labels. For root itself, it has no ancestor so we just skip it. Next for its child $u$, because the root is the only vertex in $X(u)$ other than $u$, we add the root to $u$'s label. Then for any tree node $X(v)$, it is guaranteed that all its ancestors have obtained their labels. Then for any of its ancestor $a_i$, we compute its skyline paths by taking the skyline paths from  $\{p(v,u)\oplus p(u,a_i)| \forall u\in X(v)$\}. \mycolor{The time complexity of the label assignment phase is $O(|V|(\log|V| + max(|X_i|)\times h \times w^2_{max}\log w^2_{max}))$, where $h$ is the tree height. The space complexity of the labels is $O(h\times |V|\times w_{max})$.}

% with the \textit{multiple skyline path concatenation} described in Section \ref{subsec:Skyline_Multiple}. 

For example in Figure \ref{fig:Tree Decomposition}, suppose we have already obtained the labels of $X_1, X_5, X_8$, and $X_{12}$, and we are computing the labels of $X(v_4)$, which has an ancestor set of $\{v_{12}, v_8, v_5, v_1\}$. We take the computation of $L(v_4)[v_{12}]$ as example. $X_4$ has three vertices $\{v_1,v_5,v_8\}$ apart from $v_4$, so we compute the skyline paths via these tree hops. To show the process clearly, we do not apply the pruning first.
\begin{equation*}
	\scriptsize
    \begin{aligned}
        P_c(h_1)&=p(v_4,v_1)\oplus p(v_1,v_{12})
        =\{(2,4),(4,3)\}\oplus\{(4,7),(6,2)\}\\
        &=\{(6,11),(8,6),(8,10),(10,5)\}\\  
        P_s(h_1)&=\{(6,11),(8,6),(10,5)\}\\
    %\end{aligned}
%\end{equation*}
%\begin{equation*}
    %\begin{aligned}
        P_c(h_5)&=p(v_4,v_5)\oplus p(v_5,v_{12})
        =\{(1,2)\}\oplus \{(3,5),(4,4),(5,3)\}\\
        &=\{(4,7),(5,6),(6,5)\}\\
        P_s(h_5)&=\{(4,7),(5,6),(6,5)\}\\
    %\end{aligned}
%\end{equation*}
%\begin{equation*}
    %\begin{aligned}
        P_c(h_8)&=p(v_4,v_8)\oplus p(v_8,v_{12})
        =\{(1,2)\}\oplus\{(1,1)\}=\{(2,3)\}\\
        P_s(h_8)&=\{(2,3)\}
    \end{aligned}
\end{equation*}

Because $(2,3)$ dominates all the others, we put $(2,3)$ into the label of $L(v_4)[v_{12}]$. %If we use the \textit{query rectangle} pruning, we first compute three corresponding rectangles: $h_1:(6,11)\times (10,5)$; $h_5:(4,7)\times (6,5)$; $h_8:(2,3)$. Because $(2,3)$ dominates the other two rectangles, we prune $h_1$ and $h_5$ and return $(2,3)$ directly as the skyline path.
The correctness of the label assignment procedure can be easily proved by induction. As the label values are essentially the query results using the existing labels of the ancestors, the results are correct as long as the ancestors' labels are correct. The labels are populated in the cascading way, and thus the correctness is naturally guaranteed. Therefore, the resulting label set is a \textit{CSP-2Hop}.
 
 \subsection{Path Retrieval}
\mycolor{To retrieve the path, we need to preserve intermedia vertex in the labels. Specifically, during the \textit{Tree Node Contraction} phase, we need store the contracted in each skyline path in each shortcut. During the path retrieval, suppose one of the skyline results is the concatenation of $s\rightarrow h$ and $h\rightarrow t$, then they are actually two shortcuts so we only need to insert the intermediate vertices recursively until all no shortcut remains to recover the original path.}






==> CSP-H2H (VLDBJ)/CSP2HopNew.tex <==
\section{MCSP-2Hop Labeling}
\label{sec:MCSP2Hop}

In this section, we first present the \textit{MCSP-2Hop} index structure and query processing, followed by the index construction, correctness proof and path retrieval.

\begin{table*}
\centering
\caption{MCSP-2Hop Labels of 2D Graph}
\label{table:MCSP-2Hop}
\scriptsize
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{} & \textbf{$v_3$} & \textbf{$v_7$} & \textbf{$v_{11}$} & \textbf{$v_{10}$} & \textbf{$v_9$}                                                 & \textbf{$v_4$}                                                        & \textbf{$v_1$}                                                                    & \textbf{$v_5$}                                                                   & \textbf{$v_8$}                                                        & \textbf{$v_{12}$}                                              \\ \hline
\textbf{$v_2$}     & (1, 1)         &                &                   &                   & (2, 5),(4, 3)                                                  & (1, 2)                                                                & (1, 2)                                                                            & (2, 4),(4, 3)                                                                    & (2, 4)                                                                & (3, 5),(7, 4)                                                  \\ \hline
\textbf{$v_3$}     &                &                &                   &                   & (1, 4),(6, 3)                                                  & (2, 3),(3, 2)                                                         & (2, 3)                                                                            & (3, 5),(4, 4)                                                                    & \begin{tabular}[c]{@{}l@{}}(2, 6),(3, 5)\\ (4, 4)\end{tabular}        & \begin{tabular}[c]{@{}l@{}}(3, 7),(4, 6)\\ (5, 5)\end{tabular} \\ \hline
\textbf{$v_6$}     &                & (2, 0)         &                   &                   &                                                                &                                                                       & (2, 0)                                                                            & (1, 1)                                                                           & \begin{tabular}[c]{@{}l@{}}(3, 5),(4, 4)\\ (5, 3)\end{tabular}        & (4, 2)                                                         \\ \hline
\textbf{$v_7$}     &                &                &                   &                   &                                                                &                                                                       & (3, 5),(4, 0)                                                                     & (1, 3),(3, 1)                                                                           & (3, 3)                                                                & (2, 2)                                                         \\ \hline
\textbf{$v_{13}$}  &                &                & \begin{tabular}[c]{@{}c@{}}(2, 3)\\(5, 2)\end{tabular}     & \begin{tabular}[c]{@{}c@{}}(3, 5)\\(4, 0)\end{tabular}     & \begin{tabular}[c]{@{}c@{}}(4, 9),(5, 6)\\ (6, 1)\end{tabular} & \begin{tabular}[c]{@{}c@{}}(4, 9),(5, 7)\\ (6, 4),(9, 2)\end{tabular} & \begin{tabular}[c]{@{}l@{}}(6, 13),(7, 11)\\ (8, 8),(9, 6)\\ (12, 5)\end{tabular} & \begin{tabular}[c]{@{}l@{}}(5, 11),(6, 9)\\ (7, 6),(8, 5)\\ (10, 4)\end{tabular} & \begin{tabular}[c]{@{}l@{}}(3, 7),(4, 5)\\ (5, 2)\end{tabular}        & \begin{tabular}[c]{@{}l@{}}(2, 6),(3, 4)\\ (6, 3)\end{tabular} \\ \hline
\textbf{$v_{11}$}  &                &                &                   & (1, 2)            & (3, 3)                                                         & (3, 4)                                                                & \begin{tabular}[c]{@{}l@{}}(5, 8)\\ (7, 3)\end{tabular}                           & \begin{tabular}[c]{@{}l@{}}(4, 6),(5, 5)\\ (6, 4)\end{tabular}                   & (2, 2)                                                                & (1, 1)                                                         \\ \hline
\textbf{$v_{10}$}  &                &                &                   &                   & (2, 1)                                                         & (2, 4),(5, 2)                                                         & \begin{tabular}[c]{@{}l@{}}(4, 8),(6, 7)\\ (7, 6),(8, 5)\end{tabular}             & \begin{tabular}[c]{@{}l@{}}(3, 6),(4, 5)\\ (6, 4)\end{tabular}                   & (1, 2)                                                                & (2, 3)                                                         \\ \hline
\textbf{$v_9$}     &                &                &                   &                   &                                                                & (2, 4),(3, 1)                                                         & (3, 7),(5, 5)                                                                     & (3, 6),(4, 5)                                                                    & (1, 2)                                                                & (2, 3)                                                         \\ \hline
\textbf{$v_4$}     &                &                &                   &                   &                                                                &                                                                       & (2, 4),(4, 3)                                                                     & (1, 2)                                                                           & (1, 2)                                                                & (2, 3)                                                         \\ \hline
\textbf{$v_1$}     &                &                &                   &                   &                                                                &                                                                       &                                                                                   & (2, 2),(3, 1)                                                                    & \begin{tabular}[c]{@{}l@{}}(3, 6),(5, 5)\\ (6, 4),(7, 3)\end{tabular} & (4, 7),(6, 2)                                                  \\ \hline
\textbf{$v_5$}     &                &                &                   &                   &                                                                &                                                                       &                                                                                   &                                                                                  & (2, 4),(3, 3)                                                         & \begin{tabular}[c]{@{}l@{}}(3, 5),(4, 4)\\ (5, 3)\end{tabular} \\ \hline
\textbf{$v_8$}     &                &                &                   &                   &                                                                &                                                                       &                                                                                   &                                                                                  &                                                                       & (1, 1)                                                         \\ \hline
\textbf{$v_{12}$}  &                &                &                   &                   &                                                                &                                                                       &                                                                                   &                                                                                  & (1, 1)                                                                &                                                                \\ \hline
\end{tabular}
\end{table*}

\subsection{Index Structure}
\label{subsec:MCSP2Hop_Index}
Unlike the traditional 2-hop labeling whose label is only a vertex and its corresponding distance value, \textit{MCSP-2Hop}'s label is a set of skyline paths. Specifically, for each vertex $u \in V$, it has a label set $L(u)=\{(v,$ $P(u,v))\}$, where $v$ is the hop vertex ($\{v\}$ is $u$'s hop set) and $P(u,v)$ is the skyline path set. We use $L=\{(L(u)|\forall u \in V\}$ to denote the set of all the labels. If $L$ can answer all the \textit{MCSP} queries in $G$, then we say $L$ is a \textit{MCSP-2Hop} cover. The detailed labels of the example graph in Figure \ref{fig:ExampleGraph} are shown in Table \ref{table:MCSP-2Hop}, with the rows being the vertices and columns being the hops. With the help of the tree decomposition in Figure \ref{fig:Tree Decomposition}, we can see each vertex stores all its ancestors on tree as labels. For example, $X_{12}, X_8$ and $X_5$ are the ancestors of $X_1$, then they appear in $v_1$'s labels. Because $X_2, X_{13}$, and $X_6$ are the leaves, they will not appear in any vertex's labels. Some cells have several values because they are skyline paths. The details of the index construction will be presented in Section \ref{subsec:MCSP2Hop_Construction}.



\subsection{Query Processing}
\label{subsec:MCSP2Hop_Query}
Given a \textit{MCSP} query $q(s,t,\overline{C})$, we can answer it with the \textit{MCSP-2Hop} in the same way like the single-criteria scenario:
we first determine the common intermediate hop set $H=L(s) \cap L(t)=\{h|h\in X(LCA(s,t)\}$ by retrieving the vertices in the \textit{LCA} of $s$ and $t$, where \textit{LCA}$(s,t)$ returns the \textit{LCA} of $X_s$ and $X_t$. Then for each $h_i\in H$, we compute its candidate set $P_c(h_i)$ by concatenating the paths $P(s,h_i)$ and $P(h_i,t)$. By taking the union of $P_c(h_i)$ from all hops in $H$, we obtain the candidate set $P_c(H)$:
\begin{equation*}
\begin{aligned}
P_c(H) &= \{P_c(h_i)|
\{P(s,h_i)\oplus P(h_i,t)\}\}, \forall h_i\in H\\
&=\bigcup\{ p_j\oplus p_k\},\forall p_j\in P(s,h_i) \wedge p_k\in P(h_i,t) 
\end{aligned}
\end{equation*}
where $\oplus$ is \textit{path concatenation} operator that takes the sum of paths' weights and the corresponding costs. Each $P_c(h_i)$ contains all the pairwise skyline concatenation results, and $P_c(H)$ is their union.

During the concatenation, we maintain the current optimal result (i.e., the shortest one satisfying the constraint $\overline{C}$) and keep updating it. Finally, after all the candidates are generated and validated, we return the optimal one as the \textit{MCSP} result. For example, given a query $q(v_9,v_7,\{6\})$, the \textit{LCA} of $v_9$ and $v_7$ in the tree is $X_1$, and it contains vertices $H=\{v_1,v_5,v_8,v_{12}\}$. For hop $v_1$, $L(v_9)[v_1]=\{(3,7),(5,5)\}$ and $L(v_7)[v_1]=\{(3,5),(4,0)\}$. Therefore, we can get four candidates $P_c(v_1)=\{(6,12),(7,7),(8,10),(9,5)\}$. Only $(9,5)$ has a cost smaller than $6$, so $(9,5)$ is the current best result. For hop $v_5$, we can get candidates $P_c(v_5)=\{(4,9),(5,6),$ $(6,7),(7,4)\}$. Then $(5,6)$ replaces $(9,5)$ as it has smaller weight and meet the constraint condition as well. For hop $v_8$, we can get candidates $P_c(v_8)=\{(4,5)\}$, and the current best result is updated to $(4,5)$. Finally, for hop $v_{12}$, we obtain the candidate $P_c(v_{12})=\{(4,5)\}$, which is equal to the current best result. The final result is $(4,5)$. 

As shown in the above example, although only 4 hops are needed, we actually run 10 path concatenation operations. Specifically, unlike the 2-hop labeling of the single-criterion case where only $|H|$ times of adding is needed, the concatenation of the skyline paths makes hop computation much more time-consuming. Suppose the label of $s$ to $h$ has $m$ skyline paths and the label of $h$ to $t$ has $n$ skyline paths. Then for each intermediate hop, we have to compute $mn$ times, and the total time complexity grows to $O(mn|H|)$ instead of $O(|H|)$. Therefore, pruning over this large amount of computation is crucial to the query performance and we will elaborate it in Section \ref{sec:Skyline}.



%\begin{table*}[ht]
%\centering
%\caption{Partial CSP-2Hop Labels}
%\label{table:CSP-2Hop}
%%\scriptsize
%\scalebox{0.75}{
%\begin{tabular}{|c|c|c|c|c|c|}
%\hline
%\textbf{Ancestors} & \textbf{$v_4$} & \textbf{$v_1$} & \textbf{$v_5$} & \textbf{$v_8$}                                                        & \textbf{$v_{12}$}                                              \\ \hline
%\textbf{$v_7$}     & -              & (3, 5),(4, 0)  & (1, 3),(3, 1)         & (3, 3)                                                                & (2, 2)                                                         \\ \hline
%\textbf{$v_9$}     & (2, 4),(3, 1)  & (3, 7),(5, 5)  & (3, 6),(4, 3)  & (1, 2)                                                                & (2, 3)                                                         \\ \hline
%\textbf{$v_4$}     & -              & (2, 4),(4, 3)  & (1, 2)         & (1, 2)                                                                & (2, 3)                                                         \\ \hline
%\textbf{$v_1$}     & -              & -              & (2, 2),(3, 1)  & (3, 6),(5, 5) (6, 4),(7, 3) & (4, 7),(6, 2)                                                  \\ \hline
%\textbf{$v_5$}     & -              & -              & -              & (2, 4),(3, 3)                                                         & (3, 5),(4, 4) (5, 3) \\ \hline
%\textbf{$v_8$}     & -              & -              & -              & -                                                                     & (1, 1)                                                         \\ \hline
%%\textbf{$v_{12}$}  & -              & -              & -              & (1, 1)                                                                & -                                                              \\ \hline
%\end{tabular}}
%\end{table*}

\subsection{Index Construction}
\label{subsec:MCSP2Hop_Construction}
The index construction is made up of two phases: a bottom-up \textit{Skyline Tree Decomposition} that gathers the skyline shortcuts, creates the tree nodes and forms the tree, and a top-down \textit{Skyline Label Assignment} that populates the labels with query answering, \mycolor{as shown in Algorithm \ref{Algorithm:Construction}}. \mycolor{It should be noted that both of these two phases do not involve the expensive skyline path search and only use the skyline path concatenation.}
\begin{algorithm}[ht]
	\caption{MCSP-2Hop Construction}
	\label{Algorithm:Construction}
%	\scriptsize
	\LinesNumbered
	\KwIn{Graph $G(V,E)$}
	\KwOut{MCSP-2Hop Labeling $L$}
	//	Tree Node Contraction\\
	\While{$v\in V$ has the minimum degree and $V\neq \phi$}
	{
		$X_v=N(v)$, $r(v)\leftarrow$ Iteration Number\\%\Comment{Tree Node Contraction}\\
		\For{$(u,w)\leftarrow N(v)\times N(v)$}
		{
			$P(u,w)\leftarrow Skyline(p(u,v)\oplus p(v,u), (u,w))$\;
			$E\leftarrow E\cup (P(u,w))$, $V\leftarrow V-v$, 	$E\leftarrow E-(u,v)-(v,w)$\;
		}
	}
	// Tree Formation\\
	\For{$v$ in $r(v)$ increasing order}
	{
		$u\leftarrow min\{r(u)|u\in X(v)\}, X_v.Parent\leftarrow X_u$%\Comment{Tree Formation}
	}
	// Label Assignment\\
	$X_v\leftarrow$ Tree Root, $Q.insert(X_v)$\\%\Comment{Label Assignment}\\
	\While{$X_v\leftarrow Q.pop()$}
	{
		\For{$u\in \{u|X_u$ is ancestor of $X_v\}$}
		{
			$P(v,u))\leftarrow Skyline(P(v,w)\oplus P(w,u)), \forall w\in X_v$\;
			$L(v)\leftarrow{(u,P(v,u))}$\;
		}
		$Q.insert(X_u.children)$, $L\leftarrow L\cup L(v)$\;
	}
\end{algorithm}
%\subsubsection{Skyline Tree Decomposition}
%\label{subsec::Construction_TD}
%The skyline tree decomposition is made up of two steps: \textit{node contraction} that forms the tree nodes and \textit{tree construction} that organizes these nodes into a tree.
\subsubsection{\mycolor{Skyline Tree Decomposition}}
\label{subsubsec:CSP2Hop_TD_Contraction}
We contract the vertices in the degree-increasing order, which is created by \textit{Minimum Degree Elimination}\cite{gong2019skyline,li2019scaling}. For each $v\in V$, we add a skyline shortcut $p'(u,w)$ to all of its neighbor pairs $(u,w)$ by $p(u,v)\oplus p(v,w)$. If $(u,w)$ does not exist, then we use $p'_s(u,w)$ as its skyline path $p(u,w)$ directly. Otherwise, we compute the skyline of $p(u,w)$ and $p'(u,w)$ in a linear time sort-merge way, \mycolor{which sorts the two path sets based on $w$ first and obtain the new skyline paths by comparing them in the distance-increasing order}. After that, a tree node $X(v)$ is formed with $v$ and its neighbors $N(v)$, and all their corresponding skyline paths from $v$ to $N(v)$. The tree node $X(v)$ is assigned an order $r(v)$ according to the order when $v$ is contracted. After contracting $v$, $v$ and its edges are removed from $G$ and the remaining vertices' degree are updated. Then we contract the remaining vertices in this way until none remains. \mycolor{The time complexity of the contraction phase is $O(|V|(max(|X_i|)^{2}\cdot n\cdot  c^{2(n-1)}_{max}\log c_{max}+\log |V|))$, where $max(|X_i|)$ is the tree width, $c_{max}$ is the longest edge cost (including weights) and $c_{max}^{n-1}$ determines the worst case of skyline path number, and $c^{2(n-1)}_{max}\log c^{2(n-1)}_{max}$ is concatenation complexity.}

We use the graph in Figure \ref{fig:ExampleGraph} as an example. Firstly, we contract $v_2$ with $N(v_2)=\{v_1,v_3,v_4\}$. Because there is no edge between $v_1$ and $v_3$, we add a shortcut $(v_1,v_3)$ with  by $w=w(v_1,v_2)+w(v_2,v_3)=2$ and $c=c(v_1,v_2)+c(v_2,v_3)=3$. Similarly, there is no edge between $v_1$ and $v_4$, so we add a new edge $(v_1,v_4)$ with $w=w(v_1,v_2)+w(v_2,v_4)=2$ and $c=c(v_1,v_2)+c(v_2,v_4)=4$. As for $v_4$ and $v_3$, we first generate a shortcut by $p(v_4,v_2)\oplus p(v_2,v_3)=(2,3)$. Then because there already exists an edge $(3,2)$ from $v_4$ to $v_3$, we compute the new skyline paths between the shortcut and the edge, and get the new skyline paths $p(v_4,v_3)=\{(3,2),(2,3)\}$. After that, we remove $v_2$ from the graph, leaving $v_1$'s degree changed to 4, $v_4$'s degree remaining 5, and $v_3$'s degree remaining 3. We also obtained a tree node $X(v_2,v_3,v_1,v_4)$ with the skyline paths from $v_2$ to $N(v_2)$ and order $r(v_2)=1$. This procedure runs on with the next vertex with the smallest degree. When all the vertices finished contraction, we have an order of $:v_2,v_3,v_6,v_7,v_{13},v_{11},$\\$v_{10},v_9,v_4,v_1,v_5,v_8,v_{12}$.

After that, we connect all the nodes to form a tree by connecting each tree node to its smallest order neighbor. For example, $X_{10}$ has a neighbor set of $\{v_9,v_9,v_{12}\}$ and $X_9$ has the smallest order of them, so $X_{10}$ is connected to $X_9$ as its child node.

\subsubsection{Skyline Label Assignment}
\label{subsubsec::CSP2Hop_TD_Label}
It should be noted the obtained tree preserves all the skyline path information of the original graph because every edge's information are preserved in the shortcuts. In fact, we can view it as a \textit{superset} of the \textit{MCSP-CH} result. Therefore, we can assign the labels with skyline search on this tree directly. However, it would be very time-consuming as the \textit{Sky-Dijk} is much slower than \textit{Dijkstra}'s. To this end, we use the top-down label cascading assignment method that takes advantages the existing labels with query answering to assign labels to the new nodes.

Specifically, a label $L(u)$ stores all the skyline paths from $u$ to its ancestors. Therefore, we start from the root of the tree to fill all the labels. For root itself, it has no ancestor so we just skip it. Next for its child $u$, because the root is the only vertex in $X(u)$ other than $u$, we add the root to $u$'s label. Then for any tree node $X(v)$, it is guaranteed that all its ancestors have obtained their labels. Then for any of its ancestor $a_i$, we compute its skyline paths by taking the skyline paths from  $\{p(v,u)\oplus p(u,a_i)| \forall u\in X(v)$\}. The time complexity of the label assignment phase is $O(|V|max(|X_i|) \cdot n\cdot c^{2n-2}_{max}\log c_{max})$, where $h$ is the tree height. The space complexity of the labels is $O(h\cdot |V|\cdot c^{n-1}_{max})$.

% with the \textit{multiple skyline path concatenation} described in Section \ref{subsec:Skyline_Multiple}. 

For example in Figure \ref{fig:Tree Decomposition}, suppose we have already obtained the labels of $X_1, X_5, X_8$, and $X_{12}$, and we are computing the labels of $X(v_4)$, which has an ancestor set of $\{v_{12}, v_8, v_5, v_1\}$. We take the computation of $L(v_4)[v_{12}]$ as example. $X_4$ has three vertices $\{v_1,v_5,v_8\}$ apart from $v_4$, so we compute the skyline paths via these tree hops. To show the process clearly, we do not apply the pruning first.
\begin{equation*}
%	\scriptsize
    \begin{aligned}
        P_c(h_1)&=p(v_4,v_1)\oplus p(v_1,v_{12})\\
        &=\{(2,4),(4,3)\}\oplus\{(4,7),(6,2)\}\\
        &=\{(6,11),(8,6),(8,10),(10,5)\}\\  
        P_s(h_1)&=\{(6,11),(8,6),(10,5)\}\\
    \end{aligned}
\end{equation*}
\begin{equation*}
    \begin{aligned}
        P_c(h_5)&=p(v_4,v_5)\oplus p(v_5,v_{12})\\
        &=\{(1,2)\}\oplus \{(3,5),(4,4),(5,3)\}\\
        &=\{(4,7),(5,6),(6,5)\}\\
        P_s(h_5)&=\{(4,7),(5,6),(6,5)\}\\
    \end{aligned}
\end{equation*}
\begin{equation*}
    \begin{aligned}
        P_c(h_8)&=p(v_4,v_8)\oplus p(v_8,v_{12})\\
        &=\{(1,2)\}\oplus\{(1,1)\}=\{(2,3)\}\\
        P_s(h_8)&=\{(2,3)\}
    \end{aligned}
\end{equation*}

Because $(2,3)$ dominates all the others, we put $(2,3)$ into the label of $L(v_4)[v_{12}]$. %If we use the \textit{query rectangle} pruning, we first compute three corresponding rectangles: $h_1:(6,11)\times (10,5)$; $h_5:(4,7)\times (6,5)$; $h_8:(2,3)$. Because $(2,3)$ dominates the other two rectangles, we prune $h_1$ and $h_5$ and return $(2,3)$ directly as the skyline path.
%The correctness of the label assignment procedure can be easily proved by induction. As the label values are essentially the query results using the existing labels of the ancestors, the results are correct as long as the ancestors' labels are correct. The labels are populated in the cascading way, and thus the correctness is naturally guaranteed. Therefore, the resulting label set is a \textit{CSP-2Hop}.

\subsection{Correctness}
\label{subsec:MCSP2Hop_Correctness}
In this section, we show that the \textit{MCSP-2Hop} constructed in Algorithm \ref{Algorithm:Construction} is correct, i,e., the \textit{MCSP} query between any source vertex $s$ and target vertex $t$ can be correctly answered.

As proved in Theorem \ref{the:Skyline}, the skyline paths between $s$ and $t$ are enough to answer any \textit{MCSP} query, so we only need to prove the candidate set $P_c(H)$ covers all the skyline paths between $s$ and $t$. Firstly, we introduce the following lemma:  
\begin{lemma}
	\label{lemma:SkylineSubpath}
	If a path $p$ is a skyline path, the sub-paths on $p$ are all skyline paths.
\end{lemma}
\begin{proof}
	The proof of it can be found in \cite{storandt2012route}.
\end{proof}

\begin{theorem}
	\label{the:HopSkyline}
	$P_c(h)$ covers all the skyline paths from $s$ to $t$ that travel via hop $h$.
\end{theorem}
\begin{proof}
	Suppose $p^*$ is a skyline path from $s$ to $t$ via $h$ and $p^*\notin P_c(h)$. According to Lemma \ref{lemma:SkylineSubpath}, $p^*$'s sub-paths $p^*(s,h)$ and $p^*(h,t)$ are also skyline paths from $s$ to $h$ and from $h$ to $t$. If $p^*(s,h)\notin P(s,h)$ or $p^*(h,t)\notin P(h,t)$, it contradicts the definition that $P(s,h)$ contains all the skyline paths from $s$ to $h$, and similar for $P(h,t)$. Therefore, $P_c(h)$ covers all the skyline paths from $s$ to $t$ via $h$.
\end{proof}

Next we need to prove the union of all the hops $h\in H$ covers all the skyline paths between $s$ and $t$. Because our 2-hop labeling is based on the graph cut, we only need to prove the following theorem:
\begin{theorem}
	\label{the:CSP-2Hop}
	If the hop set $H$ is the set of cuts between $s$ and $t$, then $P_c(H)=\bigcup_{h_i\in H} P_c(h_i)$ covers all the skyline paths from $s$ to $t$.
\end{theorem}
\begin{proof}
	Similar to Theorem \ref{the:HopSkyline}, we also prove it with contradiction. Suppose $p^*$ is a skyline path and $p^*\notin P_c(H)$. Because $H$ is the graph cut set, $p^*$ has to travel through one of the cut vertex $h_i\in H$, which has a candidate set $P_c(h_i)$. However, $p^*\notin P_c(h_i)$ contradicts with Theorem \ref{the:HopSkyline}. So every skyline path from $s$ to $t$ exists in $P_c(H)$.
\end{proof}

\mycolor{Finally, we prove the labels generated by Algorithm \ref{Algorithm:Construction} is a \textit{MCSP-2Hop}.}
\begin{theorem}
	\mycolor{$L$ constructed by Algorithm \ref{Algorithm:Construction} is \textit{MCSP-2Hop}, that is $\forall (v,P(u,v))\in L(u), (u, v\in V)$, the path set $P(u,v)$ covers skyline paths between $u,v$.}
\end{theorem}
\begin{proof}
	\mycolor{Firstly, we define graph $G(v)$ as the assembly of tree nodes from $X_v$ to the root of \textit{skyline tree decomposition} $T_G$. It can be easily obtained that $G(v)$ is \textit{skyline preserved} by referring to the \textit{distance preserved property} of tree decomposition in \cite{ouyang2018hierarchy}. Next, we prove that $P(u,v)$ covers skyline paths between $u,v$ through induction. We suppose that height $h$ of tree root is zero and the height of one tree node is its parent's height plus one. For the root with $h=0$, its label are \textit{MCSP-2Hop}. For $X_v$ with height $h=1$, the labels in $L(v)$ is also \textit{MCSP-2Hop} because of the skyline preserved property. Then suppose that labels in $L(v)$ with height $h=i (i>1)$ is \textit{MCSP-2Hop}, we attempt to prove that labels in $L(u)$ with $h=i+1$ are also \textit{MCSP-2Hop}. Since $G(u)$ is skyline preserved with $X_u\setminus \{u\}$ being $u's$ neighbor set in $G(u)$, then all the skylines paths must pass through vertices in this set. According to the top-down label assignment, the labels is obtained by concatenating the two paths with $X_u\setminus \{u\}$ being the hops, so the computed labels in $L(u)$ are also \textit{MCSP-2Hop}. Therefore, $L$ constructed by Algorithm \ref{Algorithm:Construction} is \textit{MCSP-2Hop}.}
\end{proof}

%In summary, our \textit{CSP-2Hop} is able to answer any \textit{CSP} query correctly with label concatenation. 
 
\subsection{Path Retrieval}
\label{subsec:MCSP2Hop_Path}
To retrieve the actual result path, we need to preserve the intermedia vertex in the labels. Specifically, during the \textit{Tree Node Contraction} phase, we need to store the contracted vertex of each skyline path in each shortcut. During the path retrieval, suppose one of the skyline results is the concatenation of $s\rightarrow h$ and $h\rightarrow t$, then they are actually two shortcuts so we only need to insert the intermediate vertices recursively until all no shortcut remains to recover the original path.






==> CSP-H2H (VLDBJ)/Conclusion.tex <==
\section{Conclusion}
\label{sec:Conclusion}
In this paper, we have proposed forest-based skyline path index structure to answer the \textit{MCSP} query efficiently. Moreover, we have proposed several skyline path concatenation methods to support index construction and query answering. The new path concatenation paradigm enables indexing and storing the complete exact skyline paths. A range of pruning techniques have been developed for the single pair concatenation, multiple hop concatenation, \textit{MCSP} query answering, and forest query answering. Extensive evaluations on real-life road networks have demonstrated that our new methods can outperform the state-of-the-art \textit{MCSP} approaches by several orders of magnitude, and our pruning techniques can provide a further 10x speedup. 

==> CSP-H2H (VLDBJ)/Construction.tex <==
\section{CSP-2Hop Construction}
\label{sec:Construction}
The index construction is made up of two phases: a bottom-up \textit{Skyline Tree Decomposition} that gathers the skyline shortcuts, creates the tree nodes and forms the tree using the concatenation discussed in Section \ref{subsec:Skyline_Full}, and a top-down \textit{Skyline Label Assignment} that populates the labels with query answering discussed in Section \ref{subsec:Skyline_Multiple}. It should be noted that both of these two phases do not involve the expensive skyline path search and only use the skyline path concatenation.

%\begin{figure}[ht]
%    \centering
%    \includegraphics[scale=0.5]{example_cutting.png}
%    \caption{}
%    \label{fig:example_cutting.png}
%\end{figure}

%We can thus apply cutting set on two skyline path sets, which shown in Figure \ref{fig:example_cutting.png}. The definition are in the following: 

%\begin{definition}[cutting set]
%Suppose all the skyline paths in $P(h_i)$ and $P'(h_i)$ are sorted by weight with an ascending order, $c_1$ is a cutting set for $P(h_i)$, which includes $x_1$ skyline paths from $p_1$ to $p_{x_1}$, where $0 \leq x_1 \leq m$. $c_2$ is a cutting set for $P'(h_i)$, which includes $x_2$ skyline paths from $p'_1$ to $p_{x_2}$, where $0 \leq x_2 \leq n$. In $c_1$, we must ensure that the weight of the last skyline path $W(p_{x_1}) \leq W(p'_{{x_2}+1})$. In $c_2$, we must guarantee $W(p'_{x_2}) \leq W(p'_{{x_1}+1})$. Therefore, all paths on the left of both $c_1$ and $c_2$ have smaller weight than the paths on the right of $c_1$ and $c_2$. 
%\end{definition}

%In order for the condition of cutting set to be true, when we generate cutting set for $P(h_i)$ and $P'(h_i)$, we need the principles in the following:

%\begin{enumerate}
%\item Find the last path $p_{x_1}$ in $c_1$ and the last path $p'_{x_2}$ in $c_2$. If $W(p_{x_1}) \geq W(p'_{{x_2}+1})$,  we move $p_{x_1}$ out of $c_1$ and move $p_{{x_2}+1}$ into $c_2$. When $c_1$ has only one path, just  move one path into $c_2$.
%\item If $W(p_{x_2}) \geq W(p'_{{x_1}+1})$,  we move $p_{{x_1}+1}$ into $c_1$ and move $p_{x_2}$ out of $c_2$. When $c_2$ has only one path, just  move one path into $c_1$.
%\item Repeat step 1 and step 2 until all the paths on the left of $c_1$ and $c_2$ have smaller weight than the paths on the right of $c_1$ and $c_2$.
%\end{enumerate}

%Hence, we propose a way to connect skyline paths in two sorted sets $P(h_i)$ and $P'(h_i)$ by means of cutting set. 

%In Figure \ref{fig:example_cutting.png}, suppose $h_i$ is the only intermediate hop from $s$ to $t$. In the basis of corollary \ref{corollary 2}, we can confirm the first $s-t$ skyline path $p_1^1$, which has the lowest weight and highest cost, by connecting $p_1$ in $P(h_i)$ and $p'_1$ in $P'(h_i)$. Afterward, we generate cutting set $c_1$ for $P(h_i)$ and cutting set $c_2$ for $P'(h_i)$. In current, $c_1$ and $c_1$ have $p_1$ and $p'_1$, respectively. Then, we compare the weight between $p_1$ and $p'_2$, if $W(p_1) \geq W(p'_2)$, thus $W(p'_1) \leq W(p_2)$, we add $p'_2$ into $c_2$. As $c_1$ only has one path, we skip the operation of moving for $c_1$. (rewrite later)




%\subsection{Labeling Approach}
%Given a road network $G(V,E)$, tree decomposition $T_G$ can be built based on the concept of a vertex cut, which is defined as follows\cite{ouyang2018hierarchy}: 

%\begin{definition}[Vertex Cut]
%Given a road network $G(V,E)$, a subset of vertices $\Gamma \subset V$ is a vertex cut of $G$ if $G$ can be partitioned into several connected components by removing all the vertices in $\Gamma$. A set $\Gamma$ is the vertices cut of vertices $u$ and $v$ if $u$ and $v$ are in different components partitioned by removing $\Gamma$ from $G$.
%\end{definition}

%Therefore, if vertices $s$ and $t$ have a vertex cut $\Gamma$, we can infer that every path from $s$ to $t$ must via at least one vertex in $\Gamma$.
%By the property 3 of Tree Decomposition, if $s$ in node $X(s)$ and $t$ in node $X(t)$ are located at different sub-trees, we can regard the lowest common ancestor (LCA) of $X(s)$ and $X(t)$ as a vertex cut of $s$ and $t$ in $G$.

%Hence, in CSP-2hop index, for a CSP query ($s, t, C$), we treat the LCA of $s$ and $t$ in $T_G$ as the intermediate hop set $H$, each vertex in $H$ will be one intermediate hop. Hence, if we can pre-compute all the skyline paths from $s$ to each vertex in $\Gamma$ and the skyline paths from such vertices in $\Gamma$ to $t$, by using the query processing method of CSP-2hop index, we can further obtain a set of skyline paths via different vertices in $\Gamma$ and return the optimal result of CSP with the cost less than $C$. Furthermore, to answer CSP queries with any two vertices, we expect to know ahead of time all the skyline paths from each vertex in an arbitrary node $X(n)$ in $T_G$ to each vertex in every ancestor node of $X(n)$.   

\subsection{Skyline Tree Decomposition}
\label{subsec::Construction_TD}
The skyline tree decomposition is made up of two steps: \textit{node contraction} that forms the tree nodes and \textit{tree construction} that organizes these nodes into a tree.

\subsubsection{Skyline Tree Node Contraction}
\label{subsubsec::Construction_TD_Contraction}
We contract the vertices in the degree-increasing order. For each $v\in V$, we add a skyline shortcut $p'(u,w)$ to all of its neighbor pairs $(u,w)$ by $p(u,v)\oplus p(v,w)$. If $(u,w)$ does not exist, then we use $p'_s(u,w)$ as its skyline path $p(u,w)$ directly. Otherwise, we compute the skyline of $p(u,w)$ and $p'(u,w)$ in a linear time sort-merge way because the skyline paths produced by Algorithm \ref{Algorithm:GreedyConcatenation} are ordered by weight. After that, a tree node $X(v)$ is formed with $v$ and its neighbors $N(v)$, and all their corresponding skyline paths from $v$ to $N(v)$. The tree node $X(v)$ is assigned a order $r(v)$ according to the order when $v$ is contracted. After contracting $v$, $v$ and its edges are removed from $G$ and the remaining vertices' degree are updated. Then we contract the remaining vertices in this way until none remains. 

We use the graph in Figure \ref{fig:ExampleGraph} as the example. Firstly, we contract $v_2$ with $N(v_2)=\{v_1,v_3,v_4\}$. Because there is no edge between $v_1$ and $v_3$, we add a shortcut $(v_1,v_3)$ with  by $w=w(v_1,v_2)+w(v_2,v_3)=2$ and $c=c(v_1,v_2)+c(v_2,v_3)=3$. Similarly, there is no edge between $v_1$ and $v_4$, so we add a new edge $(v_1,v_4)$ with $w=w(v_1,v_2)+w(v_2,v_4)=2$ and $c=c(v_1,v_2)+c(v_2,v_4)=4$. As for $v_4$ and $v_3$, we first generate a shortcut by $p(v_4,v_2)\oplus p(v_2,v_3)=(2,3)$. Then because there already exists an edge $(3,2)$ from $v_4$ to $v_3$, we compute the new skyline paths between the shortcut and the edge, and get the new skyline paths $p(v_4,v_3)=\{(3,2),(2,3)\}$. After that, we remove $v_2$ from the graph, leaving $v_1$'s degree changed to 4, $v_4$'s degree remaining 5, and $v_3$'s degree remaining 3. We also obtained a tree node $X(v_2,v_3,v_1,v_4)$ with the skyline paths from $v_2$ to $N(v_2)$ and order $r(v_2)=1$. This procedure runs on with the next vertex with the smallest degree. When all the vertices finished contraction, we have an order of $\left<v_2,v_3,v_6,v_7,v_{13},v_{11},v_{10},v_9,v_4,v_1,v_5,v_8,v_{12}\right>$.

%When we contract $v_3$, it is obvious that the neighbours of $v_3$ change to $v_1$, $v_4$, and $v_9$. We insert edge ($v_1, v_4$) and ($v_1, v_9$) in the graph. Then, assign $w(v_1, v_3)+w(v3,v4)$, $c(v_1,v_3)+c(v_3,v_4)$ for ($v_1, v_4$) and $w(v_1, v_3)+w(v_3,v_9)$ ,$c(v_1,v_3)+c(v_3,v_9)$ for ($v_1, v_9$) . We eliminate $v_3$ and build $X(v_3)$ including $v_3$, $v_1$, $v_4$, and $v_9$. We contract the vertices according to the edges degree to build all the nodes for $T_G$ and the skyline paths between any two vertices in each node.   

\subsubsection{Skyline Tree Construction}
\label{subsubsec::Construction_TD_Construction}
The intuition behind the contraction procedure is that the neighbors of $v$ form a set of cuts from $v$ to the rest of the graph and they all have a higher order than $r(v)$. Therefore, all the vertices in $N(v)$ are the ancestors of $v$ in tree. To keep this property for all the vertices, we have to use the one with the smallest order $u = arg min(r(N(v)))$ as the direct parent of $v$ to form the tree. Otherwise, we cannot guarantee all the vertices in a tree node are the ancestors of its representative vertex. For example, $v_3$ has the smallest order in $X(v_2)$, so we add $X_2$ as $X_3$'s child. $r(v_9)$ is the smallest in $X(v_3)$, so we add $X_3$ as $X_9$'s child. In this way, we obtain a tree structure as shown in Figure \ref{fig:Tree Decomposition}.



%In this section, we illustrate an efficient method to construct the CSP-2Hop index. We first introduce how to find all the vertex cuts as nodes for constituting all a tree decomposition $T_G$ . Then we discuss how to efficiently calculate the skyline paths as in label and out label for vertices in each tree node.

%We generate vertex cuts as tree nodes by contracting each vertex with the vertex rank by edges degree. We first create a contracted graph $\overline{G}$ which is initialized as $G$. We begin to contract a vertex $v$ in $\overline{G}$ with the smallest degree and create corresponding node $X(v)$ in $T_G$. The node $x(v)$ must consist of $v$ and all its adjacent vertices in $\overline{G}$. Afterwards, we remove $v$ and all the adjacent edges from $\overline{G}$ but add edges into $\overline{G}$ to ensure all the adjacent vertices of $v$ in $\overline{G}$ can connect to each other. Following the order of edges degree, we contract all the vertices and build all the nodes in $T_G$.  

%As a CSP query may ask for a CSP path from a vertex to its one neighbour, the skyline paths between two adjacent vertices are necessary to preserve as index in $T_G$. Therefore, for every pair of adjacent vertices $(u,w)$ of $v$ in $\overline{G}$, if edge $(u,w)$ does not exist, we insert edge $(u,w)$ with weight $W(u,v)+W(v,w)$ and cost $C(u,v)+C(v,w)$. On the other hand, if edge $(u,w)$ exists in $\overline{G}$, we further check the dominance relations between path $<u,w>$ and another path $<u, v, w>$. If path $<u, v, w>$ dominates path $<u, w>$, we update the weight of edge $(u,w)$ as $W(u,v)+W(v,w)$ and the cost of edge $(u,w)$ as $C(u,v)+C(v,w)$. If path $<u, v, w>$ and path $<u, w>$ can not dominate each other, we add these two paths as two skyline paths between $u$ and $w$. In consequence, we eliminate vertex $v$ from $\overline{G}$, and generate $X(v)$ in $T_G$. Moreover, we rank each vertex by the order of vertices eliminated from $\overline{G}$. The earlier the vertex eliminate, the lower rank it has. We denote the rank as $\pi$. 



%\begin{figure}[ht]
%    \centering
%    \includegraphics[scale=0.35]{Tree1.png}
%    \caption{An example of tree decomposition}
%    \label{fig:Tree1.png}
%\end{figure}

%After finishing all the contraction, suppose $G$ has $n$ vertices, $n$ nodes can be created in $T_G$. For each of node, we can find the corresponding vertex in $G$. For any non-root node of size equal to one, its corresponding vertex is unreachable, as we cannot find the its neighbours in the node. Thus, for $T_G$, we only consider the nodes of size greater than one. The method to construct the nodes is in the following: First, we select a non-root node $X(v)$. Next, we find a vertex $u$ in $X(v)$, which has the lowest rank in $\pi$ except $v$. We set node $X(u)$ as the parent of $X(v)$ in $T_G$. For instance, Figure \ref{fig:Tree Decomposition} shows the final tree decomposition result of \ref{fig:ExampleGraph}. In node $X(v_4)$, except $v_4$, the vertex with the lowest rank in $\pi$ is $v_1$, we thus set $X(v_1)$ as the parents of $X(v_4)$. 

\subsection{Skyline Label Assignment}
\label{subsec::Construction_Label}
%To $T_G$, the straightforward method to calculate skyline paths is Skyline Dijkstra. We can use the algorithm to obtain skyline paths for any pair of vertices in $T_G$ by online searching. However, it will be very time-consuming, as we need to execute the algorithm for each pair of vertices. In this section, we introduce a method to calaculate CSP-2Hop labels with the tree decomposition example in \ref{fig:Tree Decomposition}.

It should be noted the obtained tree preserves all the skyline path information of the original graph because all every edge's information are preserved in the shortcuts. In fact, we can view it as a \textit{superset} of the \textit{CSP-CH} result. Therefore, we can assign the labels with skyline search on this tree directly. However, it would be very time-consuming as the \textit{Sky-Dijk} is much slower than \textit{Dijkstra}'s. To this end, we use the top-down label cascading method that takes advantages the existing labels with query answering to assign labels to the new nodes.

Specifically, a label $L(u)$ stores all the skyline paths from $u$ to its ancestors. Therefore, we start from the root of the tree to fill all the labels. For root itself, it has no ancestor so we just skip it. Next for its child $u$, because the root is the only vertex in $X(u)$ other than $u$, we add the root to $u$'s label. Then for any tree node $X(v)$, it is guaranteed that all its ancestors have obtained their labels. Then for any of its ancestor $a_i$, we compute its skyline paths by taking the skyline paths from  $\{p(v,u)\oplus p(u,a_i), \forall u\in X(v)$\} with the \textit{multiple skyline path concatenation} described in Section \ref{subsec:Skyline_Multiple}. 

For example in Figure \ref{fig:Tree Decomposition}, suppose we have already obtained the labels of $X_1, X_5, X_8$, and $X_{12}$, and we are computing the labels of $X(v_4)$, which has an ancestor set of $\{v_{12}, v_8, v_5, v_1\}$. We take the computation of $L(v_4)[v_{12}]$ as example. $X_4$ has three vertices $\{v_1,v_5,v_8\}$ apart from $v_4$, so we compute the skyline paths via these tree hops. To show the process clearly, we do not apply the pruning first.
\begin{equation*}
    \begin{aligned}
        P_c(h_1)&=p(v_4,v_1)\oplus p(v_1,v_{12})\\
        &=\{(2,4),(4,3)\}\oplus\{(4,7),(6,2)\}\\
        &=\{(6,11),(8,6),(8,10),(10,5)\}\\  
        P_s(h_1)&=\{(6,11),(8,6),(10,5)\}
    \end{aligned}
\end{equation*}
\begin{equation*}
    \begin{aligned}
        P_c(h_5)&=p(v_4,v_5)\oplus p(v_5,v_{12})\\
        &=\{(1,2)\}\oplus \{(3,5),(4,4),(5,3)\}\\
        &=\{(4,7),(5,6),(6,5)\}\\
        P_s(h_5)&=\{(4,7),(5,6),(6,5)\}
    \end{aligned}
\end{equation*}
\begin{equation*}
    \begin{aligned}
        P_c(h_8)&=p(v_4,v_8)\oplus p(v_8,v_{12})\\
        &=\{(1,2)\}\oplus\{(1,1)\}=\{(2,3)\}\\
        P_s(h_8)&=\{(2,3)\}
    \end{aligned}
\end{equation*}

Because $(2,3)$ dominates all the others, we put $(2,3)$ into the label of $L(v_4)[v_{12}]$. If we use the \textit{query rectangle} pruning, we first compute three corresponding rectangles: 
\begin{itemize}
    \item $h_1:(6,11)\times (10,5)$
    \item $h_5:(4,7)\times (6,5)$
    \item $h_8:(2,3)$
\end{itemize}
Because $(2,3)$ dominates the other two rectangles, we prune $h_1$ and $h_5$ and return $(2,3)$ directly as the skyline path.

The correctness of the label assignment procedure can be easily proved by induction. As the label values are essentially the query results using the existing labels of the ancestors, the results are correct as long as the ancestors' labels are correct. The labels are populated in the cascading way, and thus the correctness is naturally guaranteed. Therefore, the resulting label set is a \textit{CSP-2Hop}.
 
%As each node can be regarded as a vertex cut that separate corresponding vertices of its sub-trees nodes to independent parts. For instance, in Figure \ref{fig:Tree Decomposition}, if we remove all the vertices in node $X(v_1)$ from the example graph, we can not reach $v_6$ and $v_7$ from other remaining vertices. Moreover, for a node $X(v_i)$, we can notice that all the vertices in $x(v_i)$ except $v_i$ will be the ancestors of $v_i$. Thus, if we can calculate all the skyline paths from $v_i$ to each ancestor of $v_i$, given a CSP query $(s, t, C)$ and the LCA of $s$ and $t$, we can use our query processing by connecting skyline paths from $t$ to $v$ in the LCA $s$ skyline paths from $v$ to $t$.

%Hence, for arbitrary node $X(v_i)$ in $T_G$, we first pre-compute all the skyline paths from $v_i$ to other vertices in $X(v_i)$ and record it as labels of $v_i$ in the lookup table. In Figure \ref{fig:Tree Decomposition}, to $X(v_3)$, we can obtain the $P(v_3, v_9){(1, 4), (6,3)}$, $P(v_3, v_1){(2, 3)}$, and $P(v_3, v_4){((3,2),(2,3))}$. Then, we store them in the table of CSP-2Hop labels which shown in \ref{talbe:CSP-2Hop}. After calculating all the skylines in each node, we can use these information to obtain the skylines from $v_i$ to each ancestor of it.

%For each node $X(v_i)$, We build an ancestor set $X(v_i)_{anc}$. The vertices in $X(v_i)_{anc}$ must include all the vertices in $X(v_i)$ and other vertices which has higher rank than $v_i$. To calculate the skyline paths from $v_i$ to each vertices in $X(v_i)_{anc}$, suppose $X(v_i)$ has vertices {$v_i, v_a, v_b$}, and $X(v_i)_{anc}$ is {$v_i, v_a, v_b, v_e, v_f$}, as we have already know the skyline paths from $v_i$ to either $v_a$ and $v_b$ in the previous step, we only need to calculate the skyline paths from $v_i$ to $v_e$ and $v_f$. 

%\begin{figure}[ht]
%    \centering
%    \includegraphics[scale=0.25]{Tree2.png}
%    \caption{Labels of tree decomposition}
%    \label{fig:Tree2.png}
%\end{figure}

%\begin{figure}[ht]
%    \centering
%    \includegraphics[scale=0.25]{Lookup.png}
%    \caption{2 hop labeling lookup table for CSP}
%    \label{fig:Lookup.png}
%\end{figure}



==> CSP-H2H (VLDBJ)/Experiment.tex <==
\section{Experiment}
\label{sec:Experiment}
%In this section, we evaluate the performance of our \textit{CSP-2Hop} against the state-of-the-art exact \textit{CSP} methods. Section \ref{sec:Experimental Settings} shows the experimental settings. Sections \ref{subsec:Experiment_QueryEfficiency} and \ref{sec:Index Size and Construction Time} discuss the performance of query processing and index construction. %We also discuss the range of application for CSP-2Hop in \ref{sec:Range of Application}. 

\subsection{Experimental Settings}
\label{sec:Experimental Settings}
We implement all the algorithms in C++ with full optimizations. The experiments are conducted in a 64-bit Ubuntu 18.04.3 LTS with two 8-cores Intel Xeon CPU E5-2690 2.9GHz and 186GB RAM.
%\begin{table}[]
%\centering
%\caption{Datasets Used in the Experiments}
%\label{table:Datasets}
%\scriptsize
%\scalebox{1}{
%\begin{tabular}{|l|l|l|l|}
%\hline
%\textbf{Name} & \textbf{Description}   & \textbf{Vertices} & \textbf{Edges} \\ \hline
%\textbf{NY}   & New York City          & 264,346                     & 733,846                  \\ \hline
%\textbf{BAY}  & San Francisco Bay Area & 321,270                     & 800,172                  \\ \hline
%\textbf{COL}  & Colorado               & 435,666                     & 1,057,066                \\ \hline
%%\textbf{FLA}  & Florida                & 1,070,376                   & 2,712,798                \\ \hline
%%\textbf{CAL}  & California and Nevada  & 1,890,815                   & 4,657,742                \\ \hline
%%\textbf{LKS}  & Great Lakes            & 2,758,119                   & 6,885,658                \\ \hline
%%\textbf{CTR}  & Central USA            & 14,081,816                  & 34,292,496               \\ \hline
%%\textbf{USA}  & Full USA               & 23,947,347                  & 58,333,344               \\ \hline
%\end{tabular}}
%\end{table}

    \begin{figure*}[ht]
    	\centering
    	\includegraphics[width=6.8in]{Size.pdf}
    	\caption{Index Size (Bar) and Construction Time (Ball) of Different Partition Sizes, Boundary Contraction Orders, and Algorithms in 2-Graph}
    	\label{fig:Exp_Size}
    \end{figure*}

\textbf{Datasets}. 
All the tests are conducted in three real road networks obtained from the $9^{th}$ DIMACS Implementation Challenge \footnote{http://users.diag.uniroma1.it/challenge9/download.shtml}. %as shown in Table \ref{table:Datasets}. %\textit{NY}, \textit{BAY}, and \textit{COL} are three smaller networks and \textit{FLA} is larger. 
Specifically, \textit{NY} is a dense grid-like urban area with 264,246 vertices, 733,846 edge, and several partitions connected by bridges. \textit{BAY} has a shape of doughnut around the \textit{San Francisco Bay} with 321,270 vertices, 800,172 edges, and several bridges connecting the banks. \textit{COL} has an uneven vertex distribution (dense around Denver but sparse elsewhere) with 435,666 vertices and 1,057,0666 edges. We use the road length as the weight $w$ and travel time as the first cost to test the performance of \textit{CSP}. We also generate two cost sets that have random and negative correlation with the distance for each network, and generate three more positive correlation costs for \textit{MCSP} tests. %Finally, we test four social networks: $G_1:$ \textit{Anybeat}\footnote{http://networkrepository.com} with 12.6k vertices and 67.1k edges; $G_2:$ \textit{FB-PAGES-COMPANY}$^4$ with 14.1k vertices and 52.1k edges; $G_3:$ \textit{FB-PAGES-SPORT}$^4$ with 13.9k vertices and 86.8k edges;  $G_4:$ \textit{Github}\footnote{https://snap.stanford.edu/data/} with 37k vertices and 289k edges. Their tree widths are 698, 1710, 2527, and 6157, while the road networks' are 131, 107, and 168}.

%As for the cost $c$, we test the following three scenarios:
%\begin{enumerate}
%    \item \textit{Positive Correlation}: The cost grows proportionally to the distance such travel time and fuel consumption, and we use the travel time in the dataset directly.
%    \item \textit{Random}: The cost has no clear relation with distance like the slope gradient, and we generate it randomly.
%    \item\textit{Negative Correlation}: The cost drops proportionally to the distance that causes the worst case in the skyline operations. We use the equation $c=\frac{k}{w}, k \in \mathbb{R}^+$ to generate cost for each edge.
%\end{enumerate}

%or each edge, it includes two criteria, which are travel time and travel distance. In the experiments, we treat travel distance as the weight, and travel time as the cost. The dataset sizes are in the range from small cities in USA to the full USA road networks.


\textbf{Algorithms}. We extend the following state-of-the-art exact \textit{CSP} algorithms to their \textit{MCSP} versions \cite{DBLP:conf/adc/ZhangLZL21}: \textit{Sky-Dij} \cite{hansen1980bicriterion}, \textit{cKSP} \cite{gao2010fast}, %is the $k$-Shortest path with pruned search; 
\textit{eKSP} \cite{SEDENONODA2015602}, %is the $k$-Shortest path with pruned concatenation; 
\textit{CSP-CH} \cite{storandt2012route}, \textit{COLA} \cite{wang2016effective} with $\alpha$=$1$. We denote our methods as \textit{C2Hop} and \textit{F2Hop}. The straightforward version (as implemented in \cite{Liu2021Forest}) is denoted as \textit{F2Hop-S}.
%\textit{CSP-2Hop} as \textit{C2Hop} and the forest version as \textit{F2Hop}.
% for exact CSP query processing. %The algorithms we implemented are shown as follows:
%\begin{itemize}
%    \item \textbf{Sky-D} \cite{hansen1980bicriterion}: Skyline \textit{Dijkstra};
%    \item \textbf{cKSP} \cite{gao2010fast}: $k$-Shortest path with pruned search;
%    \item \textbf{eKSP} \cite{SEDENONODA2015602}: $k$-Shortest path with pruned concatenation;
%    \item \textbf{CSP-CH} \cite{storandt2012route}: \textit{CH} for \textit{CSP} with skyline shortcuts;
%    \item \textbf{COLA} \cite{wang2016effective}: We use the same partition and set its $\alpha=1$;
%    \item \textbf{C2Hop-DC}: \textit{CSP-2Hop} using divide-and-conquer for skyline path validation in construction, and constraint pruning in query processing as used in \cite{wang2016effective};
%    \item \textbf{C2Hop-G}: \textit{CSP-2Hop} with greedy concatenation; 
%    \item \textbf{C2Hop-GM}: \textit{CSP-2Hop} with greedy concatenation and multiple hops screening;
%\end{itemize}
%\textit{COLA} \cite{wang2016effective} is not compared here because its essential idea is using the approximate skyline path search to reduce partial skyline results, whose exact version is the same as \textit{Sky-D}. However, due to its slowness as shown in Section \ref{subsec:Experiment_QueryEfficiency}, it would take weeks to construct an exact version. Besides, its query processing also involves \textit{Sky-D}, so it is not fair to compare the exact version of \textit{COLA} with our method.

%\begin{figure*}
%    \centering
%    \includegraphics[width=6.8in]{Exp_Distance.pdf}
%    \caption{Query Time of Different Distance in NY}
%    \label{fig:Exp_Distance}
%\end{figure*}
%
%\begin{figure*}
%    \centering
%    \includegraphics[width=6.8in]{Exp_Ratio.pdf}
%    \caption{Query Time of Different Constraint Ratio in NY}
%    \label{fig:Exp_Ratio}
%\end{figure*}

\textbf{Query Set}. 
For each dataset, we randomly generate five sets of OD pairs $Q_1$ to $Q_5$ and each has 1000 queries. Specifically, we first estimate the diameter $d_{max}$ of each network %with an approximation method
\cite{meyer2003delta}. Then each $Q_i$ represents a category of OD pairs falling into the distance range $[d_{max} / 2^{6-i}, d_{max}/2^{5-i}]$. For example, $Q_1$ stores the OD pairs with distances in range $[d_{max}/32, d_{max}/ 16]$ and $Q_5$ are the OD pairs within $[d_{max}/2, d_{max}]$. %The OD pairs are selected randomly and are collected by their corresponding sets. %We run each query five times and report the average time for the 1000 queries in each query set.
Then we assign the query constraints $C$ to these OD pairs. Firstly, we compute the cost range [$C_{min}, C_{max}$] for each OD. This is because if $C$\textless $C_{min}$, the optimal result can not be found then the query is invalid; and if $C$\textgreater$C_{max}$, the optimal results is the path with the shortest distance. %For this reason, we assign the cost within [$C_{min}, C_{max}$]. 
Furthermore, in order to test the constraint influence on the query performance, we generate five constraints for each OD pair: $C=r\times C_{max}+(1-r)\times C_{min}$, with $r=0.1, 0.3, 0.5, 0.7$ and 0.9. When $r$ is small, $C$ is closer to the minimum cost; and when $r$ is big, $C$ is closer to the maximum cost. This constraint generation method is applied on all the cost dimensions.
%The same procedure is applied to all the three cost correlation scenarios.

        %\vspace*{-6mm}

%\subsection{Forest Performance}
%\vspace*{-4mm}
\subsection{Index Size and Construction Time}
	\label{sec:Index Size and Construction Time}
	In this section, we first test the influence of the partition sizes and boundary contraction orders on index size and construction time. We use the 2-Graph as for the test and select the best ones for the higher dimensional tests. Specifically, we test the \textit{F2Hop}s and \textit{COLA} with three different partition sizes for each graph ($2k, 4k$, and $6k$), \textit{C2Hop} and \textit{CSP-CH} with no partition. In terms of contraction order, \textit{F2Hop-D} uses the degree elimination order with boundary label, \textit{F2Hop-PB} uses the partition order with boundary label, and \textit{F2Hop-PE} uses the partition order with the extended label. As shown in Figure \ref{fig:Exp_Size}, \textit{F2Hop} all have smaller index sizes and shorter construction time than \textit{C2Hop} because of the smaller tree sizes and parallel construction. Specifically among the \textit{F2Hop}s, \textit{F2Hop-PB} is the fastest and smallest \textit{F2Hop} because it has the smallest number of labels to construct, and \textit{F2Hop-PE} is the largest and slowest because it has the largest number of labels. It also shows that the partition order performs better than the degree elimination order in the boundary tree.  Among the baseline methods, \textit{COLA} also has a small index but it takes the longest time to construct because it uses \textit{Sky-Dijk} search. \textit{CSP-CH} takes the shortest time to construct the smallest index. In the following tests, we use $4k$ as the default partition and \textit{PB} as the boundary order and boundary label.
		
	Next, we test the index size and construction time in the higher dimensional graphs and the results are shown in Figure \ref{fig:Exp_SizeMulti}. Because \textit{COLA} already takes more than $10^4$ seconds in the 2-dimensional graph, we do not test it in the higher dimensional graphs. As for the \textit{F2Hop} and \textit{F2Hop-S}, they construct the same index so their index sizes are the same and we show them together as \textit{F2Hop Size}. As for the construction time, because they use different strategies so we distinguish them. Specifically, \textit{F2Hop} is faster than \textit{F2Hop-S} by less than $10\times$. \textit{CSP-CH} is faster in 2-dimensional but the construction time soars up in 3-dimensional, and takes longer than $10^5$ in higher dimensions so we do not show \textit{CSP-CH}'s performance on 4 and 5-graphs. This is caused by the explosion of the skyline path numbers on the entire graph, while our \textit{F2Hop} methods reduce it with forest. As for the construction time \textit{F2Hop}s, 3-graph takes an order of magnitude longer time than 2-graph, and 4-graph takes another order of magnitude longer time than 3-graph. This phenomenon demonstrates the influence of dimension number of costs on the \textit{MCSP} problem. However, compared with the 2 to 3 and 3 to 4, 5-graph's construction time is longer but is still on the same order of 4-graph. This is because the increase of skyline path slows down in higher dimensions. 
		
	\begin{figure}[h]
        \centering
    	\includegraphics[width=3.3in]{SizeMulti.pdf}
    	\caption{Index Size (Bar) and Construction Time (Ball) of $n$-Graphs}
    	\label{fig:Exp_SizeMulti}
    \end{figure}

	
		 %Nevertheless, \textit{F2Hop-PE} would have higher query efficiency as shown later, and only the partition order can support extended label, so we do not test \textit{F2Hop-D} further. Meanwhile, we use 4k as the default partition sizes of \textit{NY}, \textit{BAY}, and \textit{COL}, because they have the smallest index size and shortest construction time.


%	In Figure \ref{fig:CSP_Index}, we present the index construction time (bar) and index size (line) of \textit{C2Hop-GM}. %We use histogram and broken lines to respectively show the time consumption and space use. For the results, we limit the maximum time to ${2 \times 10^4}$ seconds.
%	\textit{CSP-CH} always has the smallest index size and least construction time, but its the query performance is much slower. On the contrary, \textit{C2Hop}'s efficiency is at the cost of larger index size and longer construction time. Among them, our pruning techniques can save more than half of \textit{C2Hop-N}'s construction time (shown in logarithm so not that apparent). Moreover, the index sizes also reflects the influence of network structure and cost correlation. \textit{BAY} has the smallest index size and fastest to construction because it has smaller number of skyline paths and tree width. Random and negative correlation costs have much larger index size and longer time because they have more skyline paths.

	%\subsubsection{Query Performance}
	%\textit{F2Hop-D} 
	%\textit{F2Hop-PB}
	%\textit{F2Hop-PE}
	%\textit{C2Hop}  	
%Test in the next section	
%	r=0.9 * 3 networks

%    \vspace*{-5mm}
	\begin{figure}[ht]
        \centering
    	\includegraphics[width=3.2in]{Concatenation.pdf}
    	\caption{Effectiveness of Skyline Concatenation of CSP}
    	\label{fig:Exp_Concatenation}
    \end{figure}
	
	\subsection{Effectiveness of Skyline Concatenation}
	In this section, we study the effectiveness of our proposed skyline concatenation methods: \textit{F2Hop-DC} uses the classic \textit{Divide-and-Conquer}, \textit{F2Hop-E} uses our \textit{Efficient concatenation} for \textit{CSP}, and \textit{F2Hop-EM} further applies the \textit{Multi-hop pruning} based on \textit{F2Hop-E}. %We test on \textit{F2Hop-PE} as it has more labels to amplify the difference. 
	As shown in Figure \ref{fig:Exp_Concatenation}, \textit{F2Hop-E} is faster than \textit{F2Hop-DC}, while \textit{F2Hop-EM} is the fastest. This validates the effectiveness of our concatenation methods. Therefore, we only use \textit{F2Hop-EM} as the concatenation algorithm in the latter experiments. Among the networks, although \textit{NY} is relatively small, it is denser than the other two so the query performance is worse. \textit{BAY} is always faster because it has smaller label size thanks to its ring-shape topology. \textit{COL}'s $Q_1$ is worse than its $Q_2$ and $Q_3$ because the shorter queries have higher chance to fall into the dense Denver city and the mid-range query have higher chance to fall into the mountains and canyons.  
	
	\begin{figure}[ht]
        \centering
    	\includegraphics[width=3.3in]{ConcatenationMulti.pdf}
    	\caption{Effectiveness of Skyline Concatenation in MCSP}
    	\label{fig:Exp_Concatenation_MCSP}
    \end{figure}

	For the higher dimensional cases, we further test our \textit{MCSP}  concatenation techniques and compare with the techniques for \textit{CSP}. The query sets are $Q_3$ with $r=0.5$. As shown in Figure \ref{fig:Exp_Concatenation_MCSP}, we can further achieve a nearly one order of magnitude faster concatenation speed.
	

%\vspace*{-5mm}
	\subsection{Query Performance}
	\label{subsec:Experiment_QueryEfficiency} 
%	In this section, we test the influence of the following parameters: distances ranging from $Q_1$ to $Q_5$, constraint ratios ranging from 0.1 to 0.9, and three different networks. %The default settings of them are: $r=0.5$, \textit{NY} road network. 
%	\textit{F2Hop-D, F2Hop-PB, F2Hop-PE, C2Hop, COLA, CSP-CH Sky-Dij, cKSP, eKSP
    \subsubsection{Query Distance}
%    \textbf{0.1 0.5 0.9 * NY BAY COL, 9 Plots}
    Figure \ref{fig:Exp_Query} (a)-(c) show the query processing time of different algorithms in distance-increasing order with $r=0.5$. Firstly, all \textit{CSP-2Hop} methods outperform the others by several orders of magnitude. Among them, \textit{C2Hop} is the fastest that runs in $10^{-5}$ seconds because it has the largest label size and only needs one multi-hop concatenation. \textit{F2Hop-PE} is only slightly slower because it also has a large index size. \textit{F2Hop-PB} is slower running in $10^{-3}$ seconds but it has the smallest index size and is the fastest to construct. Secondly, all the algorithms' running time increase as the distance increases. Compared to the other methods, the \textit{CSP-2Hop} methods are more robust as their running time only increase slightly. Among the comparing methods, when the ODs are near to each other, like $Q_1$ and $Q_2$, all of them can finish in 10 seconds. When the distance further increases, some of them soar up to thousands of seconds. Specifically, $cKSP$ is always the slowest one because it uses the pruned \textit{Dijkstra} search to generate and test the $k$ shortest paths in the distance-increasing order. Therefore, when the OD is far away from each other, there could enumerate a huge number of possible paths. The second slowest is \textit{Sky-Dij}, which has a huge amount of intermediate skyline paths to expand before reaching the destination. \textit{eKSP} is slightly faster than them because it avoids the expensive \textit{Dijkstra} search and uses the path concatenation instead. \textit{CSP-CH} is faster as expected, but its performance also deteriorates dramatically in $Q_4$ and $Q_5$. Finally, \textit{COLA} also tends to be stable because its query time is bounded by the inner-partition search, and inter-boundary results are precomputed regardless of the actual distance. %Nevertheless, its performance is still slower. 
    In summary, our \textit{CSP-2Hop} is orders of magnitude faster and also robust in terms of different distances.  

    \begin{figure}[ht]
    	\centering
    	\includegraphics[width=3.3in]{Query.pdf}
    	\caption{CSP Query Performance of Distance and Ratio}
    	\label{fig:Exp_Query}
    \end{figure} 
%    the \textit{C2Hop-N} is the slowest and runs in $10^{-3}$ seconds. The greedy version \textit{C2Hop-G} is an order faster, and our final algorithm \textit{C2Hop-GM} is further another order faster in $10^{-5}$ seconds. This result proves the effectiveness and efficiency of the proposed greedy concatenation and multi-hop screening. 

%    \begin{figure*}[ht]
%    \centering
%    \includegraphics[width=6.8in]{Exp_Correlation.pdf}
%    \caption{Query Time Under Different Cost Correlations and Network Structures}
%    \label{fig:Correlation}
%    \end{figure*}
%    
%    \begin{figure}[ht]
%    \centering
%    \includegraphics[width=3.3in]{Exp_Index.pdf}
%    \caption{Index Construction Time and Size}
%    \label{fig:CSP_Index}
%\end{figure}

    \subsubsection{Constraint Ratio}
%    \textbf{Q4 * NY BAY COL, 3 Plots}
    Figure \ref{fig:Exp_Query} (d)-(f) show the influence of the constraint ratio $r$, %Although the results appear to be flat because the time is shown in \textit{log}, 
    and there are several interesting trends. Firstly, \textit{CSP-2Hop} is still robust and fastest under different $r$. Secondly, the baseline methods fall into two trends: \textit{Sky-Dij} and \textit{CSP-CH} that grows as the $r$ increases, while \textit{cKSP} and \textit{eKSP} have a hump shape. It should be noted that because the time is shown in logarithm, a very small change over $10^2$ in the plot actually has a very large difference. %These trends become more obvious when the query distance becomes larger ($Q_4$ and $Q_5$). 
    The reason of the increase trend is that \textit{Sky-Dij} and \textit{CSP-CH} expand the search space incrementally until they reach the destination, during which they accumulate a set of partial skyline paths. Therefore, when the $r$ is small, partial skyline path set is also small because most of the infeasible ones are dominated. When $r$ is big, the partial skyline path set becomes larger so it runs slower. As for the hump trend, the two \textit{KSP} algorithms test the complete paths iteratively in the distance-increasing order. Therefore, when $r$ is big, more paths would satisfy this constraint, so there is higher chance to enumerate only a few paths to find the result. In fact, they are even faster than \textit{CSP-CH} in $Q_4$ and $Q_5$ when $r=0.9$ (not shown here). On the other hand, when $r$ is small, large amounts of infeasible paths are pruned during the enumeration so the running time is also short. But when $r$ is not big or small, the pruning power becomes weak and the actual result is much longer than the shortest path, they have to enumerate tens of thousands of path to find it, so query performance deteriorates. 
%    \subsubsection{Cost Correlation}
%    Figure \ref{fig:Correlation}-(a) to (c) display the performance change of \textit{CSP} algorithms in \textit{NY} with different cost correlations. The efficiency of all the algorithms become worse when the cost correlation change from positive to negative. This is because in the negative correlation, nearly all the concatenation results are skyline, so skyline-based pruning techniques in all these algorithms lose their power. The performance of the greedy concatenation is also affected because it is approaching its worst case. However, the rectangle is still powerful and \textit{C2Hop-GM} still performs best.  %especially for \textit{CSP-CH} that has an extremely increasing of shortcuts as show in Figure \ref{fig:CSP_Index}. On the other hand, the performance of \textit{C2Hop-GM} is relatively robust and changed in the minimum. 

%	\begin{figure}[ht]
%    	\centering
%    	\includegraphics[width=3.5in]{Test.pdf}
%    	\caption{Criteria, Correlation, and Networks (Bar: Time; Ball: Size)}
%    	\label{fig:Exp_Test}
%    \end{figure} 
%    \vspace*{-5mm}
%	\subsection{Other Influence Factors}    
	\subsubsection{\mycolor{MCSP Query}}
	We test the \textit{MCSP} queries with $Q_3$ and $r=0.5$. As shown in Figure \ref{fig:Exp_MCSP}, \textit{F2Hop} are still orders of magnitude faster than the baseline. The performance of \textit{eKSP} looks stable because it is an enumeration-based method and we terminate the enumeration when more than $10k$ paths have been tested.  Its current performance is at the cost of failing answer some queries and bounded by $10k$ enumeration. 

	\begin{figure}[ht]
    	\centering
    	\includegraphics[width=3.3in]{MCSP.pdf}
    	\caption{MCSP Query Performance}
    	\label{fig:Exp_MCSP}
    \end{figure} 

	\subsubsection{Cost Correlation}
	We use the 2-dimensional index size and construction time to demonstrate the influence of the correlation. As shown in Figure \ref{fig:Exp_Correlation}, the positive correlation has the smallest index size and smallest construction time, and the negative correlation has the largest index size and longest construction time. This phenomenon is also caused by the \textit{skyline} itself instead of our index structure. When the criteria have negative correlations, the skyline number tends to increase to the worst square case. As a result, the query time increases dramatically for the baselines, while ours only increases slightly.
	
	\begin{figure}[ht]
    	\centering
    	\includegraphics[width=3.3in]{Correlation.pdf}
    	\caption{Performance under Different Correlations (Bar: Size; Ball: Time)}
    	\label{fig:Exp_Correlation}
    \end{figure} 
	
    %\subsubsection{\mycolor{Network Structure}}
   	%\mycolor{The results in Figure \ref{fig:Exp_Size}, \ref{fig:Exp_Concatenation}, \ref{fig:Exp_Query} reveal the road network structures' influence. Specifically, \textit{COL} is the largest one so it has the largest index size, longest construction time, while \textit{BAY} and \textit{NY} are similar because they are of similar size. In terms of the query performance, \textit{BAY} is always fastest and has a fewer difference of the concatenation methods as shown in Figure \ref{fig:ConcatenationExample}. This is because its vertices distribute like a doughnut rather than grids with fewer skyline paths and hops/cuts. Therefore, \textit{CSP-CH} has fewer shortcuts and performs better especially when query distance is long, and the \textit{C2Hop} methods perform closer to each other. \textit{COL} network is dense around Denver but sparse elsewhere. Therefore, for queries in $Q_2$ and $Q_3$, they have a higher chance to avoid Denver so fewer skyline concatenations occur. When the query distance increases, Denver increases the skyline size so \textit{F2Hop-DC} deteriorates. Finally, the performance gain of rectangle pruning is smaller for both \textit{BAY} and \textit{COL} because they have smaller a number of hops than \textit{NY}, which has larger skyline results due to its dense urban grid distribution.}

    %\mycolor{Figure \ref{fig:Exp_Test}-(e) and (f) demonstrate the results of other network structures. We use \textit{C2Hop} to test them because they are hard to partition. Because \textit{tree width} is an important factor in our algorithm's complexity, these networks that have a large tree width tend to have a long construction time even when the network size is small. They have small index sizes with fewer skyline paths because their hop number is small. This phenomenon also increases \textit{CSP-CH}'s construction time because it requires shortcuts among neighbors. In fact, the \textit{Tree Decomposition}-based methods are more suitable to the small tree width graphs like road network than social network. The most suitable hop labeling method for social network is \textit{PLL} \cite{akiba2013fast,zhang2021DWPSL}, but they require \textit{Sky-Dij} search during construction. Therefore, how to construct an efficient \textit{CSP} hop labeling for social network is still an open problem.}
    
    
    %We test all the comparative algorithms in three different USA road networks in Table \ref{table:Datasets}. Apart from the difference on data size, the structures of the networks possess different properties on density. Compared with BAY and COL, the distribution of vertices in NY is relatively average. For BAY, because of the geographical shape of itself, the graph is very sparse. Most of vertices only exist a few edges. For the structure of COL, the vertices present the distribution from sparse to dense. For example, most of queries with distance in the range of Q1 to Q3 deal with the vertices having a few neighbours. When the query distance increases, most of them will pass the dense area in COL such as Q4 and Q5.
    
    %The performance of the algorithms are shown in Figure \ref{fig:Correlation} (a), (d), (e). From the experiment results, we have the following observations. First of all, in all cases, the index-free methods present dramatically increasing trends when the query distance increases. \textit{C2Hop-GM} has obvious advantage on query time over other algorithms regardless of the network structures. \textit{cKSP} perform the worst in all cases. Especially, it cannot solve all the queries in the limited time, which is 200 seconds, in COL. In NY network, compared with\textit{Sky-D}, \textit{eKSP} has slight advantage in NY, but get worse in other two cases. \textit{Sky-D} performs the best among the index-free algorithms in the sparse network like BAY, as it only need to compute a few edges when it visit each vertex. To \textit{CSP-CH}, the query efficiency is extremely depend on the amount of shortcuts between each pair vertices. Thus, it can has good performance in BAY. We can notice that the query time of \textit{CSP-CH} decreases from Q3 to Q5. The reason is that the shape of BAY is a cyclic structure, the shortcuts can cover several pairs of vertices that has actually long distance in the graph. When the graph become dense, such as Q4 in COL, the cost of computing skyline paths will highly increase that result in the dramatically increasing of query time. The query performance of \textit{CSP-CH} is even worse than \textit{Sky-D} when the number of shortcuts is getting huge. For the three CSP-2Hop algorithms, we can see than the pruning techniques have obvious effects. The performance of \textit{C2Hop-GM} is over 10 times better than the naive way.
    
    %However, the gaps of query efficiency narrow down in BAY. This is due to the network structure of BAY. The sparse edges result in a small number of skyline index. Thus, the power of pruning become weak. In COL, as the query distance covers the area from sparse to dense, the gap between the naive method and other two pruning methods is getting greater.    



%On the contrary, \textit{C2Hop-GM} efficiently increases the query processing time but give way to the large amount of index size. The trade-off between the index size and query time is also the problem we need to improve in further. However,compared with \textit{C2Hop-N}, more than half of index time has already saved by \textit{C2Hop-GM}. Especially, \textit{C2Hop-N} will be out of memory in the cases of random and negative correlations.   
%Furthermore, we find that the size of skyline-based index, including \textit{CSP-CH} and \textit{C2Hop-GM}, will dramatically increase when two criteria of a network change from positive to negative. 


 





%\subsection{Range of Application}
%\label{sec:Range of Application}
%Based on the result of previous experiments, we will discuss the optimal scope of application for CSP-2Hop in this section

%(maxC-minC)*(0.1~0.9)+minC;
%Base	Q1	Q2	Q3	Q4	Q5
%0.1	0.00077366	0.0007265	0.00080714	0.00132284	0.00169608
%0.3	0.00063985	0.00074326	0.00081265	0.00172904	0.00266527
%0.5	0.00064156	0.00069536	0.00086102	0.00144243	0.00269132
%0.7	0.00066791	0.00070029	0.00091713	0.00147862	0.00227094
%0.9	0.00067279	0.0007274	0.00090925	0.00127389	0.00193278
%Base concatenation with varying constraints distribution  					
					
					
%Greedy	Q1	Q2	Q3	Q4	Q5
%0.1	0.0002063	0.00026211	0.00036821	0.00047642	0.00077767
%0.3	0.00014757	0.00022025	0.00033477	0.00040886	0.00072711
%0.5	0.00014685	0.00021971	0.00033187	0.00042095	0.00068358
%0.7	0.00014696	0.00021982	0.00032794	0.00036774	0.00062674
%0.9	0.00014701	0.00021898	0.00032307	0.00034488	0.00057175
%Greedy concatenation with varying constraints distribution 					
					
					
%Greedy+heuristic	Q1	Q2	Q3	Q4	Q5
%0.1	0.00010067	0.00009349	0.00009513	0.00013702	0.00014425
%0.3	0.00007561	0.0000814	0.00009138	0.00014021	0.00021433
%0.5	0.00007595	0.00024954	0.00009518	0.00013519	0.00020948
%0.7	0.00007602	0.00008214	0.00009695	0.00012685	0.00019539
%0.9	0.00007569	0.00008256	0.00009643	0.00011202	0.00017281
%Greedy+heuristic concatenation with varying constraints distribution 

%CSP-CH	Q1	Q2	Q3	Q4	Q5
%0.1	0.02014879	0.02253769	0.06740114	7.6183651	18.96739435
%0.3	0.02148223	0.02438478	0.07207377	10.46362957	25.5325083
%0.5	0.02007416	0.02302624	0.06838594	14.41601044	35.2746964
%0.7	0.0200423	0.02327397	0.07288994	17.98974218	44.9087403
%0.9	0.0202736	0.02346446	0.08252547	20.17059786	52.3914177

%random constraints
%Dij 0.09614689	1.75982195	22.45967466	265.7518132	518.620165
%CH 0.22068207	8.1270167	115.9040497 INF INF
%BASE 0.00051102	0.00051718	0.00074388	0.00225618	0.00230252
%greedy 0.00039749	0.00071117	0.00104313	0.00146343	0.00179389
%greedy+multi 0.0001154	0.00013951	0.00024648	0.00045484	0.00046888





==> CSP-H2H (VLDBJ)/Extension.tex <==
\section{Extensions}
\label{sec:Extensions}
%It is worth noting that our proposed index framework and the skyline path concatenation algorithm can be easily extended to other \textit{CSP} problems or solutions.

\subsubsection*{Multi-Criteria CSP (MCSP)}
In the multi-criteria network, each edge has a weight $w(e)$ and a set of costs $\{c_1(e),\dots,c_k(e)\}$. The \textit{MCSP} \cite{korkmaz2001multi} asks for the shortest path between an OD that satisfies all the given constraints $\{C_1,\dots,C_k\}$ over the corresponding criterion. To support \textit{MCSP}, we build the index for the multi-criteria skyline path \cite{kriegel2010route,gong2019skyline}, which can be easily extended from the two dimensional skyline. The concatenation follows the same procedure, while the rectangle pruning and the constraint pruning become hyper-cube pruning. 

\subsubsection*{Other Constraint Conditions}
The criteria can be roughly classified into \textit{additive} that takes the sum along a path like travel time and toll charge, and \textit{non-additive} \cite{wang1995bandwidth} that is determined by the bottleneck like maximum height/weight/width/gradient or road type. In this work, we use the \textit{maximum additive constraint} as the example, and we can easily convert it to the \textit{minimum additive constraint} by subtracting all the path costs from a value larger than the maximum cost. As for the \textit{non-additive constraints}, we replace the path cost by the min/max edge cost along it, and all the remaining skyline path concatenation procedures are the same.

\subsubsection*{Extension to CSP-CH}
Our skyline path concatenation method can also be extended to \textit{CSP-CH} to allow it store all the complete skyline shortcuts rather than a subset of it. In fact, the procedure described in Section \ref{subsubsec::Construction_TD_Contraction} creates a superset of the complete skyline shortcuts and can be used to answer \textit{CSP} query in the \textit{CH} way directly, and it is extremely fast to construct.

==> CSP-H2H (VLDBJ)/Forest.tex <==
\section{Forest Hop Labeling}
\label{sec:Forest}
Due to the nature of skyline, the \textit{MCSP-2Hop} size could be orders of magnitude larger than the distance labels, especially when the paths are long. Therefore, we present our \textit{Forest Hop Labeling} to reduce the index size by partitioning the graph into regions and building a small tree for each region, and a boundary tree between regions.

\subsection{Graph Partition}
\label{subsec:Forest_Parition}
We partition $G$ into a set $C=\{G_1,G_2,\dots,G_{|C|}\}$ of vertex-disjoint subgraphs such that $\bigcup_{i\in[1,|C|]}G_i=G$. If an edge appears in two different subgraphs, it is a \textit{Boundary Edge}, and its end vertices are called \textit{Boundary Vertex}. Graph partitioning is a well-studied problem and we could use any existing solutions. In our implementation, we use the state-of-art \textit{Natural Cut} method \cite{delling2011graph}, because such an approach can create only a small number of boundary vertices.

\subsection{Inner Partition Tree}
\label{subsec:Forest_Inner}
Conceptually, we build a small tree (\textit{MCSP-2Hop}) for each partition and these procedures can run in parallel. However, these trees cannot be constructed directly with only the subgraph information because the actual paths may take a detour out of the current partition and come back later. Therefore, we need to pre-compute the all-pair boundary results for each partition because these boundaries form the cut of a partition naturally and their all-pair results can cover all the detours. In other word, a complete graph of the boundaries is overlapped to the partition with each edge is a skyline path set. This procedure is also fast because we only need to run several search space reduced \textit{Sky-Dijk}s in parallel. When forming the tree nodes, we also follow the degree elimination order. However, we postpone the boundary contraction to the last phase because they are also part of the boundary tree and we can utilize them for faster query answering later on. \mycolor{The inner tree's time complexity is $O(|C||V_i| (max(|X_j|)\cdot n\cdot c^{2n-2}_{max}\log c_{max} (max(|X_j|)+ h_i)+\log |V_i|)$, where $|V_i|$ is the vertex set of subgraph $G_i$, $h_i$ is the inner tree height, and $X_j$ is the tree node belongs to $G_i$. As for the node number, tree width, tree height, and $c_{max}$ for most of the sub-graphs are much smaller, it is much faster than the original big tree. As the constructions are dependent, they can run in parallel to achieve higher performance. The total inner tree label size is $O(|C|\times |V_i|\cdot |h_i|\cdot c^{n-1}_{max})$.}  %Because of the boundary all-pair result, each partition tree can answer the inner partition query directly.

\subsection{Boundary Tree}
\label{subsec:Forest_Boundary}
When we have a query from different partitions, we need inter-partition information to help answer it. One way is precomputing the all-pair boundary results. However, unlike the previous one, this all-pair result is much larger and harder to compute because it contains boundaries of all the partition and they are far away from each other. To avoid the expensive long-range \textit{Sky-Dijk}, we also resort to the concatenation-based \textit{MCSP-2Hop} to build a boundary tree.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=2.9in]{BoundaryGraph.pdf}
    \caption{Forest Hop Labeling}
    \label{fig:Forest}
\end{figure}


The boundary tree is built on a graph that contains all the boundary edges and all the partition-boundary all-pair edges, as shown in Figure \ref{fig:Forest}-(a). Although we can still use the same degree elimination order to contract the vertices, its randomness ignores the property that these boundaries are the cuts of the partitions. As a result, the inner partition trees and the boundary tree has no relation and they can hardly interchange information. Therefore, we contract the boundaries in the unit of partition instead of degree: the boundaries from the same partition are contracted together in the same order of their inner tree. In this way, we can attach the inner partition trees to the boundary tree as shown in Figure \ref{fig:Forest}-(b). Furthermore, only the new shortcuts need skyline concatenation while the existing ones can be inherited directly.

In terms of label assignment, we can populate the labels only to the boundaries and we call it \textit{boundary label}. It has smaller index size but requires 6-hop in query answering. The boundary tree construction takes $O|B| (max(|X_j|)\cdot n\cdot c^{2n-2}_{max}\log c_{max} (max(|X_i|)+ h_B)+\log |B|)$ and its label size is $O(h_B\cdot |B|\cdot c^{n-1}_{max})$, where $B$ is the boundary set and $h_B$ is the boundary tree height. We can further push down the boundary labels to the inner labels and we call them \textit{extended labels}. Specifically, for each inner partition tree, its ancestors in the boundary tree are also added to its labels. For example in Figure \ref{fig:Forest}-(b), the green region have labels in every small tree, while the yellow region only appear in the yellow, red, and orange tree. The extended label assignment takes an extra $O(|C||V_i| (max(|X_j|\cdot c^{2n-2}_{max}\log c_{max} ( max(|X_j|)+h_i+h_B))+\log |V_i|))$ time and $O(h_B\cdot |V-B|\cdot c^{n-1}_{max})$ space.

\subsection{Query Processing}
\label{subsec:Forest_Query}
Depending on the locations of the two query points $s$ and $t$, we discuss the following situations:
\begin{enumerate}
	\item \textbf{$s$ and $t$ are in the same partition}: Because the all-pair boundary information is considered during construction, we can use the local partition tree directly to answer it.
	\item \textbf{$s$ and $t$ are all boundaries}: It can be answered with the boundary label directly.
	\item \textbf{$s$ is in one partition and $t$ is another's boundary}: If we only have the boundary label, then we need to first find the results from $s$ to its boundaries within the local label, then concatenate the results from these boundaries to $t$ using the boundary labels, and it takes 4 hops. If we have the extended labels, we can use it as a 2-hop label directly. 
	\item \textbf{$s$ and $t$ are in different partitions}: If we only have the boundary label, then we need to first find the results from $s$ to its boundaries within the local label, then concatenate the results from these boundaries to $t$'s boundaries using the boundary labels, and finally concatenate these results to $t$ with $t$'s local labels. Obviously, this is a 6-hop procedure. Similar to the previous case, if we have the extended labels, we can use it as a 2-hop label directly. More advanced query processing techniques will be presented in the next section.
\end{enumerate}






==> CSP-H2H (VLDBJ)/Introduction.tex <==
\section{Introduction}
\label{sec:Introduction}
Route planning is an important application in our daily life, and various path problems have been identified and studied in the past decades.
In the real-life route planning, there are always multiple criteria depending on users' preferences. For example, a user may have a limited budget to pay the toll charge of highways, bridges, tunnels, or congestion. Some mega-cities require drivers to reduce the number of big turns (e.g., left turns in the right driving case\footnote{\mycolor{https://www.foxnews.com/auto/new-york-city-to-google-reduce-the-number-of-left-turns-in-maps-navigation-directions}} 
as they have a higher chance to cause accidents). There could be other side-criteria such as the minimum height of tunnels, the maximum capacity of roads, the maximum gradient of slopes, the total elevation increase, the length of tourist drives, the number of transportation changes, etc.
However, most of the existing algorithms only optimize one objective rather than the other side-criteria, such as minimum distance \cite{dijkstra1959note,li2020fast}, travel time of driving \cite{li2019Time,li2020fastest} or public transportation \cite{wang2015efficient,wu2014path}, fuel consumption \cite{li2017minimal,li2018go}, battery usage \cite{adler2014online}, etc. In fact, it is these criteria and their combination that endow different routes with diversified meaning and satisfy users' flexible needs. In other words, this \textit{multi-criteria} route planning is in more generalized manner, while the traditional \textit{shortest path} is only a special case. Moreover, it is an important research problem in the fields of both transportation \cite{jozefowiez2008multi,shi2017multi} and communication (Quality-of Service constraint routing) \cite{korkmaz2001multi,de1998multiple,tsaggouris2009multiobjective,van2003complexity}.



%H In fact, we normally use a set of \textit{skyline} results \cite{papadias2003optimal} in a multi-objective problem like this. Therefore, one way to implement it is through \textit{skyline path} \cite{kriegel2010route,gong2019skyline,ouyang2018towards}, which extends the skyline concept to path finding.

However, we could hardly find one result that is optimal in every criterion when there are more than one optimization goals. One way to implement the multi-criteria route planning is through \textit{skyline path} \cite{kriegel2010route,gong2019skyline,ouyang2018towards}, which provides a set of paths that cannot dominate each other in all criteria. However, skyline paths computation is very time-consuming with time complexity $O(c^{n-1}_{max}\times|V|\times(|V|\log |V|+|E|))$, where $|V|$ is the vertex number, $|E|$ is the edge number, $c_{max}$ is the largest criteria value, and $n$ is the number of criteria \cite{hansen1980bicriterion} ($c^{n-1}_{max}$ is the worst case skyline number). In addition, it is impractical to provide users with a large set of potential paths to let them choose from. Therefore, the \textit{Multi-Constraint Shortest Path (MCSP)}, as another way to consider the multiple criteria, is widely applied and studied. Specifically, it finds the best path based on one objective while requires other criteria satisfying some predefined constraints. For example, suppose we have three objectives such as distance $d$ and costs $c_1, c_2$, and we set the maximum constraints $C_1$ and $C_2$ on the corresponding costs. Then this \textit{MCSP} problem finds the shortest path $p$ whose cost $c_1(p)$ is no larger than $C_1$ and $c_2(p)$ is no larger than $C_2$. %Although the number of possible criteria is unlimited, we focus on the single-criterion \textit{CSP} problem in this paper for the following reasons: (i) It is the basis of the multi-criteria \textit{CSP}; % and our algorithm can be easily extended to address the multi-constraint version; 
%(ii) Answering the single-criterion \textit{CSP} query is already a challenging task; (iii) Combining a large number of criteria may lead to no feasible path, which reduces the usability of the routing system.% Nevertheless, we present how to extend our approaches to the multi-criteria and other constraint conditions in Section \ref{sec:Extensions}.
%Combining several criteria may lead to no feasible solution, which reduces the usability of the system. Therefore, we focus on the single-constraint \textit{CSP} in this work, and multi-criteria \textit{CSP} can be extended easily with similar procedure.

%The solutions of path planning are one of the primary considerations in the transportation field. In the conventional path planning problems, we prefer to find the path with minimum distance, fastest travel time, or the lowest cost. A wide variety of solutions, such as Dijkstra's Algorithm, landmark-based algorithms, Hierarchy-based algorithms, and hop-based algorithms, can effectively deal with such shortest path problems. However, the path planning algorithms with only one optimization criteria will face challenges in real life, as we need to consider more factors in the complex transportation environment. For instance, a driver may want to find the path with the shortest distance but avoid all the toll roads or under a predefined budget, or cyclists prefer to a few longer road if they can bypass a hard climb $\cite{storandt2012route}$. Another case is about energy consumption. With the market expansion of battery electric vehicles, the limitation of battery capacities results in their drivers not only consider the fastest route but also consider the energy consumption that can not exceed the battery capacities$\cite{baum2017modeling}$. Furthermore, driving safety is also an important metric. For example, in 2015, New York City Council requested that Google Maps reduces the number of left turns in its suggested routes to avoid a high rate of pedestrian crashes$\cite{wang2016effective}$. All of them are identified as constraint shortest path (CSP) problems.

% The CSP answers the above problems by finding the best path based on a criterion, which is constrained by another criterion. However, this kind of problem has been confirmed as an NP-hard problem. It means that we may difficult to query CSP in large-scale networks by an efficient and exact solution. The majority of existing research would like to solve the problem by approximate or exact methods. %However, in several cases, we also keen to get an exact solution within large-scale networks. For instance, ambulances or police vehicles require the exact fastest route within given budgets. In this case, an approximate result may be not able to cope with an emergency. Therefore,%
% in this paper, We focus on CSP query with an exact solution. The reasons as follows: $(i)$ exact CSP solution is still needed in large size road network. For instance, ambulances or police vehicles require the exact fastest route within given budgets.$(ii)$ Even though answering CSP query with exact solution may be low efficiency, it is feasible to improve the query speed at the expense of increasing the index size. 
 
%The existing work on CSP can classified into four groups depending on the result is exact or approximate, and the method uses index or not.   b   
%The problems of the existing exact CSP algorithms. (index-free are slow, index-based are big and still not very fast...). The shortest path index can be classified into shortcut-based and labeled based. Their difference, like label based is faster in query answering

To the best of our knowledge, the existing \textit{MCSP} algorithms are mostly based on linear programming or graph search, and their high complexity prohibits them from scaling to the large networks \cite{jaffe1984algorithms,korkmaz2001multi,shi2017multi}. As a special and simpler case with only one constraint, the \textit{CSP} problem is the basis for solving the \textit{MCSP}, which can be classified into the following categories based on \textit{exact/approximate} and \textit{index-free/index-based} solutions. The \textit{exact CSP} result provides the ground-truth and satisfies the user's actual requirement \cite{hansen1980bicriterion,handler1980dual,LOZANO2013378,SEDENONODA2015602}, but it is extremely slow to compute as a NP-H problem \cite{garey1979computers,hassin1992approximation}. Therefore, the \textit{approximate CSP} algorithms \cite{hansen1980bicriterion,hassin1992approximation,juttner2001lagrange,lorenz2001simple,tsaggouris2009multiobjective} are proposed to reduce the computation time by sacrificing the optimality of the path length. However, their speedup compared with the exact solutions is very limited \cite{kuipers2006comparison,LOZANO2013378}. To further improve the query efficiency, a few \textit{indexes} \cite{storandt2012route,wang2016effective} have been proposed by extending the existing index structures of the shortest path problem. For example, \textit{CSP-CH} \cite{storandt2012route} extends the traditional \textit{CH} index \cite{geisberger2008contraction} to support exact \textit{CSP} query processing. 
Although the index construction time is usually long, which makes them inflexible when the weight or cost changes \cite{zhang2020stream,zhang2021DWPSL,zhang2021DH2H}, the index-based methods enjoy the high efficiency of query answering. Since \textit{2-hop labeling} \cite{cohen2003reachability,akiba2013fast,ouyang2018hierarchy} is the current state-of-the-art shortest path index, in this work, we aim to provide a 2-hop labeling-based index structure for exact \textit{MCSP} queries with both faster index construction and more efficient query processing.

%However, their construction time is long, which makes them inflexible when any weight or cost changes. Nevertheless, the index-based methods still enjoy the efficiency in query answering, and 2 hop labeling \cite{cohen2003reachability,akiba2013fast,ouyang2018hierarchy} is the state-of-the-art index for the shortest path finding, so we aim to provide 2-hop labeling-based index structure for \textit{CSP} query with faster construction time and faster query answering time.

%To the CSP algorithms, the existing algorithms mainly impose index-free or index-based techniques. Although they are feasible to answer the query in polynomial time, they still face challenges when they adapt to large-scale road networks. For instance, Label Setting $\cite{hansen1980bicriterion}$ is the classic solution in index-free CSP algorithms. It applies the idea of Dijkstra's algorithm to calculate the skyline paths which consider both weights of edges and corresponding costs. The algorithm stipulates that an arbitrary vertex $v$ can store all the $s-v$ paths, which are neither dominated by any path of its outgoing vertices nor over the constraint of cost. When the search terminates, we can get all the skyline paths of the query from its end vertex. Then, the algorithm extracts the best path from them. However, as the time complexity of this algorithm is not ideal, the performance is proved to be unsatisfactory in large-scale road networks. 

%On the other hand, index-based CSP algorithms use advanced pruning techniques to improve search efficiency. For instance, the algorithm combining skyline-Dijkstra and CH (CSP-CH) solves CPS with the experiment of the bicycle route planning$\cite{storandt2012route}$. In the pre-processing stage, the algorithm contracts vertices in terms of a predefined node ordering. As similar as CH algorithm, it adds shortcuts for each vertex but considers two criteria. In detail, given a vertex $v$, the paths between the neighbours of $v$ that are not dominated by other paths are considered as candidates. From the candidates paths, the algorithm then selects paths which are constrained by the maximum cost as shortcuts. In the reconstituted CH-graph, an optimal path can be found by a bi-directional search of Label Setting. Compared with index-free algorithms, CSP-CH can speed up the query time and reduce the search space. However, as its shortcuts store all the skyline paths, the index size can be much larger than the original CH. This problem will result in the low efficiency of a query in large-scale road networks. As CSP-CH is still a Dijkstra-based algorithm. If we have a query distance that is large enough, the algorithm will still visit a large number of vertices even it uses a hierarchical technique.



%Moreover, for each vertex, we also need to make decisions on the adjacent skyline paths. Several complex cases, such as complex road networks or dense graph, thus will impact the online searching. By the issues of existing work, we aim to provide a feasible method to construct index for reducing or avoiding Dijkstra-based searching and an appropriate hierarchy that works for large-scale road networks.  

%In the index-based shortest path algorithms, the shortest path index can be classified into shortcut-based and label-based. The state-of-the-art shortcut-based algorithms, such as CH, TNR, and arc-flags, have the breakneck speed to respond to local and mid-range queries. However, from empirical results on shortest path algorithms, most of the label-based algorithms are much faster than shortcut-based algorithms. The reason is that label-based algorithms commonly use lookup tables instead of graph searching to answer a query. Moreover, a theoretical analysis has also proved the advantage of label-based algorithms$\cite{abraham2010highway}$. Compared with shortcut-based algorithms, a label-based algorithm is able to provide the best time bounds. We can also find multiple theoretical settings on label-based algorithms$\cite{cohen2003reachability}\cite{gavoille2004distance}\cite{thorup2005approximate}$.

%Challenges to use the label-based. The most obvious one is how to use it because the existing ones can only support one criterion. When using the two criteria, the labels are not consistent: they are from two different paths and cannot be treated as the same one. The second one might be the index construction time because it is already slow in one criterion.

%Therefore, we focus on a label-based solution for index construction. However, we will face challenges if we adopt labels in the field of CSP. The most obvious one is how to use it because the existing work on label-based algorithms can only support one criterion (This part need to cite latter). When using the two criteria, the labels are not consistent: they are from two different paths and cannot be treated as the same one. Second, label-based methods commonly generate a mass of index on large-scale road networks. The construction time of label-based index is already slow in one criterion. If we consider one more criterion, the pre-processing may take longer. We also have mentioned that the CSP problem is NP-hard, even we impose index to control the query answering in a short time, the index construction may be still NP-hard. Thus, it is essential to design a structure that can organize and retrieve the labels efficiently. 

However, it is non-trivial to extend the 2-hop labeling to answer the \textit{MCSP} queries. Since it is already NP-H to find the optimal labels with size of $\varOmega(|V||E|^{1/2})$ for the single-criterion shortest path as proven in \cite{cohen2003reachability}, it would be much harder for the \textit{MCSP} problem due to the following reasons:

\begin{figure}[ht]
    \centering
    \includegraphics[width=3.2in]{Overview.pdf}
    \caption{Framework Overview}
    \label{fig:Overview}
\end{figure}

Firstly, since the constraints $C$ can be of any possible combination while are unknown beforehand, the skyline path information is inevitably needed in the index to be able to deal with any scenario. However, skyline path search is very time-consuming as discussed before, and hence the existing \textit{MCSP} solutions all suffer from low efficiency. Consequently, none of the existing indexes are constructed by the exact skyline path but resort to the approximate path search. The \textit{CSP-CH} \cite{storandt2012route} chooses to contract a limited number of vertices and adopts heuristic testing before each skyline path expansion, which leads to a subset of the skyline shortcuts with smaller index size but slower query time. %Furthermore, its index construction time increases dramatically (e.g., hours) compared with the conventional \textit{CH} index (e.g., minutes). 
\textit{COLA} \cite{wang2016effective} resorts to the graph partitioning and approximates skyline path search to reduce intermediate result size, but it sacrifices the query accuracy. %Moreover, its performance is still limited by the skyline path search when the approximate ratio is small and it has to build different indexes for different approximation ratios.
Therefore, skyline path search is the bottleneck of existing methods and hinders the development of a full exact index, without which a fast exact \textit{MCSP} query answering is impossible. In this work, we propose a \textit{skyline path concatenation} algorithm to completely avoid the expensive skyline path search and construct a 2-hop-labeling index that stores the complete skyline paths without compromising query accuracy or efficiency. %It is worth noting that the concatenation technique can also benefit other \textit{CSP} solutions, as discussed in Section \ref{sec:Extensions}.

Secondly, direct concatenation of two skyline paths does not necessarily generate a skyline path, and another $O(mn\log mn)$ time is needed to validate the skyline results, where $m$ and $n$ are the size of the two skyline path sets to be concatenated. To speed up this process, we provide several insights of the multi-dimensional skyline path concatenation, and propose an efficient concatenation method to incorporate the validation into the concatenation and meanwhile prune the concatenation space. Although the worst case complexity remains the same when all the concatenation results are all skylines, our algorithm is much more efficient in practice.

Thirdly, the skyline path computation can hardly scale to larger networks. As the path length increases in large networks, the number of skyline paths becomes larger. Consequently, both the index size and index construction time raise dramatically. To address the scalability issue, we propose the \textit{forest hop labeling} framework which partitions the networks into multiple regions and constructs the index parallelly both within and across the regions.  

%Secondly, the number of skyline paths becomes larger as the path grows, so it can hardly scale to larger networks. Therefore, we propose the \textit{forest hop labeling} framework that first partitions the graph into regions and then builds indexes within and across the regions in parallel. 

Last but not least, the final index is essentially for skyline path query since it contains all the skyline path information. Hence, it would take approximately $m\times n\times h$ times of skyline concatenations before answering the query, where $h$ is the number of hops. This is much larger than the traditional 2-hop-labeling index which only needs $h$ times of calculation. In other words, the query performance of the index deteriorates dramatically and loses the promise of its high efficiency. Therefore, we propose a $n$-\textit{Cube pruning} technique to prune the useless concatenation as early as possible. Furthermore, we propose a \textit{constraint-based pruning} technique for faster \textit{MCSP} query answering, and also provide pruning technique for the forest label construction. As shown in the experiments, our approach can answer the \textit{MCSP} query within 1 ms and the proposed pruning techniques can further reduce it by two orders of magnitude, while the existing methods are thousands of times slower. Our contributions are illustrated in Figure \ref{fig:Overview} and summarized below:

%efficient query answering method that takes the query constraint $C$ into consideration to prune label concatenation space and brings the query answering time back to $O(h)$. 
\begin{itemize}
    \item We first propose a skyline path concatenation-based \textit{MCSP-2Hop} method that avoids the expensive skyline path search to achieve efficient \textit{MCSP} query answering and index construction. Several concatenation insights are further presented to reduce the concatenation space and incorporate multi-dimensional skyline validation into concatenation.
    %The proposed concatenation technique can also be easily extended to benefit other existing \textit{CSP} solutions.
    \item We further propose a \textit{forest hop labeling} for scalability. We also design a $n$-Cube pruning technique to further speed up the multi-hop concatenation during index construction and query answering, and a constraint pruning method to speed up \textit{MCSP} specifically.
    %\item We propose a tree-decomposition based index construction method that uses our concatenation methods to build a \textit{CSP-2Hop} index efficiently.
    \item We thoroughly evaluate our method with extensive experiments on real-life road networks and the results show that it outperforms the state-of-the-art methods by several orders of magnitude. 
\end{itemize}

This paper extends the work \cite{Liu2021Forest} where we introduced the \textit{Forest Hop Labeling} for \textit{CSP} with only one constraint. Because path concatenation algorithm and pruning technique were only designed for one constraint, its multi-constraint version in \cite{Liu2021Forest} was only a straightforward and slow solution. Therefore, in this paper, we generalize the path concatenation methods into multi-cost scenario and extend the pruning techniques to multi-constraint scenario to achieve higher performance. Although they are the generalizations of the \textit{CSP}, the problem in the multi-dimensional space is much harder than the 2-dimensional one such that \textit{CSP} is only a very special case of \textit{MCSP} with unique properties. Therefore, we provide new insightful properties of the high dimensional skyline path concatenation and pruning to facilitate the more efficient index construction and query answering in \textit{MCSP}. 

In the reminder of this paper, we first define our problem formally and introduce the essential concepts in Section \ref{sec:Preliminary}. Section \ref{sec:MCSP2Hop} and \ref{sec:Forest} present our \textit{MCSP-2Hop} and \textit{forest hop labeling} with their index structures and query answering methods, and Section \ref{sec:Skyline} presents the speedup techniques. We report our experimental results in Section \ref{sec:Experiment}. Finally, Section \ref{sec:RelatedWork} discusses related works and Section \ref{sec:Conclusion} concludes the paper. %Section \ref{sec:Extensions} further discusses the extendability of our approaches to other \textit{CSP} scenarios and solutions. Finally, Section \ref{sec:Conclusion} concludes the paper.
 
%How we conquer the previous challanges.
%In terms of the challenges, our index is designed based on 2 hop labeling, which assigns labels for each vertex in $G$ and allows us to answer a query by retrieving labels on lookup table instead of searching on networks. Furthermore, we use tree decomposition to help us organize the labels. The space complexity of tree decomposition is $O(nh)$, where n is the number of vertices in the graph and h is the tree height of the generated tree decomposition. Usually, the tree height of a road network is small. For instance, based on the instance of the article, the New York road network with more than 260,000 vertices and 730,000 edges can be converted to a tree decomposition with treewidth of only 131 and tree height of only 320 (\cite{ouyang2018hierarchy}). Thus, the space complexity can fit cases in large-scale road networks. Moreover, this tree structure can help us to avoid the entire search on labels. We will discuss our label-based method in section 3.  (fix this part later) 


%We answer the CSP problem by finding a path between two nodes that minimizes the total cost under a restriction of maximum resource consumption. By the previous statement, the cost here can be the single criteria identified in the shortest path problem, such as distance. The resource consumption is a summation of the extra factors need. 

%As CSP is relevant in real-world applications, there is a variety of research on speed-up techniques to CSP problem. For instance, an exact CSP algorithm that can solve networks adequate to 40,000 nodes and 800,000 arcs in an amount of time under 0.3 s based on the technique of propagating pulses through a network (Lozano and Medaglia, 2013). The CSP problem with two criteria including solution time and computer memory requirements to solve test problems in the networks within 10,000 to 40,000 nodes and 15,000 to 800,000 arcs by KSP algorithms (Santos and Rodrigues, 2007). Both articles can effectively solve the CSP problem on networks, but the average computer time maintains at seconds level. In other words, these techniques will face challenges when we translate to rather large networks. Several studies on CSP can solve the problem on large networks (millions nodes and arcs), such as the Aggressive Edge Elimination procedure based on Lagrangian relaxation techniques require solving CSP on grid-like graphs (Muhandiramge and Boland, 2009). However, the research orientation is irrelevant to road networks. Besides, an exact CSP algorithm combining skyline-Dijkstra and CH (CSP-CH) solves CPS problems with the experiment of the bicycle route planning (Storandt, 2015). The results show that the average run time and search space can have significantly reduce compared with the previous studies. Nevertheless, this algorithm requires a vast index space because of the skyline paths.

%On the other hand, even we have multiple methods to solve CSP problems by either an exact way or an approximation guarantee. The majority of algorithms that used to solve road networks on CSP are Dijkstra-based speed-up techniques. For example, dynamic programming solutions can efficiently identify and omit paths which are useless either  to build a Pareto-optimal set of paths or to be extended into  Pareto-optimal paths (Desaulniers ). The label setting method imposes the idea of Dijkstra's algorithm to iteratively identify the shortest path that is not dominated other paths and constrained by a maximum resource consumption value (Aggarwal,Aneja, and Nair, 1982). Several further studies on CSP have focused on pruning techniques to eliminate abundant nodes and edges for shrinking search space then reduce run time. Such pruning methods depend on the auxiliary index, such as CSP-CH which we mentioned above.

%Given the previous studies, we can find several existing techniques to deal with CSP problem efficiently in road networks of certain scale. However, with road transport becoming complex,  the amount of road network data is increasing quickly. It is valuable to exist and develop for CSP algorithms that are more suited to rather large-scale road networks. Even though the state of art CSP algorithms can raise efficiency remarkably, they still have several limitations, such as lower computer time and a large amount of index space. 

%Therefore, to the CSP problem, we keen to find a solution that can further reduce the query time and downsize the index based on the query distance in large-scale road networks. Refer to the performance of algorithms in shortest path problems, Hierarchical 2-Hop Index (H2H-Index) combines hierarchical based solution and hop based solution by the strategy of tree decomposition (Ouyang, 2018). Compared with other advanced algorithms, the advantage is to provide short query time and smaller index. The space complexity of H2H-index for an undirected graph is O(n·h), where n is the number of vertices in the graph and h is the tree height of the generated tree decomposition. Usually, the tree height of a road network is small. For instance, based on the instance of the article, the New York road network with more than 260,000 vertices and 730,000 edges can be converted to a tree decomposition with treewidth of only 131 and tree height of only 320 (Ouyang, 2018). Thus, the space complexity can fit cases in large-scale road networks. 

%To the shortest path problem in a road network, the idea of H2H-index algorithm is to assign a label to each vertex and also design a hierarchy for all vertices . The hierarchy is generated by tree decomposition, and it can map the road network to a rooted tree structure. Each node in the tree can be a subset of vertices in the network. Thus, it will be a feasible way to speed up several computation problems [Robertson and Seymour]. We will describe the construction of tree decomposition in section 2.  In the query stage of H2H-index algorithm, given a query q(s, t), the tree structure can help it locate to a subset of vertices covering the shortest path distance of the query. Then, the algorithm conducts 2-hop search by exploiting the vertices in the labels of s and t within the boundary of the subset. Thus, this algorithm not only avoids to visit a large number of vertices when the query distances large enough but do not have to traverse the entire labels of s and t. 

%In our case, the CSP problems have two criteria, including distance and resource consumption. For a query q(s, t), when the lookups reach the hop, the path with minimum distance and the path with lowest resource consumption may be different. Hence, we have to use an alternative strategy to make the query of tree decomposition feasible in CSP. 

%Therefore, in this paper, we aim to impose the idea of tree decomposition in CSP problem and suppose that the technique can reduce query time and index space as similar to the performance in shortest path problems. We will describe in detail how the tree decomposition can be built to support query of CSP. Moreover, we will also conduct an experimental evaluation to identify the advantages of tree decomposition in CSP compared with CSP-CH, which is the baseline in the experiment.

%In our idea, given a tree decomposition T(G) of a graph G and query q(s, t), we suppose two ways to achieve the goal: First, we conduct pruning to delete the vertices on dominated paths in the labels of s and t. Thus, we need to ensure the query processing only find the paths which resource consumption less than its maximum value. Second, we immediately answer the query by T(G). By the tree structure, we can ensure all the paths from s to t can be identified by the labels of s and t. Thus, we can find a scope to identify a dominating path further. We will discuss both ways in detail in Section 3.


==> CSP-H2H (VLDBJ)/MultiSkyline.tex <==
\section{Multi-Dimensional Constrained Shortest Path}
%Reasons why we need to extend F2Hop
%Since the complexity of road networks and user demands on different constraints, a \textit{CSP} query with only one criterion will be in limited range of applications. In this section, we extend our hop labeling method to solve \textit{CSP} queries on the road networks with multiple criteria. 

%Based on the above findings, in the remaining subsections, we study the challenges of extending \textit{F2Hop} to multiple dimensions. Then, we discuss the Multi-dimensional skyline \textit{(Multi-skyline)} path concatenation with pruning techniques.
\subsection{Extension of F2Hop to Multiple Dimensions}
%#########################################
%definition here
%\begin{definition}[MCSP Query]
%\label{def:Dominance}
%Given a $n$-dimensional graph $\overline{G}(V,\overline{E})$, where $n>2$. Each edge $e \in \overline{E}$ contains a weight $w$ and a series of cost $c_i$, where $i \in [1,n-1]$. Given a $MCSP$ query $\overline{q}(s,t,\overline{C})$. $\overline{C}={C_1,...,C_{n-1}}$ is a set of maximum cost bounds. $\forall C_i\in \mathbb{R}^+$, $\overline{q}(s,t,\overline{C})$ returns a path $p$ with the minimum $w(p)$ while guaranteeing that each $c_i(p) \leq C_i$. 
%\end{definition}
%
%\begin{definition}[Multi-dimensional Path Dominance]
%	\label{def:Multi-Dominance}
%	Given two paths $p_1$ and $p_2$ with the same OD, $p_1$ dominates $p_2$ iff $w(p_1) \leq w(p_2)$ and $c_i(p_1) \leq c_i(p_2),\forall i\in[1,n-1]$, and at least one of them is the strictly smaller relation.
%\end{definition}
%
%\begin{definition}[Multi-Skyline Path]
%	\label{def:Multi-SkylinePath}
%	Given any two paths $p_1$ and $p_2$ with the same OD, they are skyline paths if they cannot dominate each other. 
%\end{definition}
%#########################################

%Challenges of extending F2Hop
As the road network structure dictates the hierarchical structure we built, with the increasing of criteria in a road network, the structure of its tree decomposition will be changeless. However, the skyline path validation will become complex....

Also, the number of skyline paths in each label will increase dramatically, especially, in large scale networks.....


%analysing complex of multi-path domination test
%\begin{theorem}
%	\label{the:2-n skyline}
%We treat two path $p_1$ and $p_2$ are the same, if $w(p_1)=w(p_2)$ and $c_i(p_1)=c_i(p_2),\forall i\in[1,n-1]$. Thereby, if a path $p$ is a skyline path in a two dimensional space, it must be a skyline path in n dimensions. 
%\end{theorem}
%\begin{proof}

%\end{proof}
%In terms of \ref{the:2-n skyline}, we can identify a Multi-skyline path, if it can not be dominated in a two-dimensional space. However,  

%analysing number of skyline paths



\subsection{Multi-Dimensional Constraint Skyline Path Concatenation}

Theorem \ref{theorem:GreedySkyline} efficiently reduces the complexity of skyline path validation in 2D road networks. This is because the cost of 2D skyline paths is natural ranking if we sort them with weight-increasing order. In algorithm \ref{Algorithm:GreedyConcatenation}, when a new path $p_i^j$ is concatenated, its weight must be not less than all the skyline paths in $P_s$. Thus, we only need to compare the cost of $p_i^j$ with the cost of the ranked last path in $P_s$, which has the minimum cost. However, this skyline validation method will be not feasible when each path has multiple costs, as we can not guarantee the ordering of costs for a weight-sorting Multi-skyline path set. For example, in Table \ref{table:EG_skylines} has five skyline paths within 4-dimensions. Each cost is out-of-order, even though we sort them by weigh-increasing order. To reduce the comparison number of skyline validation in paths with multiple costs, we provide the following theorem:


\begin{theorem}
\label{theorem:MultiGreedySkyline}
In $n$-dimensional graph, suppose the concatenated paths are coming in the weight-increasing order. We have $k$ skyline paths and a new path $p_{k+1}$ comes with weight larger than $w_k$. $\forall c_i \in \overline{C}$, $i\leq n$, we rank $k+1$ paths in cost-increasing order and obtain the rank of $p_{k+1}$, which is denoted as $r_i(k+1)$. $\exists o \in [1,n)$ such that $r_o(k+1)$ is minimum compared with arbitrary $r_i(k+1)$. The corresponding criterion $c_o$ is named as distinct criterion. Suppose $m$ concatenated skyline paths, $m \leq k$, have higher or equal ranking than $r_o(k+1)$ on $c_o$. If all the $m$ paths cannot dominate $p_{k+1}$, then $p_{k+1}$ must be a skyline path. 
\end{theorem} 

\begin{proof}
We divide the $k$ skyline paths into two set $S_1$ and $S_2$. $S_1$ contains the $m$ skyline paths that have higher or equal ranking than $p_{k+1}$ on dimension $c_o$. $S_2$ contains the remaining skyline paths.  Compared with all the paths in $S_2$, $p_{k+1}$ has largest value on dimension $c_o$ and highest value on dimension $w$. Thereby, $p_{k+1}$ is a skyline path in set $S_2$. As $p_{k+1}$ has larger weight than the $k$ skyline paths, $p_{k+1}$ can not dominated each path in $S_1$. According to definition \ref{def:Multi-SkylinePath}, if no one path in $S_1$ can dominate $p_{k+1}$, it must be a skyline paths in $S_1$. Due to $p_{k+1}$ is a skyline path in both $S_1$ and $S_2$, it is a skyline path in the current concatenated path set. Also, we have proved that $p_{k+1}$ cannot be dominated by latter coming paths in Theorem \ref{theorem:GreedySkyline}. $p_{k+1}$ thus must be a final skyline path.
\end{proof}

For example in Table \ref{table:EG_skylines}, we have a set of skyline paths ${p_1, p_2, p_3, p_4, p_5}$. On each dimension, we rank the paths with increasing order, which is shown in Figure \ref{fig:MultiSkylineValidation}. Suppose we have the next concatenated path $p_6={8, 5, 8, 9}$. As $p_6$ has greater weight than the five paths, it must be ranked last on dimension $w$. Then, we find the ranks of $p_6$ on other dimensions, which are highlighted by red color. The distinct criterion is $c_2$. We need to identify whether $p_6$ can be dominated by $p_3$ or $p_5$. As $p_6$ cannot be dominated, $p_6$ is a skyline path.

However, in Theorem \ref{theorem:MultiGreedySkyline}, if the next concatenated path $p_{k+1}$ has the same weight with $p_k$, we need to do skyline validation between $p_{k+1}$ and each path that has the same weight with it. If $p_{k+1}$ is dominated, we concatenate next path. If $p_{k+1}$ can dominate any paths having the same weight with it, we remove the dominated paths from the concatenated set. Afterwards, we use Theorem \ref{theorem:MultiGreedySkyline} to further do the skyline validation for $p_{k+1}$. For example, suppose we change $p_6$ to ${6,5,8,9}$. It has the same weight with $p_5$. We compare $p_5$ and $p_6$, as they can not dominate each other, we further check the highest rank of $p_6$ as the same as the previous discussion. 

The efficiency of the extending algorithm is depended on the number of the paths having higher or equal ranking than the new coming path $p_{k+1}$ on distinct criterion. If $p_{k+1}$ ranks too low on distinct criterion, we may compare a large amount of skyline paths in real cases, which is still time consuming. Thus, we provide a pruning technique for the algorithm. The theorem is shown as follows.

\begin{theorem}
\label{the: MultiGreedyPruning}
In $n$-dimensional graph, suppose the concatenated paths are coming in the weight-increasing order. We have $k$ skyline paths and a new path $p_{k+1}$ comes with weight larger than $w_k$. We rank $k+1$ paths as the same as Theorem \ref{theorem:MultiGreedySkyline}. Compute the number of paths that has lower ranking than $p_{k+1}$ on at least one criterion. If the number less than $k$, $p_{k+1}$ is not a skyline path.
\end{theorem}

\begin{proof}
 We proof it by contraction. Suppose $p_{k+1}$ is a skyline path and there are $k-1$ skyline paths having lower ranking than $p_{k+1}$ on at least one criterion. As $p_{k+1}$ has the larger weight than these $k$ paths. We only need to consider the rankings on the criteria of costs. Except $p_{k+1}$, $k$ paths are considered in the rankings. Thereby, it must has at least one skyline path $p_i$, $\forall i \leq k$, having higher or equal ranking than $p_{k+1}$ on all the criteria of costs. According to definition \ref{def:Multi-Dominance}, $p_i$ can dominate $p_{k+1}$. Since the assumption is false, Theorem \ref{the: MultiGreedyPruning} is true.
\end{proof}



\begin{table}[]
\centering
\caption{An example of skyline paths}
\label{table:EG_skylines}
\scriptsize
%\scalebox{1.1}{
\begin{tabular}{|l|l|l|l|l|}
\hline
$P_c$ & $w$ & $c_1$ & $c_2$ & $c_3$ \\ \hline
$p_1$ & 2   & 4     & 10    & 2     \\ \hline
$p_2$ & 2   & 4     & 9     & 3     \\ \hline
$p_3$ & 3   & 7     & 7     & 10    \\ \hline
$p_4$ & 5   & 3     & 9     & 3     \\ \hline
$p_5$ & 6   & 6     & 8     & 4     \\ \hline
\end{tabular}
%}
\end{table}

\begin{figure}[ht]
    \centering
    \includegraphics[scale=0.25]{MultiGreedy.jpg}
    \caption{Next Skyline Path Validation in Multi-dimensions}
    \label{fig:MultiSkylineValidation}
\end{figure}
%rectangle 
%How to concatenate skylines in multi-dimensions. 
%Why it is efficient.
%\subsection{Pruning on Multi-Dimensional Skyline Path Concatenation}
%How to extend rectangle-base pruning
%running example


==> CSP-H2H (VLDBJ)/Preliminary.tex <==
\section{Preliminary}
\label{sec:Preliminary}

\subsection{Problem Definition}
\label{subsec:Preliminary_PD}
%As discussed above, we focus our discussions on directed weighted large-scale road network. 
A road network is a graph $G(V, E)$, where $V$ is a set of vertices representing intersections and $E\subseteq V\times V$ is a set of edges representing road segments. Each edge $e \in E$ has two criteria: weight $w(e)$ and cost $c(e)$.  A path $p$ from the source $s \in V$ to the target $t \in V$ is a sequence of consecutive vertices $p$=$\left<s=v_0,v_1,\dots,v_k=t\right>$=$\mycolor{\left<e_0,e_1,\dots,e_{k-1}\right>}$, where \mycolor{$e_i$=}$(v_i,v_{i+1})\in E, \forall i\in[0,k-1]$. Each path $p$ has a weight $w(p)$=$\sum_{e \in p}w(e)$ and a cost $c(p)$=$\sum_{e \in p}c(e)$. We assume the graph unweighted while it is easy to extend our techniques to the directed ones. Then we define the \textit{CSP	} query below:

\begin{definition}[CSP Query]
\label{def:CSP}
Given a graph $G$, a source $s$, a destination $t$, and a maximum cost bound $C\in \mathbb{R}^+$, a \textit{CSP} query $q(s,t,C)$ returns a path with the minimum $w(p)$ while guaranteeing that $c(p) \leq C$. 
\end{definition}

As analyzed in Section \ref{sec:Introduction}, it is quite slow to answer a \textit{CSP} query by online search. Therefore, in this paper, we resort to index-based method and study the following problem: 
\begin{definition}[Index-based CSP Query Processing]
\label{def:PD}
%Given a static undirected weighted graph $G(V, E)$, construct a hop-based index $L$ that given any \textit{CSP} query $q(s,t,c)$, it could answer $q$ efficiently only with $L$.
Given a graph $G$, we aim to construct a hop-based index $L$ that can efficiently answer any \textit{CSP} query $q(s,t,C)$ only with $L$, \mycolor{which stored in a lookup table and can avoid the online searching in road networks.}
\end{definition} 

Unlike the index for the shortest path queries which only needs to store the shortest distance from one vertex to another, the \textit{CSP} index needs to cover all the possible constraints $C$. In addition, we observe that the \textit{CSP} paths are essentially a subset of the \textit{Skyline} paths, which is introduced as follows.
% Therefore, we first introduce the skyline path as follows.

%There are three essential concepts in solving CSP, which are dominance relationship, skyline, and 2 hop labeling. 

\subsection{Skyline Path}
\label{subsec:Preliminary_Skyline}
Like the \textit{dominance} relation of the skyline query in the 2D space \cite{papadias2003optimal}, we first define the \textit{dominance} relation between any two paths with the same source and destination:
\begin{definition}[Path Dominance]
\label{def:dominance}
Given two paths $p_1$ and $p_2$ with the same $s$ and $t$, $p_1$ dominates $p_2$ iff $w(p_1) < w(p_2)$ and $c(p_1) \leq c(p_2)$, or $w(p_1) \leq w(p_2)$ and $c(p_1) < c(p_2)$. 
\end{definition}

\begin{figure}[ht]
    \centering
    \includegraphics[scale=0.22]{example_road_network.pdf}
    \caption{An example of Skyline Path. Edge labels are $(w(e), c(e))$.}
    \label{fig:ExampleGraph}
\end{figure}

%For example in Figure \ref{fig:ExampleGraph}, $p_1$=$\left<v_5, v_4, v_9\right>$ has $w(p_1)=4$ and $c(p_1)=3$, while $p_2$=$\left<v_5, v_8, v_9\right>$ has $w(p_2)=4$ and $c(p_2)=5$. Since $w(p_1)=w(p_2)$ while $c(p_1)<c(p_2)$, $p_1$ dominates $p_2$.

\begin{definition}[Skyline Path]
Given any two paths $p_1$ and $p_2$ with the same $s$ and $t$, $p_1$ and $p_2$ are skyline paths if they cannot dominate each other. %namely they satisfy either of the following two conditions: $(i)$ $w(p_1) \leq w(p_2)$ and $c(p_1) \geq c(p_2)$; or $(ii)$ $w(p_1) \geq w(p_2)$ and $c(p_1) \leq c(p_2)$. 
\end{definition}

In this paper, \mycolor{we use $P(s,t)$ to denote the set of skyline paths from $s$ to $t$. we denote a path $p$ as a skyline path $\overline{p}$ if it is in a skyline path set}. Consider the example in Figure \ref{fig:ExampleGraph}. We enumerate four paths from $v_5$ to $v_9$:
\begin{enumerate}
    \item $p_1 = \left<v_5, v_4, v_9\right>$, $w(p_1)=4$, $c(p_1)=3$
    \item $p_2 = \left<v_5, v_8, v_9\right>$, $w(p_2)=4$, $c(p_2)=5$
    \item $p_3 = \left<v_5, v_4, v_8, v_9\right>$, $w(p_3)=3$, $c(p_3)=6$
    \item $p_4 = \left<v_5, v_8, v_4, v_9\right>$, $w(p_3)=7$, $c(p_3)=6$
\end{enumerate}
According to the definition, we can identify that $p_2$ is dominated by $p_1$, and $p_4$ is dominated by the other three paths. Hence, $p_2$ and $p_4$ are not skyline paths. Meanwhile, as $p_1$ and $p_3$ cannot dominate each other, we obtain two skyline paths from $v_5$ to $v_9$: $P(v_5,v_9)=\mycolor{\{\overline{p}_1,\overline{p}_3\}}$. Next we prove that skyline paths are essential for building any \textit{CSP} index:

\begin{theorem}
\label{the:Skyline}
The skyline paths between any two vertices are complete and minimal for all the possible \textit{CSP} queries.
\end{theorem}
\begin{proof}
We first prove the completeness. Suppose the skyline paths from $s$ to $t$ are \mycolor{$\{\overline{p}_1$, $\dots$, $\overline{p}_k\}$} and they are sorted in the cost-increasing order. Therefore, the cost space is divided into $k+1$ intervals: \mycolor{$[0,c(\overline{p}_1)),[c(\overline{p}_1),c(\overline{p}_2)),\dots, [c(\overline{p}_k),\infty)$}. Then $\forall C\in \mathbb{R}^+$, we can find an $i$ such that $\mycolor{c(\overline{p}_i)}\leq C$ and $\mycolor{c(\overline{p}_{i+1})}> C$. Then it is guaranteed that $\mycolor{\overline{p}_i}$ is a \textit{CSP} result because all the paths with costs smaller than $\mycolor{c(\overline{p}_i)}$ have larger weights than $\mycolor{w(\overline{p}_i)}$, and all the paths with weights smaller than $\mycolor{w(\overline{p}_i)}$ have larger costs than the constraint $C$. When $C<\mycolor{c(\overline{p}_1)}$, no path between $s$ and $t$ satisfies the constraint; when $C>\mycolor{c(\overline{p}_k)}$, $\mycolor{\overline{p}_k}$ is the \textit{CSP} result.

Next we prove this skyline path set is minimal. Suppose we remove any skyline path $\overline{p}_i$ from the skyline result set. Then for \textit{CSP} queries whose constraint is within the range $[c(\overline{p}_i),c(\overline{p}_{i+1})]$, its result would be $\overline{p}_{i-1}$. However, the correct result should be $\overline{p}_i$ as analyzed above. Hence, no skyline path can be removed and the set is minimal.
\end{proof}

In summary, building an index for \textit{CSP} query is equivalent to building the index for skyline path query.
%Hence, building an index for skyline path query is equivalent to the \textit{CSP} query.

\subsection{2-Hop Labeling}
\label{subsec:Preliminary_2Hop}
\textit{2-hop labeling} is an index method that does not involve any search during query answering. It answers the shortest distance query by table lookup and addition. Specifically, $\forall u \in V$, we assign a label set $L(u)={\{v,w(v,u)\}}$ to store the minimum weights between a set of \textit{hop vertices} $v$ to $u$. To answer a query $q(s,t)$, we first determine the intermediate hop set $H=L(s) \cap L(t)$. Then we can find the minimum weight via the hop set: $min_{h \in H}{\{w(s,h)+w(h,t)\}}$. In this work, we extend the 2-hop labeling to support \textit{CSP} path because it can avoid any search during query processing.



==> CSP-H2H (VLDBJ)/PreliminaryNew.tex <==
\section{Preliminary}
\label{sec:Preliminary}

\subsection{Problem Definition}
\label{subsec:Preliminary_PD}
%As discussed above, we focus our discussions on directed weighted large-scale road network. 
A road network is a $n$-dimensional graph $G(V, E)$, where $V$ is a set of vertices and $E\subseteq V\times V$ is a set of edges. Each edge $e \in E$ has $n$ criteria falling into two categories: weight $w(e)$ and a set of costs $\{c_i(e)\}$, $i\in[1,n-1]$. A path $p$ from the source $s \in V$ to the target $t \in V$ is a sequence of consecutive vertices $p=\left<s=v_0,v_1,\dots,v_k=t\right>$ = $\mycolor{\left<e_0,e_1,\dots,e_{k-1}\right>}$, where $e_i$= $(v_i,v_{i+1})\in E, \forall i\in[0,k-1]$. Each path $p$ has a weight $w(p)$=$\sum_{e \in p}w(e)$ and a set of costs $\{c_i(p)$= $\sum_{e \in p}c_i(e)\}$. We assume the graph is undirected while it is easy to extend our techniques to the directed one. Then we define the \textit{MCSP} query below:

\begin{definition}[MCSP Query]
\label{def:MCSP}
%Given a $n$-dimensional graph $\overline{G}(V,\overline{E})$, where $n>2$. Each edge $e \in \overline{E}$ contains a weight $w$ and a series of cost $c_i$, where $i \in [1,n-1]$.
Given a $n$-dimensional graph $G(V, E)$, a $MCSP$ query $q(s,t,\overline{C})$ returns a path with the minimum $w(p)$ while each $c_i(p) \leq C_i\in \overline{C}$. 
\end{definition}

As analyzed in Section \ref{sec:Introduction}, it is quite slow to answer a \textit{MCSP} query by online graph search. Therefore, in this paper, we resort to index-based method and study the following problem: 

\begin{definition}[Index-based MCSP Query Processing]
\label{def:PD}
%Given a static undirected weighted graph $G(V, E)$, construct a hop-based index $L$ that given any \textit{CSP} query $q(s,t,c)$, it could answer $q$ efficiently only with $L$.
Given a graph $G$, we aim to construct a hop-based index $L$ that can efficiently answer any \textit{MCSP} query $q(s,t,\overline{C})$ only with $L$, \mycolor{which is stored in a lookup table and can avoid the online searching in road networks.}
\end{definition} 

Unlike the index for the shortest path queries which only needs to store the shortest distance from one vertex to another, the \textit{MCSP} index needs to cover all the possible constraints of each criteria $C_i$. In addition, we observe that the \textit{MCSP} paths are essentially a subset of the \textit{multi-dimensional skyline} paths, which is introduced as follows.



%\begin{definition}[CSP Query]
%\label{def:CSP}
%Given a graph $G$, a source $s$, a destination $t$, and a maximum cost bound $C\in \mathbb{R}^+$, a \textit{CSP} query $q(s,t,C)$ returns a path with the minimum $w(p)$ while guaranteeing that $c(p) \leq C$. 
%\end{definition}


% Therefore, we first introduce the skyline path as follows.

%There are three essential concepts in solving CSP, which are dominance relationship, skyline, and 2 hop labeling. 

\subsection{Multi-Dimensional Skyline Path}
\label{subsec:Preliminary_Skyline}
Like the \textit{dominance} relation of the skyline query in the 2-dimensional space \cite{papadias2003optimal}, we first define the \textit{dominance} relation between any two paths with the same source and destination:

\begin{definition}[Multi-Dimensional Path Dominan -ce]
	\label{def:Multi-Dominance}
	Given two paths $p_1$ and $p_2$ with the same $s$ and $t$, $p_1$ dominates $p_2$ iff $w(p_1) \leq w(p_2)$ and $c_i(p_1) \leq c_i(p_2),\forall i\in[1,n-1]$, and at least one of them is the strictly smaller relation.
\end{definition}



%\begin{definition}[Path Dominance]
%\label{def:dominance}
%Given two paths $p_1$ and $p_2$ with the same $s$ and $t$, $p_1$ dominates $p_2$ iff $w(p_1) < w(p_2)$ and $c(p_1) \leq c(p_2)$, or $w(p_1) \leq w(p_2)$ and $c(p_1) < c(p_2)$. 
%\end{definition}
\begin{figure}[ht]
    \centering
    \includegraphics[scale=0.3]{example_road_network.pdf}
    \caption{An Example of Skyline Path in 2D Graph. Edge Labels are $(w(e), c_1(e))$.}
    \label{fig:ExampleGraph}
\end{figure}

%For example in Figure \ref{fig:ExampleGraph}, $p_1$=$\left<v_5, v_4, v_9\right>$ has $w(p_1)=4$ and $c(p_1)=3$, while $p_2$=$\left<v_5, v_8, v_9\right>$ has $w(p_2)=4$ and $c(p_2)=5$. Since $w(p_1)=w(p_2)$ while $c(p_1)<c(p_2)$, $p_1$ dominates $p_2$.

\begin{definition}[Multi-Dimensional Skyline Path]
	\label{def:Multi-SkylinePath}
	Given two paths $p_1$ and $p_2$ with the same $s$ and $t$, they are skyline paths if they cannot dominate each other. 
\end{definition}

%\begin{definition}[Skyline Path]
%Given any two paths $p_1$ and $p_2$ with the same $s$ and $t$, $p_1$ and $p_2$ are skyline paths if they cannot dominate each other. %namely they satisfy either of the following two conditions: $(i)$ $w(p_1) \leq w(p_2)$ and $c(p_1) \geq c(p_2)$; or $(ii)$ $w(p_1) \geq w(p_2)$ and $c(p_1) \leq c(p_2)$. 
%\end{definition}

In this paper, \mycolor{we use $P(s,t)$ to denote the set of skyline paths from $s$ to $t$. We denote a path $p$ as a skyline path $\overline{p}$ if it is in a skyline path set}. Consider the 2-dimensional example in Figure \ref{fig:ExampleGraph}, we enumerate four paths from $v_5$ to $v_9$:
\begin{enumerate}
    \item $p_1 = \left<v_5, v_4, v_9\right>$, $w(p_1)=4$, $c_1(p_1)=3$
    \item $p_2 = \left<v_5, v_8, v_9\right>$, $w(p_2)=4$, $c_1(p_2)=5$
    \item $p_3 = \left<v_5, v_4, v_8, v_9\right>$, $w(p_3)=3$, $c_1(p_3)=6$
    \item $p_4 = \left<v_5, v_8, v_4, v_9\right>$, $w(p_3)=7$, $c_1(p_3)=6$
\end{enumerate}
According to the definition, we can identify that $p_2$ is dominated by $p_1$, and $p_4$ is dominated by the other three paths. Hence, $p_2$ and $p_4$ are not skyline paths. Meanwhile, as $p_1$ and $p_3$ cannot dominate each other, we obtain two skyline paths from $v_5$ to $v_9$: $P(v_5,v_9)=\mycolor{\{\overline{p}_1,\overline{p}_3\}}$. Next we prove that skyline paths are essential for building any \textit{MCSP} index:

\begin{theorem}
\label{the:Skyline}
The skyline paths between any two vertices are complete and minimal for all the possible \textit{MCSP} queries.
\end{theorem}
\begin{proof}
We first prove the completeness. Suppose the skyline paths from $s$ to $t$ are $\{\overline{p}_1$, $\dots$, $\overline{p}_k\}$, then each cost dimension  $c_i$ can be divided into $k+1$ intervals: $[0,c_i^1),[c_i^1,$ $c_i^2),\dots, [c_i^k,\infty)$, where each $c_i^j$ is the $j^{th}$ cost value of criterion $c_i$ sorted increasingly, and the entire space can be decomposed into $(k+1)^{(n-1)}$ subspaces. Then for the subspaces with any interval falling into $[0,c_i^1)$, there is no valid path satisfying all the constraints at the same time. For the subspaces with no interval falling into $[0,c_i^1)$, there is always at least one path dominating all the constraints in it, and the one with the smallest distance is the result.

Next we prove this skyline path set is minimal. Suppose we remove any skyline path $\overline{p}_j=\{c_i^j\}$ from the skyline result set. Then the \textit{MCSP} query whose constraint is within the subspace of $[c_1^{j}, c_1^{j+1})\times [c_2^{j}, c_2^{j+1})\times \dots \times [c_k^{j}, c_k^{j+1})$ will have no valid path. Hence, $\overline{p}_j$ cannot be removed and the skyline path set is minimal for all the \textit{MCSP} queries between $s$ and $t$.
\end{proof}

In summary, building an index for \textit{MCSP} query is equivalent to building the index for multi-dimensional skyline path query.
%Hence, building an index for skyline path query is equivalent to the \textit{CSP} query.

\subsection{2-Hop Labeling}
\label{subsec:Preliminary_2Hop}
\textit{2-hop labeling} is an index method that does not involve any graph search during query answering. It answers the shortest distance query by table lookup and summation. Specifically, $\forall u \in V$, we assign a label set $L(u)={\{v,w(v,u)\}}$ to store the minimum weights between a set of \textit{hop vertices} $v$ to $u$. To answer a query $q(s,t)$, we first determine the intermediate hop set $H=L(s) \cap L(t)$. Then we can find the minimum weight via the hop set: $min_{h \in H}{\{w(s,h)+w(h,t)\}}$. %In this work, we extend the 2-hop labeling to support \textit{CSP} path because it can avoid any search during query processing.
In this work, we select \textit{H2H} \cite{ouyang2018hierarchy}, the state-of-the-art 2-hop labeling, to support \textit{MCSP} query since it can avoid graph traversal in both index construction and query processing. Specifically, \textit{Tree Decomposition} \cite{robertson1986graph} is the cornerstone of \textit{H2H}, which maps a graph into a tree structure. We introduce it briefly as follows.

\begin{definition}[Tree Decomposition]
	\label{def:TreeDecomposition}
	Given a graph $G$, its tree decomposition $T$ is a rooted tree in which each node $X\in V$ is a subset of $V$. $T$ has the following tree properties:
	\begin{enumerate}
		\item $\bigcup_{X_i\in V}X_i=V$;
		\item $\forall (u, v)\in E, \exists X_i$ such that $\{u, v\}\subseteq X_i$;
		\item $\forall v\in V$, the set $\{X|v\in X\}$ forms a subtree of $T$.
	\end{enumerate}
\end{definition}

\begin{figure}[htbp]
	\centering
	\includegraphics[width=2.6in]{Tree.pdf}
	\caption{Tree Decomposition Example}
	\label{fig:Tree Decomposition}
\end{figure}

For instance, Figure \ref{fig:Tree Decomposition} shows the tree decomposition of the example graph in Figure \ref{fig:ExampleGraph}. The first vertex in each tree node is its representative vertex. %Depending on if the tree nodes have an ancestor/descendent relation not, 
This structure has a \textit{Cut Property} that can be used to assign labels: $\forall s,t\in V$ and $X_s,X_t$ are their corresponding tree nodes without an ancestor/descendent relation, their cuts are in their \textit{lowest common ancestor (LCA)} node \cite{chang2012exact}, \mycolor{which is the lowest tree node that has both $X_s$ and $X_t$}. For example, the tree nodes of $v_2$ and $v_7$ are $X_2$ and $X_7$, and their \textit{LCA} is $X_{1}=\{v_{1},v_5,v_8,v_{12}\}$. Then these four vertices form a cut between $v_2$ and $v_7$. If $s$ is $t$'s descendant, then $t$ can be viewed as a cut between itself and $s$. Therefore, the \textit{LCA} of a vertex pair contains all the cuts between them. 
%2) \textit{Ancestor Property}: $\forall X_v\in T_G, X_u(u\in X_v\{v\})$ is an ancestor of $X_v$ in $T_G$. This can also be easily checked in Figure \ref{fig:Tree Decomposition}. The ancestor property 
Accordingly, we assign labels to a vertex with all its ancestors in $T_G$. It should be noted that the vertices in each tree node are also in its label because of the \textit{Ancestor Property}: $\forall X_v\in T_G, X_u(u\in X_v\backslash\{v\})$ is an ancestor of $X_v$ in $T_G$. For example, $v_6$ has labels of $\{v_7,v_1,v_5,v_8,v_{12}\}\supseteq \{v_1,v_5,v_7\}$.





==> CSP-H2H (VLDBJ)/RelatedWork.tex <==
\section{Related Work}
\label{sec:RelatedWork}

\subsection{Shortest Path and Skyline Path}
\label{subsec:RelatedWork_SkylinePath}
\textit{Dijkstra}'s \cite{dijkstra1959note} is the fundamental shortest path algorithm that uses the best-first strategy to find the shortest paths from source to all the other vertices in the distance-increasing order. \textit{Sky-Dijk}\footnote{It was called \textit{MinSum-MinSum} problem as \textit{skyline} was not used in 1980s.} \cite{hansen1980bicriterion} is the first algorithm for skyline path query that expands the search space incrementally like the \textit{Dijkstra}'s but each vertex might be visited multiple times with one for each skyline result. Dominance relation can be applied to prune the search space. \cite{kriegel2010route} further incorporates \textit{landmark} \cite{kriegel2007proximity} to estimate the lower bounds, and prunes the search space with dominance relations. \cite{gong2019skyline} utilizes the skyline operator to find a set of skyline destinations.% instead of paths. 

\subsection{Constrained Shortest Path}
\label{subsec:RelatedWork_CSP}
As the single constraint shortest path \textit{CSP} is the basis of \textit{MCSP}, we discuss the four kinds of \textit{CSP} algorithms depending on the \textit{exact/approximate} and \textit{index-free/index} classification.

%\subsubsection*{Exact Index-Free CSP}
\paragraph{\textbf{Exact Index-Free CSP}.}
\cite{joksch1966shortest} is the first work studies \textit{CSP} and solves it with dynamic programming. \cite{handler1980dual} converts it to an \textit{integer linear programming (ILP)} problem and solves it with a standard \textit{ILP} solution. However, both of them are not scalable to large real-life road networks. Among the practical solutions, the \textit{Skyline Dijkstra} algorithm can be utilized to answer \textit{CSP} queries by setting a constraint on the cost during the skyline search. %In this way, the search space is further pruned as the CSP result is a subset of the skyline paths. 
Another practical solution to answer \textit{CSP} is through \textit{k-Path} \cite{yen1971finding}, which tests the top-$k$ paths one by one until satisfying $C$. \textit{Pulse} \cite{LOZANO2013378} improves this procedure by applying constraint pruning, but its \textit{DFS} search strategy limits its performance. \textit{cKSP} \cite{gao2010fast} uses the pruned \textit{Dijkstra} search in its $k$-path generation and incorporates the skyline dominance relation to prune the infeasible ones. \textit{eKSP} \cite{SEDENONODA2015602} further replaces \textit{cKSP}'s search with sub-path concatenation to speed up $k$-path generation. 

%\subsubsection*{Approximate Index-Free CSP}
\paragraph{\textbf{Approximate Index-Free CSP}.}
The approximation allows the result length being not longer than $(1+\alpha)$ times of the optimal path. The first approximate solution is also proposed by \cite{hansen1980bicriterion} with a complexity of $O(|E|^2$\mbox{\scriptsize $\dfrac{|V|^2}{\alpha-1}$} $\log$ \mbox{\scriptsize $\dfrac{|V|}{\alpha-1}$}), and \cite{lorenz2001simple} improves it to $O(|V||E|$ $(\log\log$\mbox{\scriptsize $\dfrac{w_{max}}{w_{min}}+\dfrac{1}{\alpha-1}))$}. \textit{Lagrange Relaxation} is applied by \cite{handler1980dual,juttner2001lagrange,carlyle2008lagrangian} to obtain the approximation result with $O(|E|\log^3|E|)$ iterations of path finding. As shown in \cite{kuipers2006comparison} and \cite{LOZANO2013378}, these approximate algorithms are even orders of magnitude slower than the \textit{k-Path}-based exact algorithms. \textit{CP-CSP} \cite{tsaggouris2009multiobjective} approximates the \textit{Skyline Dijkstra} by distributing the approximation power $\sqrt[n]{\alpha}$ to the edges. However, this approximation ratio would decrease to nearly 1 when the graph is big, so its performance is only slightly better than \textit{Sky-Dijk}.

%\subsubsection*{Exact Index-Based CSP}
\paragraph{\textbf{Exact Index-Based CSP}.}
There are many shortest path indexes, but only \textit{CH} \cite{geisberger2008contraction} has been extended to \textit{CSP} \cite{storandt2012route}, %Because the query constraint can be arbitrary, the \textit{CSP} index has to capture all the possible solutions. Hence, 
with its shortcuts being \textit{skyline paths}. Consequently, its construction and query answering are both \textit{Sky-Dijk}-based and suffers from long index construction, large index size, and slow query answering. Hence, \textit{CSP-CH} only keeps a limited number of skyline paths in each shortcut to reduce the construction time, but its query performance suffers.

%\subsubsection*{Approximate Index-Based CSP}
\paragraph{\textbf{Approximate Index-Based CSP}.}
The only approximate index method is \textit{COLA} \cite{wang2016effective}, which partitions the graph into regions and precomputes approximate skyline paths between regions. Similar to \textit{CP-CSP}, the approximate paths are also computed in the \textit{Sky-Dijk} fashion. In order to avoid the diminishing approximation power $\sqrt[n]{|V|}$, it views $\alpha$ as a budget and concentrates it on the important vertices. Similar pruning technique is also applied in the time-dependent path finding \cite{li2019Time}. In this way, the approximation power is released so it has faster construction time and smaller index size.

\subsection{Multi-Constraint Shortest Path}
Most of the existing \textit{MCSP} algorithms have very high complexity and cannot scale to real-life networks. For instance, \cite{jaffe1984algorithms} has a very high complexity of $O(|V|^5c_{max}$ $\log(|V|c_{max}))$. \cite{korkmaz2001multi} applies a heuristic-based approximation algorithm with no approximation bound, a backward \textit{Dijkstra}'s for feasibility check and a forward \textit{Dijkstra}'s to connect the results. However, it can only scale to small graph with 200 vertices. \cite{shi2017multi} takes seconds on the graphs with only 100 vertices. \cite{kriegel2010route,yang2021efficient} restricts the skyline path to the pre-defined ``preference function", so they cannot be utilized to answer \textit{MCSP} problem. \cite{DBLP:conf/adc/ZhangLZL21} compares and conducts experiments on the skyline-based and $k$-shortest path-based methods. 

\subsection{2-Hop Labeling}
\label{subsec:RelatedWork_2Hop}
The 2-hop labeling index \cite{cohen2003reachability} answers distance query without any search. \textit{PLL} \cite{akiba2013fast,zhang2021DWPSL} and \textit{PSL} \cite{li2019scaling} are designed for \textit{small-world} networks since several large degree vertices work as gateways to help reduce the search. \textit{Tree-Decomposition}-based methods \textit{H2H} \cite{ouyang2018hierarchy} and \textit{TEDI} \cite{wei2012tedi} are suitable for road networks because of the low average degree and the small tree width. \textit{CT-Index} \cite{li2020scaling} combines \textit{H2H} and \textit{PLL} to deal with the periphery and core of a graph separately.




==> CSP-H2H (VLDBJ)/Skyline.tex <==
\section{Skyline Path Concatenation}
\label{sec:Skyline}
In this section, we present insights of the skyline path concatenation that speedup the index construction and query processing. Specifically, we first discuss how to concatenate two skyline path sets via single hop in Section \ref{subsec:Skyline_Full}, which is used in the \textit{tree node contraction} phase of index construction. Then we extend to multiple hops in \ref{subsec:Skyline_Multiple}, which is used in the \textit{label assignment} phase of index construction and query processing. Finally, we explain how to efficiently answer \textit{MCSP} in Section \ref{subsec:Skyline_Constraint} and how to apply these techniques to \textit{forest labels} in Section \ref{subsec:Skyline_Forest}.
\begin{figure}[ht]
    \centering
    \includegraphics[width=3.4in]{ConcatenationDominance2.eps}
    \caption{Concatenated Path Category}
    \label{fig:ConcatenationCategory}
\end{figure}
%in the first step of the index construction phase, all the skyline results via a single hop should be preserved in the labels as required by Theorem \ref{the:HopSkyline}, so we regard it as the \textit{full concatenation} as discuss in Section \ref{subsec:Skyline_Full}; In the second label assignment phase and skyline query answering, we deal with results from multiple hops and discuss the pruning strategy in Section \ref{subsec:Skyline_Multiple}. Finally, we present the concatenation used in the \textit{CSP} query answering in Section \ref{subsec:Skyline_Constraint}.
 %To facilitate the further analysis, we use the following lemma to categorize the resulting paths:

%In Figure \ref{fig:ExampleGraph}, to find the CSP from A to E, we can check the $L_{out}(A)$ and $L_{in}(E)$. If we are at the intermediate hop D, as the path $<A, B, D>$ is the skyline path in $L_{out}(A)$ and the path $<D, E>$ is the skyline path in $L_{in}(E)$, we can calculate path $<A, B, D, E>$ with weight 7 and cost 7. As we have mentioned above, the path is not a skyline path from A to E, we can, therefore, know that the combination of two skyline paths is not necessarily a skyline path.
%\end{proof}
%\begin{enumerate}[]
%\item Whether all the paths in $P_{candi}$ are skyline paths?
%\item Whether $P_{candi}$ can include all the skyline paths from $s$ to $t$. 
%\item If it is not all the paths in $P_{candi}$ are skyline paths, how can we identify the skyline paths in the set. 
%\end{enumerate}


%Based on above discussions, we have confirmed that the set $P_{candi}$ can contain both skyline paths and dominated paths. If we can identify all the skyline paths from $P_{candi}$, the query space will be narrowed. We solve it via the following lemma. 
 
%\begin{lemma}
%\label{lemma:Quadrant}
%We first view the $w\in[0,\infty]\times c\in [0,\infty]$ as a 2-dimensional space, and the paths are the points in this space. For each path $p(w,c)$, we denote its weight as $p_w$ and its cost as $p_c$.  Then we define four quadrants accordingly:
%\begin{enumerate}
%    \item The first quadrant $p.q_1$: $p'_w > p_w$ and $p'_c > p_c$
%    \item The second quadrant $p.q_2$: $p'_w > p_w$ and $p'_c < p_c$
%    \item The third quadrant $p.q_3$: $p'_w < p_w$ and $p'_c < p_c$
%    \item The forth quadrant $p.q_4$: $p'_w < p_w$ and $p'_c > p_c$
%\end{enumerate}
%where $p'$ is any other path that is not $p$. Then it is easy to obtain the following relations: all the paths falling into $p.q_1$ are the \textit{dominated paths}. On the contrary, all the paths in $p.q_3$ are the \textit{dominating paths}. All the paths in either $p.q_2$ or $p.q_3$ are the \textit{undominated paths}.     
%\end{lemma}

%If we let weight as $x$-coordinate and cost as $y$-coordinate, a set of pairs, including weights and costs, can be points mapping on the corresponding coordinates. Therefore, we can use this method to sort all the paths in $P_{candi}$ on the coordinates. In our case, to a couple of paths $p_1$ and $p_2$, which have same origin and destination, we regard $p_1$ and $p_2$ can not dominate each other, if $p_1$ on either second or firth quadrants of $p_2$.



%...how to generate $P_{candi}$
%\subsection{Skyline Path Concatenation}

\subsection{Single Hop Skyline Path Concatenation}
\label{subsec:Skyline_Full}
Given two sets of skyline paths $P(s,h)$ and $P(h,t)$ with sizes of $m$ and $n$, it takes two operations ($O(mn)$ time \textit{path concatenation} and $O(mn\log mn)$ time \textit{skyline path validation}) to obtain the skyline result. Because the $mn$ \textit{concatenation} is inevitable, we aim to speedup the \textit{validation} by exploring the concatenation properties first. In the following, we first present the observations and algorithms for the 2D skyline path concatenation as it is simpler and has some unique characteristics. Then we generalize to the multi-dimensional case.

%Given two sets of skyline paths $P(s,h)$ and $P(h,t)$ with $|P(s,h)|=m$ and $|P(h,t)|=n$, %the full skyline path concatenation returns the skyline paths $P_s \subseteq P_c=P(s,h)\oplus P(h,t)$ %. Unlike the shortest path concatenation where one shortest path $p(s,h)$ plus another shortest path $p(h,t)$ is the shortest path from $s$ to $t$ via $h$, the s
%because the skyline concatenation does not necessarily creates a set of skylines. For example, suppose $P(s,h)=\{p_1(4,5),p_2(10,2)\}$ and $P(h,t)=\{p_3(3,2), p_4(1,20)\}$, then $p_2\oplus p_4=(11,22)$ is dominated by $p_1\oplus p_3=(7,7)$. Therefore, not all the candidates in $P_c(H)$ are still skyline paths.
%we can first generate all the candidates then use the classic \textit{nested loop} or \textit{divide-and-conquer} \cite{papadias2003optimal} to identify the skyline paths, but they are slow with complexities of $O((mn)^2)$ and $O(mn\log mn)$. %, and the latter one is the best skyline complexity without index. 
% Because the skyline path concatenation is made up of two operations: \textit{path concatenation} which takes $O(mn)$ time and \textit{skyline path validation} that takes $O(mn\log mn)$ time. In the following, we first explore  %In the following, we first prove $O(mn)$ is the minimum amount of concatenations and cannot be reduced, and then provide a greedy concatenation method to incorporate the validation into concatenation on-the-fly.



%However, it has a time complexity of $O((mn)^2)$ because $|P_c|=mn$, which is the square of the concatenation itself. A better way to solve it is through \textit{divide and conquer}, which sorts the paths based on the weight, divides them into two subsets of equal size, and finds the skyline paths of each of them recursively. During the merge phase, the results from the left are the skyline paths, while the results on the right have to compare with the left's by sorting on the cost. Obviously, the complexity decreases to $O(mn\log mn)$, and this is the best skyline complexity without index (we cannot afford to build any index in the concatenation operation as the results are generated dynamically). Finally, recall that the full skyline path concatenation is made up of two operations: path concatenation which takes $O(mn)$ time and skyline path validation that takes $O(mn\log mn)$ time. In the following, we first prove $O(mn)$ is the minimum amount of concatenations and cannot be reduced, and then provide a greedy concatenation method to incorporate the validation into concatenation on-the-fly.
%\begin{algorithm}
%	\caption{Skyline Path Nested Loop Selection}
%	\label{Algorithm:SkylineSelection}
%	\footnotesize
%	%\scriptsize
%	\LinesNumbered
%	\KwIn{Candidate Path Set $P_c$}
%	\KwOut{Skyline Path Result $P_s$}
%	$P_s\leftarrow \phi$;
%	
%	\ForEach{$p\in P_c$}
%	{
%	    $bSkyline\leftarrow True;$
%	    
%	    \ForEach{$p'\in P_c\setminus\{p\}$}
%	    {
%	        \If{$p'\in p.q_1$}
%	        {
%	            $P_c.remove(p'); continue;$
%	        }
%	        \If{$p'\in p.q_3$}
%	        {
%	            $bSkyline\leftarrow False;$
%	            $break;$
%	        }
%	    }
%        \If{$bSkyline$}
%        {
%            $P_s.insert(p);$
%        }
%        $P_c.remove(p);$
%	}
%	\Return{$P_s;$}
%\end{algorithm}

%The principle of identifying all the skyline paths in $P_{candi}$ as follows:
%\begin{enumerate}
%    \item Select one path $p_0$ in $P_{candi}$, if we find any path locates on its third quadrant, we mark $p_0$ as a dominated path;
%    \item If we can not find any path locates on its third quadrant, we mark $p_0$ as a skyline path and mark all the paths on first quadrant of $p_0$ as dominated path;
%    \item Recursively, once the selected path has been marked, we select next unmarked path in $P_{candi}$, and repeat step 1 and 2;
%\end{enumerate}


 

%\begin{definition}[divide-and-conquer]
%The technique can be summed up into three stages: $(i)$ Divide the input into two or more subsets, then $(ii)$ solve the problem separately on each subset. Afterwards, $(iii)$ Merge the solutions of the two subsets into the solution for the original input.
%\end{definition}

%In our case, we impose the screening technique to identify the dominance relationship in $P_{candi}$. The principles are shown in the following.

%For all the paths mapping on the coordinates, we first divide the set into two halves by x-coordinate. Let $P_{left}$ be the set of paths on the left half, and $P_{right}$ be the paths on the right half. Afterwards, we use the previous principle to find all skyline paths of $P_{left}$ and $P_{right}$. We denote them as $A_{left}$ and $A_{right}$ separately. The set of $A_{left}$ will be the final skyline paths of $P_{candi}$. For $A_{right}$, we need to check further. If a path in $A_{right}$ is a skyline path in $P_{candi}$, it must be undominated by all the paths in $A_{left}$. We solve $A_{right}$ by projecting both $A_{left}$ and $A_{right}$ onto the y-coordinate. As all the paths in $A_{right}$ have greater weights than the paths in $A_{left}$, to the projections of $A_{left}$ and $A_{right}$ on y-coordinate, we only screen out the points in $A_{right}$ that have less $y$ than the smallest y in $A_{left}$. We eventually return the matched points in $A_{right}$ and the set of $A_{left}$ as our final skyline paths. Furthermore, with the bound of maximum cost, we can easily select the CSP from the results. The time complexity of the search can reach $O(nlogn)$.

%(connect first and then prune -> confirm skyline paths during connecting->it is NP-hard->save the time of prune after connecting all the skyline paths)...To overcome the drawbacks of the naive solution, we intend to avoid the prune stage on $P_{candi}$, instead, we apply the strategy of conforming all the skyline paths during the connecting processing. The advantage of it is in the following:
%\begin{enumerate}
%\item In index construction, we can avoid the pruning on calculating labels for each vertex, and adjust the skyline paths of each label by the weight in an ascending order during the connecting processing.
%\item In query processing, after combining the skylines in corresponding in label and out label, if we can ensure all the skyline paths return are ordered by the weight with an ascending order, these skyline paths are naturally sorted by the cost with an descending order. Thus, we can scan the set of the paths return from the skyline path with largest cost. The first skyline path that cost less then the constraint cost $C$, which given in the query, will be the optimal result of CSP.  
%\end{enumerate}
%we introduce our heuristic method to reduce the search space of CSP. The method is designed based on the following corollaries. 

\subsubsection{2D Skyline Path Concatenation Observations}
The 2D skyline dataset has a unique characteristic compared with the multi-dimensional skyline dataset: when we sort all the data in the weight-increasing order, their costs are naturally sorted in the decreasing order. Therefore, we have the following four observations to help improve the concatenation efficiency. We first dig into the simplest \textit{1-n / m-1} skyline concatenation. The following property proves that we do not need validation for this simple case:
%different types of concatenation to identify when the validation is necessary and which path should be compared. The following lemma proves the skyline relation is preserved with 1-$N$ and $N$-1 concatenation. 
\begin{property}
\label{lemma:SingleConcatenation} \textit{\textbf{(1-n / m-1 Skyline)}}
$\forall p\in P(s,h)$, $p\oplus P(h,t)$ can generate $n=|P(h,t)|$ paths that cannot dominate each other. Similarly, $\forall p'\in P(h,t)$, $P(s,h)\oplus p'$ can generate $m=|P(s,h)|$ paths that cannot dominate each other.
\end{property}
\begin{proof}
We only need to prove the first half. Suppose we choose $p(w,c)$ from $P(s,h)$. Because $P(h,t)$ is the skyline path set, we select any two paths from it: $p_1(w_1,c_1)$ and $p_2(w_2,c_2)$. Suppose $w_1\leq w_2$ and $c_1 \geq c_2$, then this relation still holds because $w_1+w\leq w_2+w$ and $c_1+c \geq c_2+c$. 
\end{proof}

%Therefore, the paths in $p\oplus P(h,t)$ do not have to compare with each other as the results are always skyline. So do the paths in $P(s,h)\oplus p'$. 

Next we explore the \textit{m-n} concatenation case. Suppose all the skyline paths are sorted in the weight-increasing order. We define $p_i(s,h)=(w_i,c_i)$ ($i\in[1,m]$) as the $i^{th}$ skyline path in $P(s,h)$, $p'_j(h,t)=(w'_j,c'_j)$ ($j\in[1,n]$) as the $j^{th}$ skyline path in $P(h,t)$, and $p_i^j$ as the concatenation path of $p_i(s,h)$ and $p'_j(h,t)$. Therefore, $p_1^1$ is the concatenation of the first skyline path in $P(s,h)$ and the first path in $P(h,t)$, and $P_m^n$ is the  concatenation of the last skyline path in $P(s,h)$ and the last one in $P(h,t)$. Then they have the following property:
\begin{property}
\label{lemma:FirstandLast} \textit{\textbf{(Endpoint Skyline)}}
$p_1^1$ and $p_m^n$ are two endpoints of the concatenation results and they are skyline paths.
\end{property}
\begin{proof}
$p_1^1=p_1(s,h)\oplus p'_1(h,t)=p(w_1+w'_1, c_1+c'_1)$. Because $w_1$ is the smallest in $p_1(s,h)$ and $w'_1$ is the smallest in $p'_1(h,t)$, $w_1+w'_1$ is still the smallest weight in $P_c$. Similarly, $p_m^n=p_m(s,h)\oplus p'_n(h,t)=p(w_m+w'_n, c_m+c'_n)$ has the smallest cost in $P_c$. Therefore, no other path in $P_c$ can dominate $p_1^1$ and $p_m^n$.
\end{proof}

Finally, we explore the domination relations among the paths between the endpoints. Given any concatenated path $p_i^j$, we can classify the other paths (except the ones generated by $p_i$ and $p'_j$) into four categorizes as shown in Figure \ref{fig:ConcatenationCategory}. %\ref{fig:ConcatenationDominance}:
%\begin{itemize}
%    \item $P_1=p_{<i}(s,h)\oplus p'_{<j}(h,t)$ %that is concatenated by all the paths with smaller weights than $p_i(s,h)$ and all the paths with smaller weights than $p'_j(h,t)$
%    \item $P_2=p_{>i}(s,h)\oplus p'_{>j}(h,t)$ %that is concatenated by all the paths with larger weights than $p_i(s,h)$ and all the paths with larger weights than $p'_j(h,t)$
%    \item $P_3=p_{<i}(s,h)\oplus p'_{>j}(h,t)$ %that is concatenated by all the paths with smaller weights than $p_i(s,h)$ and all the paths with larger weights than $p'_j(h,t)$
%    \item $P_4=p_{>i}(s,h)\oplus p'_{<j}(h,t)$ %that is concatenated by all the paths with larger weights than $p_i(s,h)$ and all the paths with smaller weights than $p'_j(h,t)$
%\end{itemize}
The following two properties provide the dominance relations between $p_i^j$ and these four path sets.


%\begin{figure}[ht]
%    \centering
%    \includegraphics[width=3.2in]{ConcatenationDominance2.eps}
%    \caption{Concatenated Path Category}
%    \label{fig:ConcatenationDominance}
%\end{figure}


\begin{property}
\label{theorem:ConcatenationUnDominance} \textit{\textbf{(Side-Path Irrelevant)}} The concatenated path $p_i^j$ cannot be dominated by the paths in $P_1$ and $P_2$.
\end{property}
\begin{proof}
$\forall p_k\in p_{<i}$ and $p'_k\in p'_{<j}$, $c_k > c_i$ and $c'_k>c_j$. Therefore, $c_k+c'_k > c_i+c'_j$, so $P_1$ cannot dominate $p_i^j$. Similarly, $\forall p_k\in p_{>i}$ and $p'_k\in p'_{>j}$, $w_k > w_i$ and $w'_k>w_j$. Therefore, $w_k+w'_k > w_i+w'_j$, so $P_2$ cannot dominate $p_i^j$.
\end{proof}



%Based on the corollaries, we can identify the dominance during the connecting processing. The theorem are shown as follows.
\begin{property}
\label{theorem:ConcatenationDominance} \textit{\textbf{(Cross-Path Relevant)}}
$p_i^j$ is a skyline path iff it is not dominated by any path in $P_3$ and $P_4$.
\end{property}
\begin{proof}
$\forall p_k\in p_{<i}$ and $p'_k\in p'_{>j}$, we have $c_k > c_i$ and $c'_k<c_j$, $w_k > w_i$ and $w'_k<w_j$, so $c_k+c'_k$ has no relation with $c_i+c'_j$, and $w_k+w'_k$ has no relation with $w_i+w'_j$. Therefore, paths in $P_3$ has the possibility to dominate $p_i^j$, and same for $P_4$. In other words, it is the paths in $P_3$ and $P_4$ that determines if $p_i^j$ could be a skyline path or not.
\end{proof}

%For each $p_i^j$, its $P_3$ has $O((i-1)\times(n-j))$ paths and $P_4$ has $O((m-i)\times(j-1))$ paths. Therefore, the dominance $p_i^j$ is determined by $|P_3|\times|P_4|=O((i-1)\times(n-j)+(m-i)\times(j-1))$ paths. The total number of comparisons is:
%\begin{equation*}
%\scriptsize
%\begin{aligned}
%    &\sum_{i=1}^m \sum_{j=1}^n (i-1)\times(n-j)+(m-i)\times(j-1)\\
%    &=\sum_{i=1}^m \sum_{j=1}^n (in+jm-2ij+i+j-(m+n))\\
%    &=\dfrac{(n^2+n)m^2+(n^2+n-2)m-2n}{2}<m^2n^2
%\end{aligned}
%\end{equation*}


%Thus, to a connecting path $p_{x_2}^{x_1}$, the dominance relations of it can be confirmed by a set of paths $p_{{x_2}+k_2}^{{x_1}-k_1}$,$0 \leq k_1 \leq x_1$, $0 \leq k_2 \leq n-x_2$ and a set of paths $p_{{x_2}-k_2}^{{x_1}+k_1}$, $0 \leq k_1 \leq m-x_1$, $0 \leq k_2 \leq x_2$.                    

%By corollary \ref{corollary 2}, we can prove that the problem of conforming the skyline paths during the connecting processing is NP-hard, as we have to check the dominance relations of one connecting path $k_1(n-k_2)+(m-k_1)k_2)$ times.
%$p_{x_2}^{x_1}$ is a connecting path by  $p_{x_1}.h_i$ and  $p'_{x_2}.h_i$. Each path on the left of $x_1$ can constitute a $s-t$ path set $P_1$ by connecting each path on the right of $x_2$. Each path on the right of $x_1$ can constitute a $s-t$ path set $P_2$ by connecting each path on the left of $x_2$. We can identify if $p_{x_2}^{x_1}$ is a skyline path from $s$ to $t$, it must not dominated by any path in $P_1$ and $P_2$. 
%We define $p_{x_1}.h_i$ as the ${x_1}^{th}$ skyline path in $P(h_i)$, $0 \leq x_1 \leq m$, $p'_{x_2}.h_i$ is the ${x_2}^{th}$ skyline path in $p'(h_i)$, $0 \leq x_2 \leq n$. $p_{x_2}^{x_1}$ is a connecting path by  $p_{x_1}.h_i$ and $p'_{x_2}.h_i$. Each path on the left of $x_1$ can constitute a $s-t$ path set $P_1$ by connecting each path on the right of $x_2$. Each path on the right of $x_1$ can constitute a $s-t$ path set $P_2$ by connecting each path on the left of $x_2$. We can identify if $p_{x_2}^{x_1}$ is a skyline path from $s$ to $t$, it must not dominated by any path in $P_1$ and $P_2$. 

%$p_{m}.h_i$ and $p_{m-1}.h_i$ are two skyline paths in $P(h_i)$, $p'_{n}.h_i$ and $p'_{n+1}.h_i$ are two skyline paths in $P'(h_i)$.   


%\begin{figure}[ht]
%    \centering
%    \includegraphics[scale=0.5]{2-2.png}
%    \caption{}
%    \label{fig:2-2.png}
%\end{figure}


%We can first identify the case when $m=2$ and $n=2$, which shown in Figure \ref{fig:2-2.png}. Suppose $s$ to $t$ has only one intermediate hop $h_i$, $P(h_i)$ has two skyline paths $p_1$ and $p_2$, $P'(h_i)$ has two skyline paths $p'_1$ and $p'_2$. These two sets can generate four different paths from $s$ to $t$, which are $p_1^1$, $p_2^1$, $p_1^2$, and $p_2^2$. On the basis of corollary \ref{corollary 1}, we can identify that $p_1^1$ and $p_2^1$ cannot dominate each other. In the same way, $p_2^1$ and $p_2^2$ cannot dominate each other as well. Thus, the dominance relations of $p_1^2$ can be only confirmed by $p_2^1$ and and vice versa. 

%When $P(h_i)$ has $m$ skyline paths and $P'(h_i)$ has $n$ skyline paths, to generate $s$ to $t$ paths, we can produce $mn$ pairs by pair-wise connecting. Any two pairs will satisfy the rules in Figure \ref{fig:2-2.png}. 


\subsubsection{Efficient 2D Skyline Path Concatenation}
The above properties enable us to reduce the validation operations and speed up the 2D concatenation. The following theorem further reduces the comparison number in the validation operation:
%Unlike the classic skyline problem whose input is a set of points, the skyline path concatenation problem takes two sets of skyline paths as input and generates results on the fly. Therefore, we can take advantage of this difference and test a small number of paths to validate the skyline efficiently.

\begin{theorem}
\label{theorem:GreedySkyline}
Suppose the concatenated paths are coming in the weight-increasing order. We have $k$ skyline paths and a new path $p_{k+1}$ comes with weight larger than $w_k$. If $p_k$ cannot dominate $p_{k+1}$, then $p_{k+1}$ must be a skyline path. 
\end{theorem}
\begin{proof}
%Since paths are coming in the weight-increasing order, 
$p_{k+1}$ cannot be dominated by latter paths because $w_{k+1}\leq w_j, \forall j>k+1$. $p_k$ has the smallest cost of the current skyline paths. If $c_k\geq c_{k+1}$, then the other paths' cost are also larger than $c_{k+1}$. Therefore, if $p_k$ cannot dominate $p_{k+1}$, then no  future path can dominate it.
\end{proof}

%To solve the problem above, we introduce a method to identify all the skyline paths in $P_{candi}$ during the connecting processing with the idea of divide and conquer. This method can ensure that we can only check the dominance relations of each connecting path one time. 

%\begin{figure}[ht]
%    \centering
%    \includegraphics[width=1.7in]{Increasing.pdf}
%    \caption{Next Skyline Path Validation}
%    \label{fig:Increasing}
%\end{figure}

\begin{figure}[ht]
    \centering
    \includegraphics[width=2.3in]{Concatenation2.pdf}
    \caption{Next Skyline Path Validation}
    \label{fig:ConcatenationExample}
\end{figure}
For example in Figure \ref{fig:ConcatenationExample}, we have a set of skyline paths $\{p_1,p_2,p_3,p_4\}$ sorted in the weight-increasing order and $p_5$ is the next concatenated path with the next smallest weight. Therefore, $p_5$ can only locate in the right regions of $p_4$. If $p_5$ is in the red region, it is dominated by $p_4$ and discarded; If $p_5$ is in the green region, it will become the next skyline path. 

%Based on Theorem \ref{theorem: dominating a bicriterion path}, in the connecting processing, if we can obtain connecting paths from the one with the smallest weight to the one with the largest weight, for each connecting, we can identify the dominance relations of the current connecting path by the last conformed skyline path. Thus we introduce a greedy method of connecting in the following section.

\begin{algorithm}[ht]
	\caption{Efficient 2D Skyline Path Concatenation}
	\label{Algorithm:GreedyConcatenation}
%	\scriptsize
	\LinesNumbered
	\KwIn{Sorted Skyline Path Set $P(s,h)$ and $P'(h,t)$}
	\KwOut{Skyline Concatenated Path $P_s\subseteq P(s,h)\oplus P'(h,t)$}
	\SetKwProg{Fn}{Procedure}{}{}
	$p_1^1\leftarrow p_1(s,h)\oplus p'_1(h,t)$; $P_s.insert(p_1^1)$\;
	$p_1^2\leftarrow p_1(s,h)\oplus p'_2(h,t)$; $Q.insert(p_1^2)$\;
	$p_2^1\leftarrow p_2(s,h)\oplus p'_1(h,t)$; $Q.insert(p_2^1)$\;
	%;//$Q$ is a priority queue sorted on weight \; 
	\While{$!Q.empty()$}
	{
	    $p_i^j\leftarrow Q.pop()$; $p_{max}\leftarrow P_s[|P_s|-1]$\;
	    \If{$c_i^j\leq c_{max}$}
	    {
	        $P_s.insert(p_i^j)$\;
	    }
	    $LazyInsert(i,j)$\;
	}
	\Return $P_s$\;
%	\begin{multicols}{2}
%	\end{multicols}
	%\Fn{$LazyInsert(i,j)$}{}
%	\textbf{Procedure} $LazyInsert(i,j)$\\
	\Fn{$LazyInsert(i,j)$}
		%\begin{multicols}{2}
	{
	    \If{$i+1<m$}
	    {
	        \If{$p_{i+1}^j$ is visited}
	        {
	            $LazyInsert(i+1,j)$\;
	            break\;
	        }
	    
	            $p_{i+1}^j\leftarrow p_{i+1}(s,h)\oplus p'_j(h,t)$\;
	            \If{$c_{i+1}^j>c_{max}$}
	            {
	                $LazyInsert(i+1,j)$\;
	            }
	            \Else{$Q.insert(p_{i+1}^j)$}
	        
	    }
	    \If{$j+1<n$}
	    { 
	        \If{$p_i^{j+1}$ is visited}
	        {
	            $LazyInsert(i,j+1)$\;
	            break\;
	        }
	            $p_i^{j+1}\leftarrow p_{i}(s,h)\oplus p'_{j+1}(h,t)$\;
	            \If{$c_{i}^{j+1}>c_{max}$}
	            {
	                $LazyInsert(i,j+1)$\;
	            }
	            \Else{$Q.insert(p_{i}^{j+1})$}
	        
	    }
	   }
	  %  \end{multicols}
\end{algorithm}


Based on Theorem \ref{theorem:GreedySkyline}, we propose an efficient skyline path concatenation as shown in Algorithm \ref{Algorithm:GreedyConcatenation}. As proved in Property \ref{lemma:FirstandLast}, $p_1^1=p_1(s,h)\oplus p'_1(h,t)$ is definitely a skyline result and we put it into the result set $P_s$. Because the next path with the smallest weight is either $p_1^2$ or $p_2^1$, we put them in a priority queue $Q$ as candidates. Then we iterate the candidate queue until it is empty. Each time we retrieve the top path $p_i^j$ in $Q$ and compare it with the last path in $P_s$. If $p_i^j$ is not dominated, we put $p_i^j$ into $P_s$. Then we generate the next two candidates $p_{i+1}^j$ and $p_i^{j+1}$ if they exist. However, we do not insert them into $Q$ directly as they could be dominated by the last path in $P_s$ already, or they could have already been generated by other paths. Therefore, we use the \textit{LazyInsert} to identify the next set of candidates that are not dominated (Line 16 and 25) and not generated (Line 12 and 21) recursively. In this way, the pruning power of the current skyline path is maximized, and we could have a $Q$ of smaller size and eliminate the redundancy.



\textit{Correctness:} Firstly, because we generate and test both $p_{i+1}^j$ and $p_i^{j+1}$ of all $p_i^j$ even if some of them are not inserted into $Q$, we have produced all $mn$ candidates. Secondly, because $Q$ is sorted by weight, and both $p_{i+1}^j$ and $p_i^{j+1}$ have larger weight than $p_i^j$, we visit the $p_i^j$ from $Q$ in the weight-increasing order. Therefore, according to Theorem \ref{theorem:GreedySkyline}, Algorithm \ref{Algorithm:GreedyConcatenation} returns a set of concatenated skyline paths.

\textit{Complexity:} The maximum depth of $Q$ is $log(mn)$, so it takes $O(mn\log(mn))$ to pop out all the elements. Since we just check the dominant relation once for each connecting path, the skyline validation time for each path is constant. Although the worst case time complexity of concatenating all the skyline paths via $h$ is still $O(mn\log(mn))$, the \textit{LazyInsert} pruning can keep the size of $Q$ small in practice.
%\subsection{Greedy method on connecting skyline paths}
%We stick with the previous assumption that $h_i$ is the unique intermediate hop from $s$ to $t$. $P(h_i)$ has a set of skyline paths ($p_1, p_2, p_3,...,p_m$), which sorted in an ascending order of weight. $P'(h_i)$ has a set of skyline paths ($p'_1, p'_2, p'_3,...,p'_n$) that sorted in an ascending order of weight as well. Therefore, the path $p_1^1$, which connected by $p_1$ and $p'_1$, must be a skyline path from $s$ to $t$ that has the smallest weight. 

%Then, we need a priority queue $q$ to store the connected paths. $p_1^1$ will be the first element in $q$. In the heap of $q$, we set the top element is always the path with the smallest weight. Thus, the first element that pops out must be $p_1^1$, which means we have obtain a path with the smallest weight. As it must be an skyline path, we store it in a $s-t$ skyline list $S$.  Consequently, as $p_1^1$ is connected by $p_1$ and $p'_1$, we select the right adjacent paths of $p_1$ and $p'_1$, which are $p_2$ and $p'_2$ respectively. Apart from $p_1^1$, we can conform that the path with smallest weight must be $p_2^1$ or $p_1^2$. We push both $p_2^1$ and $p_1^2$ into $q$. Suppose the weight of $p_2^1$ is greater than the weight of $p_1^2$, $p_2^1$ will be taken out as the top element in $q$. For a top element $p_j^i$ in $q$, we have the principles in the following:
%\begin{enumerate}
%    \item Pop out $p_j^i$ from $q$.
%    \item Connect $p_i$ with $p_{j+1}$ to constitute $p_{j+1}^i$. Then, we connect $p_j$ with $p_{i+1}$ to constitute $p_j^{i+1}$.
%    \item Push $p_{j+1}^i$ and $p_j^{i+1}$ in $q$.
%    \item Fine the next top element in $q$ and repeat the above three steps.
%\end{enumerate}

%When $p_j^i$ pops out, suppose $S$ already has $k$ skyline paths from $s$ to $t$, we need to check the dominance relations between $p_j^i$ and the $k_{th}$ skyline paths in $S$. Based on Theorem \ref{theorem: dominating a bicriterion path}, if the $k_{th}$ skyline paths can not dominate $p_j^i$, we treat $p_j^i$ as a skyline path from $s$ to $t$ and store it in $S$. Otherwise, we discard $p_j^i$ and pops out the next element in $q$. By this way, we can ensure that all the paths in $S$ are skyline paths from $s$ to $t$ via $h_i$. 

%\begin{figure}[ht]
%    \centering
%    \includegraphics[width=1.7in]{SkylineRectangle.pdf}
%    \caption{Multiple Skyline Rectangle and Query Rectangle (Shaded)}
%    \label{fig:SkylineRectangle}
%\end{figure}

\subsubsection{Multi-Dimensional Skyline Path Concatenation}
Although the previous observations, theorems, and algorithms efficiently reduce the complexity of skyline path validation in 2D road networks, they take the advantages of the 2D skyline path cost being natural ranking when sorted in weight-increasing order, which does not hold in the higher dimensional space. For instance, in algorithm \ref{Algorithm:GreedyConcatenation}, when a new path $p_i^j$ is concatenated, its weight must be no less than all the skyline paths in $P_s$. Thus, we only need to compare the cost of $p_i^j$ with the cost of the ranked last path in $P_s$, which has the minimum cost. However, this skyline validation method will be not feasible when each path has multiple costs, as we can not guarantee the ordering of costs for a weight-sorting multi-skyline path set. For example in Table \ref{table:EG_skylines}, it has five 4D skyline paths. Even though we sort them by the weigh-increasing order, the remaining three costs have no order at all. To reduce the comparison number of skyline validation in paths with multiple costs, we first investigate into the order properties of the multi-dimensional skyline paths:

\begin{definition}[Cost Rank]
	\label{def:Cost_Rank}
	Given a set of skyline paths in a $n$-dimensional graph, we sort them in each of the cost $c_i$ in the increasing order. Then $r_i[p_k]$ denotes the rank of path $p_k$ in cost $c_i$. 
	\end{definition}

For example, in Table \ref{table:EG_skylines}, we have a set of skyline paths $\{p_1, p_2, p_3, p_4, p_5\}$. On each dimension, we rank the paths with increasing order, which is shown in Figure \ref{fig:MultiSkylineValidation} (ignore $p_6$ at this stage). Then $r_1[p_4]=1$ because $p_4$ has the smallest value in cost $c_1$. Similarly, $r_2[p_5]=2$ and $r_3[p_4]=3$. For each path $p$, it has a rank in each dimension, and the following \textit{distinct criterion} is the one we are most interested in:

\begin{definition}[Distinct Criterion]
	Among the $n$ rankings of a path $p$ in $G$, its \textit{Distinct Criterion} is the one with the highest rank denoted as $c_{dc}[p]$.
\end{definition}

\begin{table}[]
\centering
\caption{An Example of 4D Skyline Paths}
\label{table:EG_skylines}
%\scriptsize
%\scalebox{1.1}{
\begin{tabular}{|l|l|l|l|l|}
\hline
$P_c$ & $w$ & $c_1$ & $c_2$ & $c_3$ \\ \hline
$p_1$ & 2   & 4     & 10    & 2     \\ \hline
$p_2$ & 2   & 4     & 9     & 3     \\ \hline
$p_3$ & 3   & 7     & 7     & 10    \\ \hline
$p_4$ & 5   & 3     & 9     & 3     \\ \hline
$p_5$ & 6   & 6     & 8     & 4     \\ \hline
\end{tabular}
%}
\end{table}

For example, $p_3$'s distance criterion is $c_2$ as it is the smallest compared its ranking in other criteria: $r_w[p_3]=3$, $r_1[p_3]=5$, and $r_3[p_3]=5$. Similarly, the distinct criterion of $p_1$ is $w$, $c_{dc}[p_2]$ is $c_3$, $c_{dc}[p_4]$ is $c_1$, and $c_{dc}[p_5]$ is $c_2$. Then we utilize the distinct criterion to further investigate the dominant relation in the high-dimensional space:

\begin{lemma}
\label{lemma:Multi-Non-Dominate}
%In $n$-dimensional graph, suppose the concatenated paths are coming in the weight-increasing order. We have $k$ skyline paths and a new path $p_{k+1}$ comes with weight larger than $w_k$. $\forall c_i \in \overline{C}$, $i\leq n$, we rank $k+1$ paths in cost-increasing order and obtain the rank of $p_{k+1}$, which is denoted as $r_i(k+1)$. $\exists o \in [1,n)$ such that $r_o(k+1)$ is minimum compared with arbitrary $r_i(k+1)$. The corresponding criterion $c_o$ is named as distinct criterion. Suppose $m$ concatenated skyline paths, $m \leq k$, have higher or equal ranking than $r_o(k+1)$ on $c_o$. If all the $m$ paths cannot dominate $p_{k+1}$, then $p_{k+1}$ must be a skyline path. 
	Suppose we already have $k$ skyline paths, and we aim to test a new path $p_{k+1}$ with weight no-smaller than the existing ones. After inserting into the existing criteria sorting lists, we can obtain the ranks $m_i$ of $p_{k+1}$ in each criteria $c_i$. Suppose $p_{k+1}$ is ranked last among all the paths with the same value. Then all the paths $P_i^{>m}$ that have ranking lower than $m_i$ have larger value than $p_{k+1}$ in criteria $c_i$, and they cannot dominate $p_{k+1}$.
\end{lemma} 
\begin{proof}
	Because the dominance relation requires smaller value, they cannot dominate $p_{k+1}$.
\end{proof}

For example in Figure \ref{fig:MultiSkylineValidation}, we insert a new path $p_6=(8,5,8,9)$. As $p_6$ has greater weight than the five existing paths, it must be ranked last on dimension $w$. Then, we find the ranks of $p_6$ on other dimensions, which are highlighted in red. $p_6$ is ranked 4, 3 and 5 in $c_1$, $c_2$ and $c_3$. Then along criteria $c_2$, paths $P_c^{>3}=\{p_2,p_4,p_1\}$ have lower ranking and larger values than $p_4$, so they cannot dominate $p_6$. We can have the following lemma by taking complementary set of Lemma \ref{lemma:Multi-Non-Dominate}.

\begin{lemma}
	\label{lemma:Multi-Dominate}
	Following Lemma \ref{lemma:Multi-Non-Dominate}, all the paths $P_i^{\leq m}$ that have ranking higher in criteria $c_1$ than $p_{k+1}$ are possible to dominate $p_{k+1}$.
\end{lemma}

For example in Figure \ref{fig:MultiSkylineValidation}, $P_1^{\leq 4}=\{p_4,p_1,p_2\}$ can possibly dominate because they rank higher than $p_6$ along $c_1$.  Now we have the sufficient and necessary requirement for $p_{k+1}$ being a new skyline path:
\begin{theorem}
	\label{theorem:MultiGreedySkyline}
	Following Lemma \ref{lemma:Multi-Dominate}, $p_{k+1}$ is a skyline path if and only if none of the $m-1$ higher ranking paths $P_i^{\leq m}$ in any criteria $c_i$ can dominate $p_{k+1}$.
\end{theorem}

\begin{proof}
	Because the paths $P_i^{\leq m}$ have either equal or smaller values than $p_{k+1}$ along criteria $c_i$, then the other paths $P_i^{>m}$ have larger values and cannot dominate $p_{k+1}$. Therefore, if none of the paths in $P_i^{\leq m}$ can dominate $p_{k+1}$, then no existing skyline path can dominate $p_{k+1}$, so $p_{k+1}$ is a skyline path.
%We divide the $k$ skyline paths into two set $S_1$ and $S_2$. $S_1$ contains the $m$ skyline paths that have higher or equal ranking than $p_{k+1}$ on dimension $c_{dc}[p_{k+1}]$. $S_2$ contains the remaining skyline paths.  Compared with all the paths in $S_2$, $p_{k+1}$ has largest value on dimension $c_o$ and highest value on dimension $w$. Thereby, $p_{k+1}$ is a skyline path in set $S_2$. As $p_{k+1}$ has larger weight than the $k$ skyline paths, $p_{k+1}$ can not dominated each path in $S_1$. According to definition \ref{def:Multi-SkylinePath}, if no path in $S_1$ can dominate $p_{k+1}$, it must be a skyline paths in $S_1$. Due to $p_{k+1}$ is a skyline path in both $S_1$ and $S_2$, it is a skyline path in the current concatenated path set. Also, we have proved that $p_{k+1}$ cannot be dominated by latter coming paths in Theorem \ref{theorem:GreedySkyline}. $p_{k+1}$ thus must be a final skyline path.
\end{proof}

\begin{figure}[ht]
    \centering
    \includegraphics[scale=0.25]{MultiGreedy.pdf}
    \caption{Next Skyline Path Validation in Multi-dimensions. New $p_6=(8,5,8,9)$.}
    \label{fig:MultiSkylineValidation}
\end{figure}

%Suppose we have the next concatenated path $p_6={8, 5, 8, 9}$. The distinct criterion is $c_2$. We need to identify whether $p_6$ can be dominated by $p_3$ or $p_5$. As $p_6$ cannot be dominated, $p_6$ is a skyline path.

Although any criterion can work for Theorem \ref{theorem:MultiGreedySkyline}, not all of them have the same quality. For instance, along the dimension $w$, $p_{k+1}$ is ranked last and has $k$ possible dominating paths, so we have to compare $p_{k+1}$ with all $k$ previous paths. Therefore, using the criterion with the least number of possible dominating path would be beneficial, and the distinct criterion $c_{dc}[p]$ is guaranteed to have the smallest $P_i^{\leq m}$ as $p_{k+1}$ ranks highest along it. Then we have the following tighter condition:

\begin{theorem}
	\label{theorem:MultiGreedySkylineDC}
	$p_{k+1}$ is a skyline path if and only if none of the $m-1$ higher ranking paths $P_i^{\leq m}$ in the distinct criteria $c_{dc}[p]$ can dominate $p_{k+1}$.
\end{theorem}

%However, in Theorem \ref{theorem:MultiGreedySkylineDC}, if the next concatenated path $p_{k+1}$ has the same weight with $p_k$, we need to do skyline validation between $p_{k+1}$ and each path that has the same weight with it. If $p_{k+1}$ is dominated, we concatenate next path. If $p_{k+1}$ can dominate any paths having the same weight with it, we remove the dominated paths from the concatenated set. Afterwards, we use Theorem \ref{theorem:MultiGreedySkyline} to further do the skyline validation for $p_{k+1}$. For example, suppose we change $p_6$ to ${6,5,8,9}$. It has the same weight with $p_5$. We compare $p_5$ and $p_6$, as they can not dominate each other, we further check the highest rank of $p_6$ as the same as the previous discussion. 

The complexity of using Theorem \ref{theorem:MultiGreedySkylineDC} is $O((|P_{r_{dc}[p_{k+1}]}^{\leq m}|+log k)\times n)$. It requires obtaining all the ranks first and comparing with all the criteria. One way to improve the efficiency is converting the value comparison to the dominating path set intersection:

\begin{theorem}
	\label{theorem:MultiGreedySkylineIntersection}
	Suppose we have obtained all the $P_i^{\leq m_i}$, then	$p_{k+1}$ is a skyline path $\Leftrightarrow\bigcap_{i\in[1,n]} P_i^{\leq m_i} = \phi$
	% none of the $m-1$ higher ranking paths $P_i^{\leq m}$ in the distinct criteria $c_{dc}[p]$ can dominate $p_{k+1}$.
\end{theorem}
\begin{proof}
	Suppose $\exists p_i \in \bigcap_{i\in[1,n]} P_i^{\leq m_i}$, then $p_i$ has higher rank than $p_{k+1}$ in all criteria, so $p_i$ dominates $p_{k+1}$ and $p_{k+1}$ is not a skyline path.
\end{proof}

As the intersection result cannot become larger, we can compute the result in the $|P_i^{\leq m_i}|$ increasing order to keep reducing the intermediate result size. This order can also be used in the value testing method. To further reduce the sorting complexity, we apply the \textit{lazy comparison} to only continue the sorting on the criteria when needed. We first introduce the hierarchical approximate rank as follows:

\begin{definition}[Hierarchical Approximate Rank]
	\label{def:HA-Rank}
	Given a set of $m$ sorted numbers $S$ and a query value $q$, $q$'s rank binary search at level $h_0$ is $HA_0(q)=m/4$ if $q<S[m/2]$ and $HA_0(q)=m/2$ if $q\geq S[m/2]$. Suppose we are at level $h_i$ and the current \textit{HA-Rank} is $HA_i(q)$, then for the next level $h_{i+1}$, we have the following three scenarios: 1) $HA_{i+1}(q)=(2HA_i(q)-1)/2$ if $q<S[HA_i(q)]$; 2) $HA_{i+1}(q)=HA_i(q)$ if $q\geq S[HA_i(q)]$ and $q< S[HA_{i-1}(q)]$; and 3) $HA_{i+1}(q)=(2HA_i(q)+1)/2$ if $q\geq S[HA_i(q)]$ and $q\geq S[HA_{i-1}(q)]$. Regardless of the level number, the \textit{HA-Rank} are compared with their values.
\end{definition}

The intuition behind it is that we set the \textit{HA-Rank} optimistically. When $q$ is smaller than the value at the current  \textit{HA-Rank}, we set it to a smaller \textit{HA-Rank}; when $q$ is not smaller than the value at the current \textit{HA-Rank} but smaller than the previous one, we keep the current \textit{HA-Rank}; when $q$ is not smaller than the values at the current \textit{HA-Rank} and the previous one, we set it to a larger rank.

Now in our case of $k$ $n$-dimensional skyline paths, we sort them using the \textit{HA-Rank} with query value $p_{k+1}$. Specifically, each time we update the \textit{HA-Rank} of the criterion that has the highest \textit{HA-Rank} value until one criterion has reached the actual data. Then this criterion is $p_{k+1}$'s distinct criterion, and we have also got $p_{k+1}$'s rank on it. We can keep sorting to get the $2^{nd}$, $3^{rd}$ till the last distinct criterion if keeps searching on. Algorithm \ref{Algorithm:Multi-Validation} shows the details of the validation using the lazy comparison with \textit{HA-Rank}.


\begin{algorithm}[ht]
	\caption{Multi-Dimension Skyline Path Intersection Validation}
	\label{Algorithm:Multi-Validation}
%	\scriptsize
	\LinesNumbered
	\KwIn{$n$-Dimensional Skyline Paths $\{p_1,\dots,p_k\}$, new path $p_{k+1}$}
	\KwOut{If $p_{k+1}$ is a skyline path}
	$(c, m)\leftarrow HA\_Sort(p_{k+1})$; \Comment{$c$ is the distinct criteria and $m$ is its corresponding rank}\;
	$P'\leftarrow P^{\leq m}_c$\;
	$counter\leftarrow 1$\;
	\While{$P'\neq \phi$ and $counter< n$}
	{
		$(c', m')\leftarrow HA\_Sort(p_{k+1})$\;
		$P' \leftarrow P' \bigcap P^{\leq m'}_{c'}$\;
		$counter\leftarrow counter+1$\;
	}
	
	\If{$P'\neq \phi$}
	{
		\Return{$p_{k+1}$ is a skyline path}
	}
	\Else
	{
		\Return{$p_{k+1}$ is not a skyline path}
	}
	
	
\end{algorithm}

However, the efficiency of Algorithm \ref{Algorithm:Multi-Validation} depends on the number of the paths having higher or equal ranking than the new coming path $p_{k+1}$. If $p_{k+1}$ ranks very low on distinct criterion, then we may compare a large amount of skyline paths, which is still time consuming. Thus, we provide a pruning technique to identify the non-skyline earlier with the help of the following theorem.

\begin{theorem}
	\label{theorem: MultiGreedyPruning}
	Suppose we have obtained all the $P_i^{> m_i}$, then $p_{k+1}$ is not a skyline path $\Leftrightarrow |\bigcup_{i\in[1,n]} P_i^{\leq m_i}| < k$.
	%In $n$-dimensional graph, suppose the concatenated paths are coming in the weight-increasing order. We have $k$ skyline paths and a new path $p_{k+1}$ comes with weight larger than $w_k$. We rank $k+1$ paths as the same as Theorem \ref{theorem:MultiGreedySkyline}. Compute the number of paths that has lower ranking than $p_{k+1}$ on at least one criterion. If the number less than $k$, $p_{k+1}$ is not a skyline path.
\end{theorem}

\begin{proof}
	 We proof it by contraction. Suppose $p_{k+1}$ is a skyline path and there are $k-1$ skyline paths having lower ranking than $p_{k+1}$ on at least one criterion. As $p_{k+1}$ has the larger weight than these $k$ paths. We only need to consider the rankings on the criteria of costs. Except $p_{k+1}$, $k$ paths are considered in the rankings. Thereby, it must has at least one skyline path $p_i$, $\forall i \leq k$, having higher or equal ranking than $p_{k+1}$ on all the criteria of costs. According to definition \ref{def:Multi-Dominance}, $p_i$ can dominate $p_{k+1}$. Since the assumption is false, Theorem \ref{theorem: MultiGreedyPruning} is true.
\end{proof}

Therefore, when $c_{dc}[p_{k+1}]$ is very low like falling into the last quarter, we can use Theorem \ref{theorem: MultiGreedyPruning} to do the validation instead of using the intersection. We can further terminate earlier when the distinct criteria is smaller than a threshold according to the following theorem:

\begin{theorem}
	\label{theorem: MultiGreedyPruning2}
	$p_{k+1}$ is not a skyline path $\Leftrightarrow r_{dc}[p_{k+1}] > k + 1 - \dfrac{k}{n-1}=k(1-\dfrac{1}{n-1})$.
\end{theorem}
\begin{proof}
	Because $r_{dc}[p_{k+1}]$ has the highest rank, then $p_{k+1}$'s ranks on other criteria cannot be higher. In other words, there are at most $k+1-r_{dc}[p_{k+1}]$ paths in each $P_i^{> m_i}$. Therefore, if $(k+1-r_{dc}[p_{k+1}])\times (n-1)< k$, then $\sum |P_i^{> m_i}|<k\Rightarrow |\bigcup_{i\in[1,n]} P_i^{\leq m_i}| < k$. 
\end{proof}

Although Theorem \ref{theorem: MultiGreedyPruning2} seems loose at the first glance, it becomes power when $k$ is big and $n$ is small. For instance, when $n$ is 4 and $k$ is 10,000, then when $r_{dc}[p_{k+1}]$ is larger than $10000\times(1-\dfrac{1}{4-1}=6667)$, we can prune $p_{k+1}$ safely.



\subsection{Multiple Hop Skyline Path Concatenation}
\label{subsec:Skyline_Multiple}
%In the previous section, we describe how to concatenate the skyline paths via one single hop. However, d
%During the construction and query answering, we have to determine the results from several hops at the same time. Obviously, the skyline paths from one hop could be dominated by results from others. Besides, it would be inefficient to generate all their skylines first and then reduce from them. Therefore, we provide a rectangle-based pruning method to further reduce the concatenation operations among the hops.

In the previous subsections, we have illustrated how to identify all the skyline paths from $s$ to $t$ when $h_i$ is the unique intermediate hop. However, the intersection of $s$' out-label and $t$'s in-label may contain multiple hops. In this case, the identified skyline paths via $h_i$ could be dominated by the skyline paths via other intermediate hops. Therefore, after we produce all the skyline paths via each intermediate hop, we need further validation on these path sets. Obviously, it is very time-consuming due to the large concatenation number and time complexity. Therefore, in this section, we introduce some pruning methods to screen the skyline paths via different hops before the actual concatenation to reduce total concatenation number. We first introduce the \textit{Rectangle Pruning} for \textit{2}-dimensional graph in Section \ref{subsubsec:Skyline_Multiple_Rectangle}, and then generalize it to $n$-Cube pruning for \textit{n}-dimensional graph in Section \ref{subsubsec:Skyline_Multiple_Cube}. %and return the optimal result of CSP for given CSP query ($s, t, C$). 

\begin{figure}[ht]
    \centering
    \includegraphics[width=2.3in]{CSPPruning.pdf}
    \caption{Multiple Skyline Rectangles and \textit{CSP} Query Rectangle (Shaded)}
    \label{fig:ConcatenationPruning}
\end{figure}

\subsubsection{Rectangle Pruning for 2D Graph}
\label{subsubsec:Skyline_Multiple_Rectangle}
Given two skyline path sets $P(s,h)$ and $P(h,t)$, according to Property \ref{lemma:FirstandLast}, $p_1^1$ and $p_m^n$ are the two end points and they can determine a rectangle $[w_1^1,w_m^n]\times [c_1^1, c_m^n]$  ($p_1^1$ as the top-left and $p_m^n$ as the bottom-right) such that all the other skyline paths must locate in it. Therefore, we can use this rectangle to approximate the skyline paths distribution of a hop without computing them. In other word, this rectangle is a \textit{MBR (Minimum Bounding Rectangle)} for all the skyline paths via $h$. For example in Figure \ref{fig:ConcatenationPruning}, suppose we have the skyline rectangles of six hops and each of them is identified with only two computations for the two endpoints. Among these end points, we find one with the smallest weight and another one with the smallest cost, then we can obtain a new \textit{hop rectangle} that guarantees the all the skyline results must be inside it (the shaded area formed by top-left of $h_2$ and the bottom-right of $h_3$). We only consider the rectangles of hops that intersect or inside \textit{query rectangle} as our final concatenated hops. For instance, as the rectangle $h_5$ and $h_6$ are outside the query rectangle, we can prune them directly. For $h_4$, we further consider the paths with weight less than $w(p_n.h_3)$. Finally, all the paths in $h_1$, $h_2$ and $h_3$ need actual concatenations. The detailed pruning procedure is described in Algorithm \ref{Algorithm:MultiHop}. The time complexity is $O(max|X_i|)$ as $max|X_i|$ is max size of $H$. 

For example, in the label assignment example of Section \ref{subsubsec::CSP2Hop_TD_Label}, we first compute three rectangles of the corresponding hops: $h_1:[6,11]\times [10,5]$; $h_5:[4,7]\times [6,5]$; $h_8:(2,3)$. Because $(2,3)$ dominates the other two rectangles, we prune $h_1$ and $h_5$ and return $(2,3)$ directly as the skyline path.



%To a set of skyline paths ($p_1.h_i,p_2.h_i,p_3.h_i,..,p_n.h_i$) via $h_i$, which are sorted by the weight in an ascending order. We can identify that $p_1$ must have the smallest weight and the largest cost, but $p_n$ has the largest weight and the smallest cost. If we map the two paths as points on the weight-cost coordinates, we can generate a bound rectangle based on the two points. The other paths must be the points that inside the rectangle.

%Hence, for $h_i$, we can represent it by the rectangle that contains all the skyline paths via it. The top left point is $p_1.h_i$, and the bottom right point is $p_n.h_i$. Therefore, instead of mapping all the skyline paths on multiple hops, we use different rectangles to represent each hop and the range of corresponding skyline paths. Suppose $p_1.h_i$ has the smallest weight, and $p_n.h_j$ has the smallest cost, we can ensure that the optimal result of CSP from $s$ to $t$ must locate in a bound rectangle which generated by $p_1.h_i$ and $p_n.h_j$, we define it as our query region. 

\begin{algorithm}[ht]
	\caption{Rectangle-based Hop Pruning}
	\label{Algorithm:MultiHop}
%	\footnotesize
	\LinesNumbered
	\KwIn{The Hop Set $H$ in \textit{LCA} of $s$ and $t$}%, Sorted Skyline Path Set $P(s,h_i)$ and $P'(h_i,t)$,$\forall h_i\in H$}
	\KwOut{Pruned hop set $H'$}
	$TL\leftarrow (\infty,0), BR\leftarrow(0,\infty)$;\algorithmiccomment{Two end-point}\\
	\ForEach{$h_i\in H$}{
	 $P(s,h_i) \leftarrow L(s)[h_i], P(h_i,t) \leftarrow L(t)[h_i]$\;
	 
	 $p_1^1 \leftarrow p_1(s,h_i) \oplus p_1(h_i,t)$;\algorithmiccomment{Top Left}\\
	 $p_m^n \gets p_m(h_i,t) \oplus p_n(h_i,t)$;\algorithmiccomment{Bottom Right}\\
	 \If{$p_1^1.w< TL.w$}
	 {
	    $TL	\leftarrow p_1^1$\;
	 }
	 \If{$p_m^n).c< BR.c$}
	 {
	    $BR\leftarrow p_m^n$\;
	 }

	 $Rectangle[h_i]\gets(p_1^1, p_m^n)$\;
	}

	$R\leftarrow (TL, BR)$\;
	\ForEach{$h_i\in H$}{
	    \If{$R$  $\cap Rectangle[h_i] \neq \phi$}{
	    $H'.insert(h_i)$
	    }
	}
	\Return $H'$\;
\end{algorithm}


%Suppose we have six intermediate hops from $h_1$ to $h_6$, the final skyline paths from $s$ to $t$ must in the dark bound rectangle which generated by $p_1.h_2$ and $p_n.h_3$. 

\subsubsection{$n$-Cube Pruning for n-Graph}
\label{subsubsec:Skyline_Multiple_Cube}

% 将hypercube通过convex hull形式表示->
%2D ->{(d_0,d_1) \in D^2| Min_di<=d_i<=Max_di} -> rectangle
%(n+1)D->{(d_0,d_1,...,d_n)\in D^{n}|Min_di<=d_i<=Max_di} ->hypercube

%Min_di 和max_di的确定
%对于一组skyline集合
%->找到在各个维度值最小的skyline集合 (最多n+1个) ->找出集合中各个维度最小的值作为下确界
%->找出集合中各个维度最大的值作为上确界

%对于每个hop,找到其上下确界确定凸包

%hypercube pruning-> 确定每个hop中,在各个维度值最小的skylines ->从而确定所有hops中各个维度值最小的skylines ->从而确定hypercube pruning的凸包

%筛选hops-> 各个hop凸包与hypercube pruning的凸包进行比较 -> 范围之外则排除该hop
%In 2D road networks, query rectangle pruning can efficiently reduce the hops considered. Thereby, the number of concatenations can be further reduced. 
Different from the 2D scenario, in the multi-dimensional road networks, such rectangles can not be found, as the Property \ref{lemma:FirstandLast} cannot hold for the concatenated skyline paths with over 2 criteria. This is caused by the fact that the path with the largest weight does not necessarily have the largest cost in each dimension. For instance in Table \ref{table:EG_skylines}, $p_5$ has the largest $w$ but it does not have the largest cost in any of the three cost dimensions. Therefore, we can only find a hop rectangle in each 2D subspace, i.e., hop rectangles based on all two criteria combinations. By intersecting the projection of these faces, we obtain a hypercube that encloses all the concatenated skyline paths. For better description of the pruning in $n$-graph, we first map the $n$-graph to a $n$-dimensional space: Given a $n$-dimensional graph $G(V,E)$ and $n$-dimensional space $D^n=\{d_0,d_1,...,d_{n-1}\}$, for arbitrary path $p$, we use dimension $d_0$ to describe the value of $w(p)$, and $d_i$ to describe the value of $c_i(p)$, where $i \in [1, n-1]$. Now we are ready to describe the $n$-Cubes.

%To enclose all the concatenated skyline paths in 3D, the querying space will become a cube including three query rectangles in different faces of the cube. We denote the cube in 3D as $3$-cube. When the dimensions keep increasing, the querying space will become a hypercube, which is difficult to describe by geometry. For instance, in a n-dimensional graph, the querying space can be a $n$-cube. In the following, we give the definition for $n$-cube.  


%\begin{definition}[Multi-Dimensional Space]
%   Given a $n$-dimensional graph $G(V,E)$ and $n$-dimensional space $D^n=\{d_0,d_1,...,d_{n-1}\}$, for arbitrary path $p$, we use dimension $d_0$ to describe the value of $w(p)$, and $d_i$ to describe the value of $c_i(p)$, where $i \in [1, n-1]$. 
%\end{definition}

\begin{definition}[Skyline Path Set Intervals]
\label{def:Skyline_Intervals}
	Given a path set $P_c$ and its corresponding space $D^n$, $\forall d_i\in D^n$, its lower-bound $Min(d_i)$ is the smallest value of all path $p\in P_c$ on dimension $d_i$. Similarly, its upper-bound $Max(d_i)$ is the largest value of all path on $d_i$. An interval $I_i=[Min(d_i), Max(d_i)]$ covers all the path values in $P_c$ on dimension $d_i$.
\end{definition}

\begin{definition}[$n$-Cube]
\label{def:n_cube}
 Given a path set $P_c$, a $n$-cube $\Gamma^n(P_c)=\{I_0,I_1,..,I_{n-1}\}$ covers all the skyline paths in $P_c$.
\end{definition}

We use the following \textit{supremum} and \textit{infimum} to assist the pruning:
\begin{definition}[$n$-Cube Supremum and Infimum]
For a $n$-cube $\Gamma^n$, its supremum $Sup[\Gamma^n(P_c)]$=$\{Max(d_0),$ $...,Max(d_{n-1})\}$ is a set that contains the upper-bounds of $P_c$ on each dimension, and its infimum $Inf[\Gamma^n(P_c)]=\{Min(d_0),...,Min(d_{n-1})\}$ is a set that contains the lower-bounds of $P_c$.
\end{definition}

For instance in Table $\ref{table:EG_skylines}$, there are five skyline paths in $P_c$. We use $d_0$ to denote skyline path values on criterion $w$, and $d_1$ to $d_3$ to denote the values on the criteria from $c_1$ to $c_3$. As the smallest value on $d_0$ is 2 and the largest on is 6, we can find a set $I_0=[2,6]$ to contain the five skyline path values on $d_0$. By the same token, we obtain $I_1=[3,7]$, $I_2=[7,10]$, and $I_3=[2,10]$. Therefore, we can identify a 4-cube $\Gamma^4(P_c)=\{[2,6], [3,7], [7,10], [2,10]\}$ for the example skyline paths. Note that this 4-cube can cover all skyline path values in table $\ref{table:EG_skylines}$. In addition, $Inf[\Gamma^4(P_c)]=\{2,3,7,2\}$ and $Sup[\Gamma^4(P_c)]=\{6,7,10,10\}$. Naturally, we have the following property:

\begin{property}
\label{property:n-cube}
    Given a set of $n$-dimensional skyline paths $P_c$, its $n$-cube $\Gamma^n(P_c)$ contains all the paths in $P_c$.
\end{property}

Similar to the 2D scenario, we first create the $n$-cube for each hop to approximate the concatenation result space. According to definition \ref{def:n_cube}, to identify a $n$-cube of hop $h_k$, we need to computing both the lowest bound and the highest bound on each dimension. Specifically , we compute the concatenated skyline path $p_{Min(d_i)}$ with the smallest value on dimension $d_i$. Suppose $p$ has the smallest value on $d_i$ in $P(s,h_k)$ and $p'$ has the smallest value on $d_i$ in $P(t,h_k)$. Then $Min(d_i)$ can be obtained by concatenating $p$ and $p'$. If $p_{Min(d_i)}$ is a unique path that has the smallest value on $d_i$, we can easily prove that $p_{Min(d_i)}$ must be a concatenated skyline path. Thus, the $d_i$ value of $p_{Min(d_i)}$ must be the lower-bound of $d_i$ for all the concatenated skyline paths. We can use the same way to compute the upper-bound by finding $Max(d_i)$ in both $P(s,h_k)$ and $P(t,h_k)$. However, different to the 2D case, we can not guarantee that the concatenated path with the largest value on $d_i$ is a $n$-dimensional skyline path. %such as $p_5$ in Table \ref{table:EG_skylines}.
Therefore, the obtained upper-bounds are actually looser than the actual bounds. For ease of presentation, we refer to $n$-cube of concatenated skyline path set via $h_k$ as $\Gamma(h_k)$, and $\Gamma(h_k)\supseteq \Gamma(P(s,h_k)\oplus P(h_k,t))$. Also, we refer to $Sup[\Gamma^n(h_k)]$ and $Inf[\Gamma^n(h_k)]$ as $Sup(h_k)$ and $Inf(h_k)$, if no special instructions on dimensions are needed. 

%As similar as the querying rectangle pruning on multiple hops, we can use a $n$-cube to enclose all skyline paths for each hop on $n$-dimensions.

\begin{figure}[ht]
    \centering
    \includegraphics[scale=0.3]{SupAndInf.png}
    \caption{Supremum and Infimum for Hops (left) and Supremum Shrinking( right)}
    \label{fig:SubAndInf}
\end{figure}

Because the $n$-cube is a hypercube, it is difficult to clearly demonstrate a range of skyline paths in an example plot like as the hop rectangle in 2D. Nevertheless, if we treat the dimensions as $x$-coordinates and supremum/infimum values on each dimension as $y$-coordinates, we are able to map a $n$-cube to a 2D plot in the form of two polylines. For instance, Figure \ref{fig:SubAndInf} (left) shows four $4$-cubes, each represented by two polylines with the same color. In the following, we discuss the $n$-cube pruning with the help of Figure \ref{fig:SubAndInf}.



\begin{property}
	\label{property:n-cube_dominance}
	\textbf{($n$-Cube Dominance)} Given any two $n$-cube $\Gamma_i$ and $\Gamma_j$, if $Sup[\Gamma_i]$ dominates $Inf[\Gamma_j]$, then $\Gamma_i$ dominates $\Gamma_j$ and all the paths in $\Gamma_j$ are also dominated by the paths in $\Gamma_i$ .
\end{property}

%We can observe that if there is a $n$-cube having the supremum over the infimum of $n$-cube $\Gamma_i$. All the paths enclosed by $\Gamma_i$ will be dominated. 
For example in Figure \ref{fig:SubAndInf}, the polyline $Sup(h_4)$ is over the supremum of other three $4$-cube. Therefore, all the paths in $\Gamma(h_4)$ have greater value on each dimension than the paths in other $4$-cubes. However, as the polylines of other three $4$-cubes are intersected with each other, we need further pruning method on them.

As discussed previously, the infimum of each estimated hop's $n$-cube $\Gamma(h_i)$ is fixed, but the supremum is loose. Therefore, it is promising to further prune more hops by shrinking the supremums, which could be achieved by concatenating the skyline paths on some hops earlier. For instance in Figure \ref{fig:SubAndInf}, if we first compute all the concatenated skyline paths on $h_1$, we can obtain a fixed $Sup(h_1)$, which is shrunken to the position in Figure \ref{fig:SubAndInf} (right). Thus, $\Gamma(h_2)$ can be pruned directly by $\Gamma(h_1)$. Thereby, it is important to determine an efficient concatenating order for the hops, which is defined as follows.

\begin{definition}[$n$-Cube Comparison]
	\label{def:n-Cube_Comparions}
	Given two of $n$-Cubes $\Gamma_i$ and $\Gamma_j$ that cannot dominate each other. We use $|Inf^{<}[\Gamma_i]|$ to denote the number of dimensions $Inf[\Gamma_i]$ is smaller, and $|Inf^<[\Gamma_j]|$ to denote $\Gamma_j$'s. Then we say $\Gamma_i < \Gamma_j$ if $|Inf^<[\Gamma_i]|>|Inf^<[\Gamma_j]|$. The draw of comparison can be settled by comparing the supremum. The further draw is settled by comparing infimum dimensions in the decreasing order, and the one with first smaller dimension lower-bound is smaller. 
\end{definition}

The intuition behind this order is that if a hop has lower infimum, it has higher change contain skyline paths. Especially, the hop with the lowest infimum must contain skyline paths. Moreover, a $n$-cube with a lower infimum has higher chance to prune more $n$-cubes after it shrinks. Based on this observation, we have the following order the $n$-cubes.

\begin{definition}[$n$-Cube Concatenation Priority]
	\label{def:Priority}
	Given a set of $n$-Cubes that cannot dominate each other, their concatenation order is the same as their increasing infimum order.
\end{definition}

%We first determine the order by infimum, if the infimum of a $n$-cube of a hop is lower in the coordinates, we increase the priority of concatenation on the former. 

%his is because  To determine whether a hop has lower infimum than other one, we just compare how many the lowest bound of the hop can be lower than the other hop. 
For instance, because all the lowest bounds of $Inf(h_1)$ are lower than $Inf(h_2)$, we need to concatenate skyline paths on $h_1$ before $h_2$. $\Gamma_1<\Gamma_3$ because $|Inf^{<}[\Gamma_1]|=|Inf^{<}[\Gamma_3]|$ but $|Sup^{<}[\Gamma_1]|>|Sup^{<}[\Gamma_3]|$. Finally, $\Gamma_3<\Gamma_2$ because $|Inf^{<}[\Gamma_3]|<|Inf^{<}[\Gamma_2]|$. Therefore, the three $4$-Cubes should be concatenated in the order of $\Gamma_1$, $\Gamma_3$, and $\Gamma_2$. It should be noted that this order can be change dynamically when any $n$-cube is pruned or when any supremum is fixed. The detailed procedure is shown in Algorithm \ref{Algorithm:n-cube_pruning}. %However, this method can not support all cases, such as $Inf(h_1)$ and $Inf(h_2)$, as $h_1$ has two the lowest bounds are lower than $h_2$ and two the lowest bounds are greater than $h_2$, we can not judge the priority by the rule above. If it is the case, we check the supremum of the two hops. If one hop has lower supremum than the other one, we increase the priority of concatenation on the former. As we can not determine a priority for the two hops in terms of the infimums, these two hops have no chance to prune each other. We prefer to select the one hop that is easier to get a lower supremum, which has higher chance to prune other hops.

%As same as the 2D case, we first find $n$-cube containing all the concatenated skyline paths on each hop.  (use constraints as supremums)

\begin{algorithm}[ht]
	\caption{$n$-Cube Hop Pruning}
	\label{Algorithm:n-cube_pruning}
%	\footnotesize
	\LinesNumbered
	\KwIn{The Hop Set $H$ in \textit{LCA} of $s$ and $t$}%, Sorted Skyline Path Set $P(s,h_i)$ and $P'(h_i,t)$,$\forall h_i\in H$}
	\KwOut{Skyline Paths Set $P_{s,t}$}
	$P_{s,t}\gets \phi$\;
	\ForEach{$h_i\in H$}
	{
		\ForEach{$d_j\in D^n$}
		{
			$Inf[\Gamma_i][j]\gets p_1(s,h_i).d_j+p_1'(h_i,t).d_j$\;
			$Sup[\Gamma_i][j]\gets p_n(s,h_i).d_j+p_m'(h_i,t).d_j$\;
		}
		$\Gamma_i\gets (Inf[\Gamma_i], Sup[\Gamma_i])$\;
	}
	$\hat{\Gamma}\gets $n-Cube-Sort($\{\Gamma_i\})$\;
	$Sup[\hat{\Gamma}]\gets [-1]\times n$\;
	\ForEach{$\Gamma_i\in \hat{\Gamma}$}
	{
		\If{$Sup[\hat{\Gamma}]$ dominates $Inf[\Gamma_i]$}
		{
			$Continue$\;
		}
		$P_{s,t}\gets Skyline(P_{s,t}, P(s,h_i)\oplus P(h_i,t))$\;
		\ForEach{$d_j\in D^n$}
		{
			\If{$Sup[\hat{\Gamma}< Max(P_{s,t}.d_j)$}
			{
				$Sup[\hat{\Gamma}\gets Max(P_{s,t}.d_j)$\;
			}
		}
	}
	\Return $P_{s,t}$\;
\end{algorithm}

Finally, the rectangle pruning in the 2D scenario can be viewed as a special case of the $n$-Cube pruning with $n=2$. Although its supremum is fixed initially, its performance can also be improved with the 2-Cube concatenation priority.
%On multiple hop skyline path concatenation, we should concatenate two skyline path sets on each intermediate hop. In the previous 2D case, we reduce the number of hops considered by defining a querying rectangle. In terms of Definition \ref{def:n_cube}, we can describe the querying rectangle of the concatenated skyline path set $P_c$ by $\Gamma^2(P_c)={I_1,I_2}$. For this rectangle, the $Min(d_0)$ of $I_1$ is the weight value of the top-left endpoint and the $Max(d_0)$ of $I_1$ is the weight value of the bottom-right endpoint. Furthermore, the $Min(d_1)$ of $I_1$ is the cost value of the bottom-right endpoint and the $Max(d_1)$ of $I_1$ is the cost value of the top-left endpoint. (Example?) 

%We can compute a set of paths with as infimums on different dimensions. We denote it as $P_{inf}=\{p_{Min(d_0)},p_{Min(d_1)},...,p_{Min(d_{n-1})}\}$. 

%For instance, in table \ref{table:EG_skylines}, we can find $P_{inf}=\{{p_1,p_2},p_4,p_3,p_1\}$. We first check $\{p_1,p_2\}$, the current largest supremum on $c_1$ is 4, $c_2$ is 10, $c_3$ is 3. Then, we check $p_4$, the largest supremum on $w$ is 5, and there are no update on $c_1$, $c_2$, and $c_3$. Next, we check $p_3$, 

\begin{figure*}[ht]
    \centering
    \includegraphics[width=6.8in]{ForestQuery.pdf}
    \caption{Constraint Shortest Path Query with Forest Labels}
    \label{fig:ForestQuery}
\end{figure*}

\subsection{Constraint Skyline Path Concatenation}
\label{subsec:Skyline_Constraint}
In this section, we further dig into the concatenation when the query constraints $\overline{C}$ are provided. Similar to the previous sections, we also first discuss the easier 2D case and then generalize it to the $n$ dimensional case.
\subsubsection{CSP Concatenation}
\label{subsec:Skyline_Constraint_Single}
We first deal with the \textit{CSP} query $q(s,t,C)$. As illustrated in Figure \ref{fig:ConcatenationPruning}, the query rectangle is further reduced to a smaller one by applying an upper-bound of $C$ (like the dotted area created by $C_3$). If $C$ is smaller than the lowest cost (like $C_1$), then the result is empty. If there exists one rectangle whose upper-left point is the only left most point in the query rectangle (like $C_2$ and $h_3$), we return this point directly. Otherwise, there must be some partial rectangles. We first find the most upper-left point in the query region and denote it as $p^*$ and use for the current best point ($w^*$ as its weight). Then for all the partial rectangles whose left boundary is larger than $w^*$, we can prune them directly (e.g., $h_4$ is pruned by $h_3$). After that, we enumerate the candidates in the remaining partial rectangles (like $h_1$) in a similar way like 
Algorithm \ref{Algorithm:GreedyConcatenation}. The difference is we only start testing when the sub-path's cost is smaller than $C$, and stop if either the current minimum weight is larger than $w^*$ or we obtain the first one whose cost is no larger than $C$. Traversal from multiple partial hops can run in parallel as they have the same termination condition and do not interfere each other. 

%For the query region, we can get the a interval of cost, which are [$C(p_n.h_j)$, C($p_1.h_i$)]. Given a CSP query ($s,t, C$), if $C \geq C(p_1.j_1)$, the optimal result of CSP is $p_1.h_i$. If $C \leq C(p_n.h_j)$, there is no result for the query. If $C$ intersects with the interval, we deal with the paths of query region in the following:
%\subsection{$n$-cube Pruning}

\subsubsection{MCSP Concatenation}
\label{subsec:Skyline_Constraint_Multi}
Different from the $n$-Cube in Section \ref{subsubsec:Skyline_Multiple_Cube}, the supremums that are larger than the constraint $\overline{C}$ can be replaced by  $\overline{C}$ during query answering. Besides, a $n$-Cube can be further pruned by the following property.

\begin{property}
	\label{Property:MCSP_Constraint}
	Given a $n$-Cube and a set of query constraints $\overline{C}$, $n$-Cube can be pruned if any of its infimum is larger than the corresponding cost.
\end{property} 

Then for the concatenation of each $n$-Cube, because the paths are concatenated in the distance-increasing order, we only need to concatenate the first one that satisfies $\overline{C}$ for each hop. Within each hop concatenation, the paths in the labels are also pruned when any of its cost does not satisfy $\overline{C}$. When have the first candidate, its distance can also be used to prune the remaining concatenations for other hops. 


\subsection{Forest Constraint Skyline Path Concatenation}
\label{subsec:Skyline_Forest}
\subsubsection{Rectangle Pruning for 2D Graph}
In this section, we present how to apply the above techniques to answer \textit{MCSP} with forest labels. The extended labels can use the methods in Section \ref{subsec:Skyline_Constraint} directly. As for the forest labels, we break it into three parts as shown in \mycolor{Figure \ref{fig:ForestQuery}}-(a): 1) from $s$ to its boundary $B_1$, 2) from $B_1$ to $B_2$, and 3) from $B_2$ to $t$. However, different from the previous query that needs concatenation, the skyline results of 1) and 3) can be retrieved from their sub-trees directly because their boundaries are all their ancestors. As for the boundaries results, we first obtain their rectangles, then obtain the approximate results from $s$ to $B_2$ by viewing each boundary in $B_1$ as a hop. For example in \mycolor{Figure \ref{fig:ForestQuery}}-(b), we get a candidate rectangle $\bar{R_1}$ from $s$ to $b'_1$ by pruning the multi-hop of $B_1$. By applying the same procedure to the boundaries $B_2$ in parallel, we can have a set of candidate rectangles as shown in \mycolor{Figure \ref{fig:ForestQuery}}-(c). After that, these rectangles will be ``enlarged and moved" to the new locations by viewing the first and last skyline paths of each $B_2$ to $t$ as a vector as shown in \mycolor{Figure \ref{fig:ForestQuery}}-(d). Then we have a final set of rectangles $\bar{R_t}$ that approximate the skyline path space from $s$ to $t$. Finally, we can apply the constraint $C$ to shrink the search to a small area (shaded area in \mycolor{Figure \ref{fig:ForestQuery}}-(e)) and conduct the actual concatenation similar as Section \ref{subsec:Skyline_Constraint}.

\subsubsection{n-Cube Pruning for n-Graph}

Similar to the 2D scenario, the query processing is the same as the steps in Figure \ref{fig:ForestQuery}-(a). However, the rectangle pruning will be displaced by $n$-cube pruning. When pruning from $s$ to $b_1'$, we construct an $n$-cube for each hop in $B_1$. According to Property \ref{property:n-cube_dominance}, we can prune the dominated $n$-cubes.Then, we approximate the concatenation result space from $s$ to $b_1'$ by updating an infimum and a supremum depending on the undominated $n$-cubes in $B_1$. If it is the case, we compare their infimums to find the lowest value on each dimension and compare their supremums to find the highest values. For example in Figure \ref{fig:ForestQuery}-(a), assume we are considering 4-cube. For the four hops in $B_1$, we have $\Gamma_1=\{[4,7],[5,7],[5,8],[1,9]\}$, $\Gamma_2=\{[3,6],[4,6],[4,7],[3,10]\}$,
$\Gamma_3=\{[8,12],[8,10],
[9,12],[10,13]\}$, and 
$\Gamma_4=\{[7,12],$\\$[8, 10],[9,14],[12,14]\}$
, $\Gamma_3$ and $\Gamma_4$ can be pruned in terms of Property \ref{property:n-cube_dominance}. By viewing the infimums and supermums of $\Gamma_1$ and $\Gamma_2$,
a new infimum from $s$ to $b_1'$ is $\{3,4,4,1\}$ and a new supremum is $\{7,7,8,10\}$. Afterwards, we enlarge the $n$-cube from $s$ to $b_1'$ by adding on the infimum and the supremum of the $n$-cube from $B_2$ to $t$. For instance, assume the $n$-cube from $b_1'$ to $t$ is $\Gamma_1'=\{[3,5],[2,6],[5,9],[1,4]\}$, we can get the concatenation result space from $s$ to $b_1'$ to $t$ as $n$-cube, which has the infimum $\{6,6,9,2\}$ and the supremum $\{12,13,17,14\}$. We can use the same way to compute the $n$-cubes from $s$ to $t$ via other hops in $B_2$. We prune the dominated $n$-cubes from $s$ to $t$ and update a infimum and a supremum as the concatenation result space from $s$ to $t$ by viewing the remaining $n$-cubes. We can apply the constraints $\overline{C}$ as the final supremum to shrink the $n$-cube from $s$ to $t$.

















==> CSP-H2H (VLDBJ)/SkylineQuery.tex <==
\section{Extension to Skyline Query}



%\subsection{Index Construction Using Skyline Preserved Graph}

%\subsection{Label with Distance and Cost Skyline}

==> CSP2Hop.tex <==
\section{CSP-2Hop Labeling}
\label{sec:CSP2Hop}
%In our case, except computing weighs, the 2 hop labeling have to consider another criterion which is cost. Therefore, the definition of constrained 2 hop labeling (CSP-2Hop) as follows:
%Unlike the 2-hop labeling in the single-criteria scenario whose label is only a distance value, the 
\textit{CSP-2Hop}'s label is a set of skyline paths. Specifically, for each vertex $u \in V$, it has a label set \mycolor{$L(u)=\{(v,P(u,v))\}$}, where $v$ is the hop vertex (\mycolor{$\{v\}$ is $u$'s hop set}) and $P(u,v)$ is the skyline path set. We use $L=\{(L(u)|\forall u \in V\}$ to denote the set of all the labels. If $L$ can answer all the \textit{CSP} queries in $G$, then we say $L$ is a \textit{CSP-2Hop} cover. Given a \textit{CSP} query $q(s,t,C)$, we first determine the common intermediate hop set \mycolor{$H=L(s) \cap L(t)$}. Then, we can find a set of candidate paths from $s$ to $t$ for validation by concatenating the skyline paths:
\begin{equation*}
\begin{aligned}
    P_c(H) &= \{P_c(h_i)|
    \{P(s,h_i)\oplus P(h_i,t)\}\}, \forall h_i\in H\\
    &=\{\{ p_j(w_j(s,h_i)+w_k(h_i,t),c_j(s,h_i)+c_k(h_i,t))\}\}\\
    &\forall p_j\in p(s,h_i) \wedge p_k\in p(h_i,t) 
\end{aligned}
\end{equation*}
where $\oplus$ is \textit{path concatenation} operator. Each $P_c(h_i)$ contains all the pairwise skyline concatenation results, and $P_c(H)$ is their union.
For instance, suppose the out-label of $s$ to $h$ has two skyline paths $p_1$ and $p_2$ and the in-label of $h$ to $t$ contains $p_3$ and $p_4$. Then we can obtain four paths from $s$ to $t$ by concatenating $p_1$ and $p_2$ interchangeably with $p_3$ and $p_4$, and obtain $P_c(h)=\{p_1\oplus p_3, p_1\oplus p_4, p_2\oplus p_3, p_2\oplus p_4\}$. 
%P_{candi}{\{i|p_i(w(s,h)+w(h,t),c(s,h)+c(h, t))|h \in H\}}$.

%\begin{definition}[Skyline Path Candidate]
%Suppose $h_i$ is an intermediate hop in $H$, we define $P(h_i)$ is the set of skyline paths from $s$ to $h_i$, $P’(h_i)$ is the set of skyline paths from $h_i$ to $s$. We denote $p_n.h_i$ is an arbitrary skyline path in $P(h_i)$, $p_m.h_i$ is an arbitrary skyline path in $P’(h_i)$. $p$ is a stitching path using a path in $P(h_i)$ and another path $P’(h_i)$. A set $P_{candi}$ has all the pair-wise connecting paths by paths in $P(h_i)$ and  $P’(h_i)$.
%\end{definition}


%the definition above need to be edited later. 

%In detail, for an arbitrary vertex $v$, we create its in-label set by storing skyline paths from other vertices to $v$, and also create its out-label set by storing skyline paths from $v$ to other vertices. To answer a query $q(s, t, C)$, we should first find the intermediate hop set $H$ by $L_{out}(s)$ and $L_{in}(t)$. For each intermediate hop $h$ in $H$, we combine the skyline paths from $s$ to $h$ with the skyline paths from $h$ to $t$.  We then generate a set of candidate path $P_{candi}$ for all intermediate hop in $H$. 

%We then identify the paths in candidate paths set $P_{candi}$ and ensure the set $P_{candi}$ must contain the result of the CSP query. To prove the existence of CSP in $P_{candi}$, the question can transfer to identify that $P_{candi}$ can contain all the skyline paths from $s$ to $t$. If all the skyline paths can be found in the set, the CSP also can be identified in the set of skyline paths.

As proved in Theorem \ref{the:Skyline}, the skyline paths between $s$ and $t$ are enough to answer any \textit{CSP} query, so we only need to prove the candidate set $P_c(H)$ covers all the skyline paths between $s$ and $t$. Firstly, we introduce the following lemma:  
%Due to each path in $P_{candi}$ is generated by two sub-skyline paths, we provide the theorem on the existence and corresponding proof as follows:

\begin{lemma}
\label{lemma:SkylineSubpath}
If a path $p$ is a skyline path, the sub-paths on $p$ are all skyline paths.
\end{lemma}
\begin{proof}
The proof of it can be found in \cite{storandt2012route}.
\end{proof}


\begin{theorem}
\label{the:HopSkyline}
$P_c(h)$ covers all the skyline paths from $s$ to $t$ that travel via hop $h$.
%Given an intermediate hop set $H$, let a set $P_1$ has all the skyline paths from vertex $s \in V$ to each vertex $h \in H$, and a set $P_2$ has all the skyline paths from $h$ to vertex $t \in V$. $P_{candi}$ has all the matching paths by $P_1$ and $P_2$. We ensure that all the paths in $P_{candi}$ must cover all the skyline paths from $s$ to $t$. 
\end{theorem}
\begin{proof}
Suppose $p^*$ is a skyline path from $s$ to $t$ via $h$ and $p^*\notin P_c(h)$. According to Lemma \ref{lemma:SkylineSubpath}, $p^*$'s sub-paths $p^*(s,h)$ and $p^*(h,t)$ are also skyline paths from $s$ to $h$ and from $h$ to $t$. If $p^*(s,h)\notin P(s,h)$ or $p^*(h,t)\notin P(h,t)$, it contradicts the definition that $P(s,h)$ contains all the skyline paths from $s$ to $h$, and similar for $P(h,t)$. Therefore, $P_c(h)$ covers all the skyline paths from $s$ to $t$ via $h$.
 %Initially, we ensure that if a path $p$ is a skyline path, all the sub-paths on $p$ are skyline paths{\cite{storandt2012route}}. For this reason, if we have a path $p$ from $s$ to $t$, and select a intermediate hop $h$ on $p$, $s-h$ path $p_1$  and $h-t$ path $p_2$ will also be the skyline paths. By the definition of 2 hop labeling in CSP, $L_{out}(s)$ can cover all the skyline paths from $s$ to $h$, $L_{in}(t)$ also have all the skyline paths from $h$ to $t$. Hence, we can conclude that $p_1$ and $p_2$ must exist in the labels of $s$ and $t$. This is, if $s$ to $t$ has skyline paths, the two sub-paths of each skyline path can be found in the labels of $s$ and $t$. We can identify that the combination set $P_{candi}$ must include all the skyline paths from $s$ to $t$.
\end{proof}


\iffalse
\begin{table*}
\centering
\caption{CSP-2Hop Labels}
\label{talbe:CSP-2Hop}
\scriptsize
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{} & \textbf{$v_3$} & \textbf{$v_7$} & \textbf{$v_{11}$} & \textbf{$v_{10}$} & \textbf{$v_9$}                                                 & \textbf{$v_4$}                                                        & \textbf{$v_1$}                                                                    & \textbf{$v_5$}                                                                   & \textbf{$v_8$}                                                        & \textbf{$v_{12}$}                                              \\ \hline
\textbf{$v_2$}     & (1, 1)         &                &                   &                   & (2, 5),(4, 3)                                                  & (1, 2)                                                                & (1, 2)                                                                            & (2, 4),(4, 3)                                                                    & (2, 4)                                                                & (3, 5),(7, 4)                                                  \\ \hline
\textbf{$v_3$}     &                &                &                   &                   & (1, 4),(6, 3)                                                  & (2, 3),(3, 2)                                                         & (2, 3)                                                                            & (3, 5),(4, 4)                                                                    & \begin{tabular}[c]{@{}l@{}}(2, 6),(3, 5)\\ (4, 4)\end{tabular}        & \begin{tabular}[c]{@{}l@{}}(3, 7),(4, 6)\\ (5, 5)\end{tabular} \\ \hline
\textbf{$v_6$}     &                & (2, 0)         &                   &                   &                                                                &                                                                       & (2, 0)                                                                            & (1, 1)                                                                           & \begin{tabular}[c]{@{}l@{}}(3, 5),(4, 4)\\ (5, 3)\end{tabular}        & (4, 2)                                                         \\ \hline
\textbf{$v_7$}     &                &                &                   &                   &                                                                &                                                                       & (3, 5),(4, 0)                                                                     & (1, 3),(3, 1)                                                                           & (3, 3)                                                                & (2, 2)                                                         \\ \hline
\textbf{$v_{13}$}  &                &                & \begin{tabular}[c]{@{}c@{}}(2, 3)\\(5, 2)\end{tabular}     & \begin{tabular}[c]{@{}c@{}}(3, 5)\\(4, 0)\end{tabular}     & \begin{tabular}[c]{@{}c@{}}(4, 9),(5, 6)\\ (6, 1)\end{tabular} & \begin{tabular}[c]{@{}c@{}}(4, 9),(5, 7)\\ (6, 4),(9, 2)\end{tabular} & \begin{tabular}[c]{@{}l@{}}(6, 13),(7, 11)\\ (8, 8),(9, 6)\\ (12, 5)\end{tabular} & \begin{tabular}[c]{@{}l@{}}(5, 11),(6, 9)\\ (7, 6),(8, 5)\\ (10, 4)\end{tabular} & \begin{tabular}[c]{@{}l@{}}(3, 7),(4, 5)\\ (5, 2)\end{tabular}        & \begin{tabular}[c]{@{}l@{}}(2, 6),(3, 4)\\ (6, 3)\end{tabular} \\ \hline
\textbf{$v_{11}$}  &                &                &                   & (1, 2)            & (3, 3)                                                         & (3, 4)                                                                & \begin{tabular}[c]{@{}l@{}}(5, 8)\\ (7, 3)\end{tabular}                           & \begin{tabular}[c]{@{}l@{}}(4, 6),(5, 5)\\ (6, 4)\end{tabular}                   & (2, 2)                                                                & (1, 1)                                                         \\ \hline
\textbf{$v_{10}$}  &                &                &                   &                   & (2, 1)                                                         & (2, 4),(5, 2)                                                         & \begin{tabular}[c]{@{}l@{}}(4, 8),(6, 7)\\ (7, 6),(8, 5)\end{tabular}             & \begin{tabular}[c]{@{}l@{}}(3, 6),(4, 5)\\ (6, 4)\end{tabular}                   & (1, 2)                                                                & (2, 3)                                                         \\ \hline
\textbf{$v_9$}     &                &                &                   &                   &                                                                & (2, 4),(3, 1)                                                         & (3, 7),(5, 5)                                                                     & (3, 6),(4, 5)                                                                    & (1, 2)                                                                & (2, 3)                                                         \\ \hline
\textbf{$v_4$}     &                &                &                   &                   &                                                                &                                                                       & (2, 4),(4, 3)                                                                     & (1, 2)                                                                           & (1, 2)                                                                & (2, 3)                                                         \\ \hline
\textbf{$v_1$}     &                &                &                   &                   &                                                                &                                                                       &                                                                                   & (2, 2),(3, 1)                                                                    & \begin{tabular}[c]{@{}l@{}}(3, 6),(5, 5)\\ (6, 4),(7, 3)\end{tabular} & (4, 7),(6, 2)                                                  \\ \hline
\textbf{$v_5$}     &                &                &                   &                   &                                                                &                                                                       &                                                                                   &                                                                                  & (2, 4),(3, 3)                                                         & \begin{tabular}[c]{@{}l@{}}(3, 5),(4, 4)\\ (5, 3)\end{tabular} \\ \hline
\textbf{$v_8$}     &                &                &                   &                   &                                                                &                                                                       &                                                                                   &                                                                                  &                                                                       & (1, 1)                                                         \\ \hline
\textbf{$v_{12}$}  &                &                &                   &                   &                                                                &                                                                       &                                                                                   &                                                                                  & (1, 1)                                                                &                                                                \\ \hline
\end{tabular}
\end{table*}
\fi

\begin{table}[]
\centering
\caption{Partial CSP-2Hop Labels}
\label{talbe:CSP-2Hop}
\scriptsize
\scalebox{0.75}{
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Ancestors} & \textbf{$v_4$} & \textbf{$v_1$} & \textbf{$v_5$} & \textbf{$v_8$}                                                        & \textbf{$v_{12}$}                                              \\ \hline
\textbf{$v_7$}     & -              & (3, 5),(4, 0)  & (1, 3),(3, 1)         & (3, 3)                                                                & (2, 2)                                                         \\ \hline
\textbf{$v_9$}     & (2, 4),(3, 1)  & (3, 7),(5, 5)  & (3, 6),(4, 3)  & (1, 2)                                                                & (2, 3)                                                         \\ \hline
\textbf{$v_4$}     & -              & (2, 4),(4, 3)  & (1, 2)         & (1, 2)                                                                & (2, 3)                                                         \\ \hline
\textbf{$v_1$}     & -              & -              & (2, 2),(3, 1)  & (3, 6),(5, 5) (6, 4),(7, 3) & (4, 7),(6, 2)                                                  \\ \hline
\textbf{$v_5$}     & -              & -              & -              & (2, 4),(3, 3)                                                         & (3, 5),(4, 4) (5, 3) \\ \hline
\textbf{$v_8$}     & -              & -              & -              & -                                                                     & (1, 1)                                                         \\ \hline
%\textbf{$v_{12}$}  & -              & -              & -              & (1, 1)                                                                & -                                                              \\ \hline
\end{tabular}}
\end{table}


Next we need to prove the union of all the hops $h\in H$ covers all the skyline paths between $s$ and $t$. Because our 2-hop labeling is based on the graph cut, we only need to prove the following theorem:
\begin{theorem}
\label{the:CSP-2Hop}
If the hop set $H$ is the set of cuts between $s$ and $t$, then $P_c(H)=\bigcup_{h_i\in H} P_c(h_i)$ covers all the skyline paths from $s$ to $t$.
\end{theorem}
\begin{proof}
Similar to Theorem \ref{the:HopSkyline}, we also prove it with contradiction. Suppose $p^*$ is a skyline path and $p^*\notin P_c(H)$. Because $H$ is the graph cut set, $p^*$ has to travel through one of the cut vertex $h_i\in H$, which has a candidate set $P_c(h_i)$. However, $p^*\notin P_c(h_i)$ contradicts with Theorem \ref{the:HopSkyline}. So every skyline path from $s$ to $t$ exists in $P_c(H)$.
\end{proof}

In summary, our \textit{CSP-2Hop} is able to answer any \textit{CSP} query with label concatenation. 


\subsection{Index Structure}
\label{subsec:CSP2Hop_Index}
Our \textit{CSP-2Hop} is based on the \textit{Tree Decomposition} \cite{robertson1986graph,ouyang2018hierarchy}, which maps a graph into a tree structure with each tree node corresponding to a vertex and the graph cut information is captured by its ancestors:

\begin{definition}[Tree Decomposition]
\label{def:TreeDecomposition}
Given a graph $G$, its tree decomposition $T$ is a rooted tree in which each node $X\in V$ is a subset of $V$. $T$ has the following tree properties:
\begin{enumerate}
\item $\bigcup_{X_i\in V}X_i=V$;
\item $\forall (u, v)\in E, \exists X_i$ such that $\{u, v\}\subseteq X_i$;
\item $\forall v\in V$, the set $\{X|v\in X\}$ forms a subtree of $T$.
\end{enumerate}
\end{definition}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=2in]{Tree.pdf}
    \caption{Tree Decomposition Example}
    \label{fig:Tree Decomposition}
\end{figure}

For instance, Figure \ref{fig:Tree Decomposition} shows the tree decomposition of the example graph in Figure \ref{fig:ExampleGraph}. The first vertex in each tree node is its representative vertex. %Depending on if the tree nodes have an ancestor/descendent relation not, 
This structure has a \textit{Cut Property} that can be used to assign labels: $\forall s,t\in V$ and $X_s,X_t$ are their corresponding tree nodes without an ancestor/descendent relation, their cuts are in their \textit{lowest common ancestor (LCA)} node \cite{chang2012exact}, \mycolor{which is the lowest tree node that has both $X_s$ and $X_t$}. For example, the tree nodes of $v_2$ and $v_7$ are $X_2$ and $X_7$, and their \textit{LCA} is $X_{1}=\{v_{1},v_5,v_8,v_{12}\}$. Then these four vertices form a cut between $v_2$ and $v_7$. If $s$ is $t$'s descendant, then $t$ can be viewed as a cut between itself and $s$. Therefore, the \textit{LCA} of a vertex pair contains all the cuts between them. 
%2) \textit{Ancestor Property}: $\forall X_v\in T_G, X_u(u\in X_v\{v\})$ is an ancestor of $X_v$ in $T_G$. This can also be easily checked in Figure \ref{fig:Tree Decomposition}. The ancestor property 
Accordingly, we assign labels to a vertex with all its ancestors in $T_G$. It should be noted that the vertices in each tree node are also in its label because of the \textit{Ancestor Property}: $\forall X_v\in T_G, X_u(u\in X_v\backslash\{v\})$ is an ancestor of $X_v$ in $T_G$. For example, $v_6$ has labels of $\{v_7,v_1,v_5,v_8,v_{12}\}\supseteq \{v_1,v_5,v_7\}$. The detailed labels are shown in Table \ref{talbe:CSP-2Hop}, with the rows being the vertices and columns being the hops. Some cells have several values because they are skyline paths. \mycolor{The details of the index computation will be discussed in Section \ref{subsec:Construction}}. The following theorem proves the correctness of the labels:
\begin{theorem}
\label{the:LabelCorrectness}
The above procedure creates a \textit{CSP-2Hop}.
\end{theorem}
\begin{proof}
Because the labels assigned by the above procedure contains all the cuts between every vertex pair, it is a \textit{CSP-2Hop} according to Theorem \ref{the:CSP-2Hop}.
\end{proof}

\subsection{Query Processing}
\label{subsec:CSP2Hop_Query}
%To  solve the CSP queries using the CSP-2hop index, the naive solution for the CSP from $s$ to $t$ as follows: First, we generate the set $P_{candi}$ by connecting the skyline paths in the out label of $s$ to $h$ and the skyline paths in the in label of $h$ to $t$. Afterward, we screen out the paths with costs less than $C$ from $P_{candi}$. Then, we select the path with minimum weight as our output. 

Given a \textit{CSP} query $q(s,t,C)$, we can answer it with the \textit{CSP-2Hop} in the same way like the single-criteria scenario: Firstly, we generate the hop set $H=L(s) \cap L(t)=\{h|h\in X(LCA(s,t)\}$ by retrieving the vertices in the \textit{LCA} of $s$ and $t$, \mycolor{where \textit{LCA}$(s,t)$ returns the \textit{LCA} of $s$ and $t$}. Then for each $h_i\in H$, we compute $P_c(h_i)$ by $P(s,h_i)\oplus P(h_i,t)$. By taking the union of all $P_c(h_i)$, we obtain the candidate set $P_c(H)$. During the concatenation, we maintain the current optimal result (i.e., the shortest one satisfying the constraint $C$) and keep updating it. Finally, after all the candidates are generated and validated, we return the optimal one as the \textit{CSP} result.

However, unlike the 2-hop labeling of the single-criteria case where only $|H|$ times of adding is needed, the concatenation of the skyline paths makes hop computation much more time-consuming. Suppose the label of $s$ to $h$ has $m$ skyline paths and the label of $h$ to $t$ has $n$ skyline paths. Then for each intermediate hop, we have to compute $mn$ times, and the total time complexity grows to $O(mn|H|)$ instead of $O(|H|)$. 

For example, given a query $q(v_9,v_7,6)$, the \textit{LCA} of $v_9$ and $v_7$ in the tree is $X_1$, and it contains vertices $H=\{v_1,v_5,v_8,v_{12}\}$. For hop $v_1$, $L(v_9)[v_1]=\{(3,7),(5,5)\}$ and $L(v_7)[v_1]=\{(3,5),(4,0)\}$. Therefore, we can get four candidates $P_c(v_1)=\{(6,12),(7,7),(8,10),(9,5)\}$. Only $(9,5)$ has a cost smaller than $6$, so $(9,5)$ is the current best result. For hop $v_5$, we can get candidates $P_c(v_5)=\{(4,9),(5,6),(6,7),\\(7,4)\}$. Then $(5,6)$ replaces $(9,5)$ as it has smaller weight and meet the constraint condition as well. For hop $v_8$, we can get candidates $P_c(v_8)=\{(4,5)\}$, and the current best result is updated to $(4,5)$. Finally, for hop $v_{12}$, we obtain the candidate $P_c(v_{12})=\{(4,5)\}$, which is equal to the current best result. The final result is $(4,5)$. As shown in this example, although only 4 hops are needed, we actually run 10 path concatenation operations. Therefore, pruning over this large amount of computation is crucial to the query performance and we will elaborate it in Section \ref{sec:Skyline}.

\subsection{CSP-2Hop Construction}
\label{subsec:Construction}
The index construction is made up of two phases: a bottom-up \textit{Skyline Tree Decomposition} that gathers the skyline shortcuts, creates the tree nodes and forms the tree, and a top-down \textit{Skyline Label Assignment} that populates the labels with query answering, \mycolor{as shown in Algorithm \ref{Algorithm:Construction}}. It should be noted that both of these two phases do not involve the expensive skyline path search and only use the skyline path concatenation.

\begin{algorithm}[ht]
	\caption{\mycolor{CSP-2Hop Construction}}
	\label{Algorithm:Construction}
	\scriptsize
	\LinesNumbered
	\KwIn{Graph $G(V,E)$}
	\KwOut{CSP-2Hop Labeling $L$}
	\mycolor{
	\While{$v\in V$ has the minimum degree and $V\neq \phi$}
	{
		$X_v=N(v)$, $r(v)\leftarrow$ Iteration Number\Comment{Tree Node Contraction}\\
		\For{$(u,w)\leftarrow N(v)\times N(v)$}
		{
			$P(u,w)\leftarrow Skyline(p(u,v)\oplus p(v,u), (u,w))$\;
			$E\leftarrow E\cup (P(u,w))$, $V\leftarrow V-v$, 	$E\leftarrow E-(u,v)-(v,w)$\;
		}
	}
	\For{$v$ in $r(v)$ increasing order}
	{
		$u\leftarrow min\{r(u)|u\in X(v)\}, X_v.Parent\leftarrow X_u$\Comment{Tree Formation}
	}
	$X_v\leftarrow$ Tree Root, $Q.insert(X_v)$\Comment{Label Assignment}\\
	\While{$X_v\leftarrow Q.pop()$}
	{
		\For{$u\in \{u|X_u$ is ancestor of $X_v\}$}
		{
			$P(v,u))\leftarrow Skyline(P(v,w)\oplus P(w,u)), \forall w\in X_v$\;
			$L(v)\leftarrow{(u,P(v,u))}$\;
		}
		$Q.insert(X_u.children)$, $L\leftarrow L\cup L(v)$\;
	}	
	}
	
\end{algorithm}

%\subsubsection{Skyline Tree Decomposition}
%\label{subsec::Construction_TD}
%The skyline tree decomposition is made up of two steps: \textit{node contraction} that forms the tree nodes and \textit{tree construction} that organizes these nodes into a tree.

\subsubsection{Skyline Tree Node Contraction}
\label{subsubsec::CSP2Hop_TD_Contraction}
We contract the vertices in the degree-increasing order. For each $v\in V$, we add a skyline shortcut $p'(u,w)$ to all of its neighbor pairs $(u,w)$ by $p(u,v)\oplus p(v,w)$. If $(u,w)$ does not exist, then we use $p'_s(u,w)$ as its skyline path $p(u,w)$ directly. Otherwise, we compute the skyline of $p(u,w)$ and $p'(u,w)$ in a linear time sort-merge way, \mycolor{which sorts the two path sets based on $w$ first and obtain the new skyline paths by comparing them in the distance-increasing order}. After that, a tree node $X(v)$ is formed with $v$ and its neighbors $N(v)$, and all their corresponding skyline paths from $v$ to $N(v)$. The tree node $X(v)$ is assigned an order $r(v)$ according to the order when $v$ is contracted. After contracting $v$, $v$ and its edges are removed from $G$ and the remaining vertices' degree are updated. Then we contract the remaining vertices in this way until none remains. \mycolor{The time complexity of the contraction phase is $O(|V|(max(|X_i|)^2\times w^2_{max}\log w^2_{max}+\log |V|))$, where $max(|X_i|)$ is the tree width, $w_{max}$ is the longest edge distance that determines the worst case of skyline number, and $w^2_{max}\log w^2_{max}$ is concatenation.}

We use the graph in Figure \ref{fig:ExampleGraph} as the example. Firstly, we contract $v_2$ with $N(v_2)=\{v_1,v_3,v_4\}$. Because there is no edge between $v_1$ and $v_3$, we add a shortcut $(v_1,v_3)$ with  by $w=w(v_1,v_2)+w(v_2,v_3)=2$ and $c=c(v_1,v_2)+c(v_2,v_3)=3$. Similarly, there is no edge between $v_1$ and $v_4$, so we add a new edge $(v_1,v_4)$ with $w=w(v_1,v_2)+w(v_2,v_4)=2$ and $c=c(v_1,v_2)+c(v_2,v_4)=4$. As for $v_4$ and $v_3$, we first generate a shortcut by $p(v_4,v_2)\oplus p(v_2,v_3)=(2,3)$. Then because there already exists an edge $(3,2)$ from $v_4$ to $v_3$, we compute the new skyline paths between the shortcut and the edge, and get the new skyline paths $p(v_4,v_3)=\{(3,2),(2,3)\}$. After that, we remove $v_2$ from the graph, leaving $v_1$'s degree changed to 4, $v_4$'s degree remaining 5, and $v_3$'s degree remaining 3. We also obtained a tree node $X(v_2,v_3,v_1,v_4)$ with the skyline paths from $v_2$ to $N(v_2)$ and order $r(v_2)=1$. This procedure runs on with the next vertex with the smallest degree. When all the vertices finished contraction, we have an order of $\left<v_2,v_3,v_6,v_7,v_{13},v_{11},v_{10},v_9,v_4,v_1,v_5,v_8,v_{12}\right>$.


%We can have the following in sights in terms of the properties above: First, every node in $T_G$ must have at least one vertex, and every vertex in G can exist in more than one tree node. Moreover, arbitrary edge $(u, v)$  can embed in one or more tree nodes, but it is not means any two vertices u, v in a tree node must be an edge. In addition, the node $X$ can acts as separator, if we remove vertices in X from its subtree resulting in the remaining vertices in the subtree are independent.

%We can describe a tree decomposition by its treewidth and treeheight. The definition is:

%\begin{definition}[Treewidth and Treeheight]
%Given a tree decomposition $T_G$, The treewidth of $T_G$ is $max_{X\in T_G} |X|-1$. The treeheight of $T_G$ is the maximum depth from the leaves to the root of $T_G$. 
%\end{definition}

\subsubsection{Skyline Label Assignment}
\label{subsubsec::CSP2Hop_TD_Label}
It should be noted the obtained tree preserves all the skyline path information of the original graph because every edge's information are preserved in the shortcuts. In fact, we can view it as a \textit{superset} of the \textit{CSP-CH} result. Therefore, we can assign the labels with skyline search on this tree directly. However, it would be very time-consuming as the \textit{Sky-Dijk} is much slower than \textit{Dijkstra}'s. To this end, we use the top-down label cascading method that takes advantages the existing labels with query answering to assign labels to the new nodes.

Specifically, a label $L(u)$ stores all the skyline paths from $u$ to its ancestors. Therefore, we start from the root of the tree to fill all the labels. For root itself, it has no ancestor so we just skip it. Next for its child $u$, because the root is the only vertex in $X(u)$ other than $u$, we add the root to $u$'s label. Then for any tree node $X(v)$, it is guaranteed that all its ancestors have obtained their labels. Then for any of its ancestor $a_i$, we compute its skyline paths by taking the skyline paths from  $\{p(v,u)\oplus p(u,a_i)| \forall u\in X(v)$\}. \mycolor{The time complexity of the label assignment phase is $O(|V|(\log|V| + max(|X_i|)\times h \times w^2_{max}\log w^2_{max}))$, where $h$ is the tree height. The space complexity of the labels is $O(h\times |V|\times w_{max})$.}

% with the \textit{multiple skyline path concatenation} described in Section \ref{subsec:Skyline_Multiple}. 

For example in Figure \ref{fig:Tree Decomposition}, suppose we have already obtained the labels of $X_1, X_5, X_8$, and $X_{12}$, and we are computing the labels of $X(v_4)$, which has an ancestor set of $\{v_{12}, v_8, v_5, v_1\}$. We take the computation of $L(v_4)[v_{12}]$ as example. $X_4$ has three vertices $\{v_1,v_5,v_8\}$ apart from $v_4$, so we compute the skyline paths via these tree hops. To show the process clearly, we do not apply the pruning first.
\begin{equation*}
	\scriptsize
    \begin{aligned}
        P_c(h_1)&=p(v_4,v_1)\oplus p(v_1,v_{12})
        =\{(2,4),(4,3)\}\oplus\{(4,7),(6,2)\}\\
        &=\{(6,11),(8,6),(8,10),(10,5)\}\\  
        P_s(h_1)&=\{(6,11),(8,6),(10,5)\}\\
    %\end{aligned}
%\end{equation*}
%\begin{equation*}
    %\begin{aligned}
        P_c(h_5)&=p(v_4,v_5)\oplus p(v_5,v_{12})
        =\{(1,2)\}\oplus \{(3,5),(4,4),(5,3)\}\\
        &=\{(4,7),(5,6),(6,5)\}\\
        P_s(h_5)&=\{(4,7),(5,6),(6,5)\}\\
    %\end{aligned}
%\end{equation*}
%\begin{equation*}
    %\begin{aligned}
        P_c(h_8)&=p(v_4,v_8)\oplus p(v_8,v_{12})
        =\{(1,2)\}\oplus\{(1,1)\}=\{(2,3)\}\\
        P_s(h_8)&=\{(2,3)\}
    \end{aligned}
\end{equation*}

Because $(2,3)$ dominates all the others, we put $(2,3)$ into the label of $L(v_4)[v_{12}]$. %If we use the \textit{query rectangle} pruning, we first compute three corresponding rectangles: $h_1:(6,11)\times (10,5)$; $h_5:(4,7)\times (6,5)$; $h_8:(2,3)$. Because $(2,3)$ dominates the other two rectangles, we prune $h_1$ and $h_5$ and return $(2,3)$ directly as the skyline path.
The correctness of the label assignment procedure can be easily proved by induction. As the label values are essentially the query results using the existing labels of the ancestors, the results are correct as long as the ancestors' labels are correct. The labels are populated in the cascading way, and thus the correctness is naturally guaranteed. Therefore, the resulting label set is a \textit{CSP-2Hop}.
 
 \subsection{Path Retrieval}
\mycolor{To retrieve the path, we need to preserve intermedia vertex in the labels. Specifically, during the \textit{Tree Node Contraction} phase, we need store the contracted in each skyline path in each shortcut. During the path retrieval, suppose one of the skyline results is the concatenation of $s\rightarrow h$ and $h\rightarrow t$, then they are actually two shortcuts so we only need to insert the intermediate vertices recursively until all no shortcut remains to recover the original path.}






==> Construction.tex <==
\section{CSP-2Hop Construction}
\label{sec:Construction}
The index construction is made up of two phases: a bottom-up \textit{Skyline Tree Decomposition} that gathers the skyline shortcuts, creates the tree nodes and forms the tree using the concatenation discussed in Section \ref{subsec:Skyline_Full}, and a top-down \textit{Skyline Label Assignment} that populates the labels with query answering discussed in Section \ref{subsec:Skyline_Multiple}. It should be noted that both of these two phases do not involve the expensive skyline path search and only use the skyline path concatenation.

%\begin{figure}[ht]
%    \centering
%    \includegraphics[scale=0.5]{example_cutting.png}
%    \caption{}
%    \label{fig:example_cutting.png}
%\end{figure}

%We can thus apply cutting set on two skyline path sets, which shown in Figure \ref{fig:example_cutting.png}. The definition are in the following: 

%\begin{definition}[cutting set]
%Suppose all the skyline paths in $P(h_i)$ and $P'(h_i)$ are sorted by weight with an ascending order, $c_1$ is a cutting set for $P(h_i)$, which includes $x_1$ skyline paths from $p_1$ to $p_{x_1}$, where $0 \leq x_1 \leq m$. $c_2$ is a cutting set for $P'(h_i)$, which includes $x_2$ skyline paths from $p'_1$ to $p_{x_2}$, where $0 \leq x_2 \leq n$. In $c_1$, we must ensure that the weight of the last skyline path $W(p_{x_1}) \leq W(p'_{{x_2}+1})$. In $c_2$, we must guarantee $W(p'_{x_2}) \leq W(p'_{{x_1}+1})$. Therefore, all paths on the left of both $c_1$ and $c_2$ have smaller weight than the paths on the right of $c_1$ and $c_2$. 
%\end{definition}

%In order for the condition of cutting set to be true, when we generate cutting set for $P(h_i)$ and $P'(h_i)$, we need the principles in the following:

%\begin{enumerate}
%\item Find the last path $p_{x_1}$ in $c_1$ and the last path $p'_{x_2}$ in $c_2$. If $W(p_{x_1}) \geq W(p'_{{x_2}+1})$,  we move $p_{x_1}$ out of $c_1$ and move $p_{{x_2}+1}$ into $c_2$. When $c_1$ has only one path, just  move one path into $c_2$.
%\item If $W(p_{x_2}) \geq W(p'_{{x_1}+1})$,  we move $p_{{x_1}+1}$ into $c_1$ and move $p_{x_2}$ out of $c_2$. When $c_2$ has only one path, just  move one path into $c_1$.
%\item Repeat step 1 and step 2 until all the paths on the left of $c_1$ and $c_2$ have smaller weight than the paths on the right of $c_1$ and $c_2$.
%\end{enumerate}

%Hence, we propose a way to connect skyline paths in two sorted sets $P(h_i)$ and $P'(h_i)$ by means of cutting set. 

%In Figure \ref{fig:example_cutting.png}, suppose $h_i$ is the only intermediate hop from $s$ to $t$. In the basis of corollary \ref{corollary 2}, we can confirm the first $s-t$ skyline path $p_1^1$, which has the lowest weight and highest cost, by connecting $p_1$ in $P(h_i)$ and $p'_1$ in $P'(h_i)$. Afterward, we generate cutting set $c_1$ for $P(h_i)$ and cutting set $c_2$ for $P'(h_i)$. In current, $c_1$ and $c_1$ have $p_1$ and $p'_1$, respectively. Then, we compare the weight between $p_1$ and $p'_2$, if $W(p_1) \geq W(p'_2)$, thus $W(p'_1) \leq W(p_2)$, we add $p'_2$ into $c_2$. As $c_1$ only has one path, we skip the operation of moving for $c_1$. (rewrite later)




%\subsection{Labeling Approach}
%Given a road network $G(V,E)$, tree decomposition $T_G$ can be built based on the concept of a vertex cut, which is defined as follows\cite{ouyang2018hierarchy}: 

%\begin{definition}[Vertex Cut]
%Given a road network $G(V,E)$, a subset of vertices $\Gamma \subset V$ is a vertex cut of $G$ if $G$ can be partitioned into several connected components by removing all the vertices in $\Gamma$. A set $\Gamma$ is the vertices cut of vertices $u$ and $v$ if $u$ and $v$ are in different components partitioned by removing $\Gamma$ from $G$.
%\end{definition}

%Therefore, if vertices $s$ and $t$ have a vertex cut $\Gamma$, we can infer that every path from $s$ to $t$ must via at least one vertex in $\Gamma$.
%By the property 3 of Tree Decomposition, if $s$ in node $X(s)$ and $t$ in node $X(t)$ are located at different sub-trees, we can regard the lowest common ancestor (LCA) of $X(s)$ and $X(t)$ as a vertex cut of $s$ and $t$ in $G$.

%Hence, in CSP-2hop index, for a CSP query ($s, t, C$), we treat the LCA of $s$ and $t$ in $T_G$ as the intermediate hop set $H$, each vertex in $H$ will be one intermediate hop. Hence, if we can pre-compute all the skyline paths from $s$ to each vertex in $\Gamma$ and the skyline paths from such vertices in $\Gamma$ to $t$, by using the query processing method of CSP-2hop index, we can further obtain a set of skyline paths via different vertices in $\Gamma$ and return the optimal result of CSP with the cost less than $C$. Furthermore, to answer CSP queries with any two vertices, we expect to know ahead of time all the skyline paths from each vertex in an arbitrary node $X(n)$ in $T_G$ to each vertex in every ancestor node of $X(n)$.   

\subsection{Skyline Tree Decomposition}
\label{subsec::Construction_TD}
The skyline tree decomposition is made up of two steps: \textit{node contraction} that forms the tree nodes and \textit{tree construction} that organizes these nodes into a tree.

\subsubsection{Skyline Tree Node Contraction}
\label{subsubsec::Construction_TD_Contraction}
We contract the vertices in the degree-increasing order. For each $v\in V$, we add a skyline shortcut $p'(u,w)$ to all of its neighbor pairs $(u,w)$ by $p(u,v)\oplus p(v,w)$. If $(u,w)$ does not exist, then we use $p'_s(u,w)$ as its skyline path $p(u,w)$ directly. Otherwise, we compute the skyline of $p(u,w)$ and $p'(u,w)$ in a linear time sort-merge way because the skyline paths produced by Algorithm \ref{Algorithm:GreedyConcatenation} are ordered by weight. After that, a tree node $X(v)$ is formed with $v$ and its neighbors $N(v)$, and all their corresponding skyline paths from $v$ to $N(v)$. The tree node $X(v)$ is assigned a order $r(v)$ according to the order when $v$ is contracted. After contracting $v$, $v$ and its edges are removed from $G$ and the remaining vertices' degree are updated. Then we contract the remaining vertices in this way until none remains. 

We use the graph in Figure \ref{fig:ExampleGraph} as the example. Firstly, we contract $v_2$ with $N(v_2)=\{v_1,v_3,v_4\}$. Because there is no edge between $v_1$ and $v_3$, we add a shortcut $(v_1,v_3)$ with  by $w=w(v_1,v_2)+w(v_2,v_3)=2$ and $c=c(v_1,v_2)+c(v_2,v_3)=3$. Similarly, there is no edge between $v_1$ and $v_4$, so we add a new edge $(v_1,v_4)$ with $w=w(v_1,v_2)+w(v_2,v_4)=2$ and $c=c(v_1,v_2)+c(v_2,v_4)=4$. As for $v_4$ and $v_3$, we first generate a shortcut by $p(v_4,v_2)\oplus p(v_2,v_3)=(2,3)$. Then because there already exists an edge $(3,2)$ from $v_4$ to $v_3$, we compute the new skyline paths between the shortcut and the edge, and get the new skyline paths $p(v_4,v_3)=\{(3,2),(2,3)\}$. After that, we remove $v_2$ from the graph, leaving $v_1$'s degree changed to 4, $v_4$'s degree remaining 5, and $v_3$'s degree remaining 3. We also obtained a tree node $X(v_2,v_3,v_1,v_4)$ with the skyline paths from $v_2$ to $N(v_2)$ and order $r(v_2)=1$. This procedure runs on with the next vertex with the smallest degree. When all the vertices finished contraction, we have an order of $\left<v_2,v_3,v_6,v_7,v_{13},v_{11},v_{10},v_9,v_4,v_1,v_5,v_8,v_{12}\right>$.

%When we contract $v_3$, it is obvious that the neighbours of $v_3$ change to $v_1$, $v_4$, and $v_9$. We insert edge ($v_1, v_4$) and ($v_1, v_9$) in the graph. Then, assign $w(v_1, v_3)+w(v3,v4)$, $c(v_1,v_3)+c(v_3,v_4)$ for ($v_1, v_4$) and $w(v_1, v_3)+w(v_3,v_9)$ ,$c(v_1,v_3)+c(v_3,v_9)$ for ($v_1, v_9$) . We eliminate $v_3$ and build $X(v_3)$ including $v_3$, $v_1$, $v_4$, and $v_9$. We contract the vertices according to the edges degree to build all the nodes for $T_G$ and the skyline paths between any two vertices in each node.   

\subsubsection{Skyline Tree Construction}
\label{subsubsec::Construction_TD_Construction}
The intuition behind the contraction procedure is that the neighbors of $v$ form a set of cuts from $v$ to the rest of the graph and they all have a higher order than $r(v)$. Therefore, all the vertices in $N(v)$ are the ancestors of $v$ in tree. To keep this property for all the vertices, we have to use the one with the smallest order $u = arg min(r(N(v)))$ as the direct parent of $v$ to form the tree. Otherwise, we cannot guarantee all the vertices in a tree node are the ancestors of its representative vertex. For example, $v_3$ has the smallest order in $X(v_2)$, so we add $X_2$ as $X_3$'s child. $r(v_9)$ is the smallest in $X(v_3)$, so we add $X_3$ as $X_9$'s child. In this way, we obtain a tree structure as shown in Figure \ref{fig:Tree Decomposition}.



%In this section, we illustrate an efficient method to construct the CSP-2Hop index. We first introduce how to find all the vertex cuts as nodes for constituting all a tree decomposition $T_G$ . Then we discuss how to efficiently calculate the skyline paths as in label and out label for vertices in each tree node.

%We generate vertex cuts as tree nodes by contracting each vertex with the vertex rank by edges degree. We first create a contracted graph $\overline{G}$ which is initialized as $G$. We begin to contract a vertex $v$ in $\overline{G}$ with the smallest degree and create corresponding node $X(v)$ in $T_G$. The node $x(v)$ must consist of $v$ and all its adjacent vertices in $\overline{G}$. Afterwards, we remove $v$ and all the adjacent edges from $\overline{G}$ but add edges into $\overline{G}$ to ensure all the adjacent vertices of $v$ in $\overline{G}$ can connect to each other. Following the order of edges degree, we contract all the vertices and build all the nodes in $T_G$.  

%As a CSP query may ask for a CSP path from a vertex to its one neighbour, the skyline paths between two adjacent vertices are necessary to preserve as index in $T_G$. Therefore, for every pair of adjacent vertices $(u,w)$ of $v$ in $\overline{G}$, if edge $(u,w)$ does not exist, we insert edge $(u,w)$ with weight $W(u,v)+W(v,w)$ and cost $C(u,v)+C(v,w)$. On the other hand, if edge $(u,w)$ exists in $\overline{G}$, we further check the dominance relations between path $<u,w>$ and another path $<u, v, w>$. If path $<u, v, w>$ dominates path $<u, w>$, we update the weight of edge $(u,w)$ as $W(u,v)+W(v,w)$ and the cost of edge $(u,w)$ as $C(u,v)+C(v,w)$. If path $<u, v, w>$ and path $<u, w>$ can not dominate each other, we add these two paths as two skyline paths between $u$ and $w$. In consequence, we eliminate vertex $v$ from $\overline{G}$, and generate $X(v)$ in $T_G$. Moreover, we rank each vertex by the order of vertices eliminated from $\overline{G}$. The earlier the vertex eliminate, the lower rank it has. We denote the rank as $\pi$. 



%\begin{figure}[ht]
%    \centering
%    \includegraphics[scale=0.35]{Tree1.png}
%    \caption{An example of tree decomposition}
%    \label{fig:Tree1.png}
%\end{figure}

%After finishing all the contraction, suppose $G$ has $n$ vertices, $n$ nodes can be created in $T_G$. For each of node, we can find the corresponding vertex in $G$. For any non-root node of size equal to one, its corresponding vertex is unreachable, as we cannot find the its neighbours in the node. Thus, for $T_G$, we only consider the nodes of size greater than one. The method to construct the nodes is in the following: First, we select a non-root node $X(v)$. Next, we find a vertex $u$ in $X(v)$, which has the lowest rank in $\pi$ except $v$. We set node $X(u)$ as the parent of $X(v)$ in $T_G$. For instance, Figure \ref{fig:Tree Decomposition} shows the final tree decomposition result of \ref{fig:ExampleGraph}. In node $X(v_4)$, except $v_4$, the vertex with the lowest rank in $\pi$ is $v_1$, we thus set $X(v_1)$ as the parents of $X(v_4)$. 

\subsection{Skyline Label Assignment}
\label{subsec::Construction_Label}
%To $T_G$, the straightforward method to calculate skyline paths is Skyline Dijkstra. We can use the algorithm to obtain skyline paths for any pair of vertices in $T_G$ by online searching. However, it will be very time-consuming, as we need to execute the algorithm for each pair of vertices. In this section, we introduce a method to calaculate CSP-2Hop labels with the tree decomposition example in \ref{fig:Tree Decomposition}.

It should be noted the obtained tree preserves all the skyline path information of the original graph because all every edge's information are preserved in the shortcuts. In fact, we can view it as a \textit{superset} of the \textit{CSP-CH} result. Therefore, we can assign the labels with skyline search on this tree directly. However, it would be very time-consuming as the \textit{Sky-Dijk} is much slower than \textit{Dijkstra}'s. To this end, we use the top-down label cascading method that takes advantages the existing labels with query answering to assign labels to the new nodes.

Specifically, a label $L(u)$ stores all the skyline paths from $u$ to its ancestors. Therefore, we start from the root of the tree to fill all the labels. For root itself, it has no ancestor so we just skip it. Next for its child $u$, because the root is the only vertex in $X(u)$ other than $u$, we add the root to $u$'s label. Then for any tree node $X(v)$, it is guaranteed that all its ancestors have obtained their labels. Then for any of its ancestor $a_i$, we compute its skyline paths by taking the skyline paths from  $\{p(v,u)\oplus p(u,a_i), \forall u\in X(v)$\} with the \textit{multiple skyline path concatenation} described in Section \ref{subsec:Skyline_Multiple}. 

For example in Figure \ref{fig:Tree Decomposition}, suppose we have already obtained the labels of $X_1, X_5, X_8$, and $X_{12}$, and we are computing the labels of $X(v_4)$, which has an ancestor set of $\{v_{12}, v_8, v_5, v_1\}$. We take the computation of $L(v_4)[v_{12}]$ as example. $X_4$ has three vertices $\{v_1,v_5,v_8\}$ apart from $v_4$, so we compute the skyline paths via these tree hops. To show the process clearly, we do not apply the pruning first.
\begin{equation*}
    \begin{aligned}
        P_c(h_1)&=p(v_4,v_1)\oplus p(v_1,v_{12})\\
        &=\{(2,4),(4,3)\}\oplus\{(4,7),(6,2)\}\\
        &=\{(6,11),(8,6),(8,10),(10,5)\}\\  
        P_s(h_1)&=\{(6,11),(8,6),(10,5)\}
    \end{aligned}
\end{equation*}
\begin{equation*}
    \begin{aligned}
        P_c(h_5)&=p(v_4,v_5)\oplus p(v_5,v_{12})\\
        &=\{(1,2)\}\oplus \{(3,5),(4,4),(5,3)\}\\
        &=\{(4,7),(5,6),(6,5)\}\\
        P_s(h_5)&=\{(4,7),(5,6),(6,5)\}
    \end{aligned}
\end{equation*}
\begin{equation*}
    \begin{aligned}
        P_c(h_8)&=p(v_4,v_8)\oplus p(v_8,v_{12})\\
        &=\{(1,2)\}\oplus\{(1,1)\}=\{(2,3)\}\\
        P_s(h_8)&=\{(2,3)\}
    \end{aligned}
\end{equation*}

Because $(2,3)$ dominates all the others, we put $(2,3)$ into the label of $L(v_4)[v_{12}]$. If we use the \textit{query rectangle} pruning, we first compute three corresponding rectangles: 
\begin{itemize}
    \item $h_1:(6,11)\times (10,5)$
    \item $h_5:(4,7)\times (6,5)$
    \item $h_8:(2,3)$
\end{itemize}
Because $(2,3)$ dominates the other two rectangles, we prune $h_1$ and $h_5$ and return $(2,3)$ directly as the skyline path.

The correctness of the label assignment procedure can be easily proved by induction. As the label values are essentially the query results using the existing labels of the ancestors, the results are correct as long as the ancestors' labels are correct. The labels are populated in the cascading way, and thus the correctness is naturally guaranteed. Therefore, the resulting label set is a \textit{CSP-2Hop}.
 
%As each node can be regarded as a vertex cut that separate corresponding vertices of its sub-trees nodes to independent parts. For instance, in Figure \ref{fig:Tree Decomposition}, if we remove all the vertices in node $X(v_1)$ from the example graph, we can not reach $v_6$ and $v_7$ from other remaining vertices. Moreover, for a node $X(v_i)$, we can notice that all the vertices in $x(v_i)$ except $v_i$ will be the ancestors of $v_i$. Thus, if we can calculate all the skyline paths from $v_i$ to each ancestor of $v_i$, given a CSP query $(s, t, C)$ and the LCA of $s$ and $t$, we can use our query processing by connecting skyline paths from $t$ to $v$ in the LCA $s$ skyline paths from $v$ to $t$.

%Hence, for arbitrary node $X(v_i)$ in $T_G$, we first pre-compute all the skyline paths from $v_i$ to other vertices in $X(v_i)$ and record it as labels of $v_i$ in the lookup table. In Figure \ref{fig:Tree Decomposition}, to $X(v_3)$, we can obtain the $P(v_3, v_9){(1, 4), (6,3)}$, $P(v_3, v_1){(2, 3)}$, and $P(v_3, v_4){((3,2),(2,3))}$. Then, we store them in the table of CSP-2Hop labels which shown in \ref{talbe:CSP-2Hop}. After calculating all the skylines in each node, we can use these information to obtain the skylines from $v_i$ to each ancestor of it.

%For each node $X(v_i)$, We build an ancestor set $X(v_i)_{anc}$. The vertices in $X(v_i)_{anc}$ must include all the vertices in $X(v_i)$ and other vertices which has higher rank than $v_i$. To calculate the skyline paths from $v_i$ to each vertices in $X(v_i)_{anc}$, suppose $X(v_i)$ has vertices {$v_i, v_a, v_b$}, and $X(v_i)_{anc}$ is {$v_i, v_a, v_b, v_e, v_f$}, as we have already know the skyline paths from $v_i$ to either $v_a$ and $v_b$ in the previous step, we only need to calculate the skyline paths from $v_i$ to $v_e$ and $v_f$. 

%\begin{figure}[ht]
%    \centering
%    \includegraphics[scale=0.25]{Tree2.png}
%    \caption{Labels of tree decomposition}
%    \label{fig:Tree2.png}
%\end{figure}

%\begin{figure}[ht]
%    \centering
%    \includegraphics[scale=0.25]{Lookup.png}
%    \caption{2 hop labeling lookup table for CSP}
%    \label{fig:Lookup.png}
%\end{figure}



==> Extension.tex <==
\section{Extensions}
\label{sec:Extensions}
%It is worth noting that our proposed index framework and the skyline path concatenation algorithm can be easily extended to other \textit{CSP} problems or solutions.

\subsubsection*{Multi-Criteria CSP (MCSP)}
In the multi-criteria network, each edge has a weight $w(e)$ and a set of costs $\{c_1(e),\dots,c_k(e)\}$. The \textit{MCSP} \cite{korkmaz2001multi} asks for the shortest path between an OD that satisfies all the given constraints $\{C_1,\dots,C_k\}$ over the corresponding criterion. To support \textit{MCSP}, we build the index for the multi-criteria skyline path \cite{kriegel2010route,gong2019skyline}, which can be easily extended from the two dimensional skyline. The concatenation follows the same procedure, while the rectangle pruning and the constraint pruning become hyper-cube pruning. 

\subsubsection*{Other Constraint Conditions}
The criteria can be roughly classified into \textit{additive} that takes the sum along a path like travel time and toll charge, and \textit{non-additive} \cite{wang1995bandwidth} that is determined by the bottleneck like maximum height/weight/width/gradient or road type. In this work, we use the \textit{maximum additive constraint} as the example, and we can easily convert it to the \textit{minimum additive constraint} by subtracting all the path costs from a value larger than the maximum cost. As for the \textit{non-additive constraints}, we replace the path cost by the min/max edge cost along it, and all the remaining skyline path concatenation procedures are the same.

\subsubsection*{Extension to CSP-CH}
Our skyline path concatenation method can also be extended to \textit{CSP-CH} to allow it store all the complete skyline shortcuts rather than a subset of it. In fact, the procedure described in Section \ref{subsubsec::Construction_TD_Contraction} creates a superset of the complete skyline shortcuts and can be used to answer \textit{CSP} query in the \textit{CH} way directly, and it is extremely fast to construct.

==> MultiSkyline.tex <==
\section{Multi-Dimensional Constrained Shortest Path}
%Reasons why we need to extend F2Hop
%Since the complexity of road networks and user demands on different constraints, a \textit{CSP} query with only one criterion will be in limited range of applications. In this section, we extend our hop labeling method to solve \textit{CSP} queries on the road networks with multiple criteria. 

%Based on the above findings, in the remaining subsections, we study the challenges of extending \textit{F2Hop} to multiple dimensions. Then, we discuss the Multi-dimensional skyline \textit{(Multi-skyline)} path concatenation with pruning techniques.
\subsection{Extension of F2Hop to Multiple Dimensions}
%#########################################
%definition here
%\begin{definition}[MCSP Query]
%\label{def:Dominance}
%Given a $n$-dimensional graph $\overline{G}(V,\overline{E})$, where $n>2$. Each edge $e \in \overline{E}$ contains a weight $w$ and a series of cost $c_i$, where $i \in [1,n-1]$. Given a $MCSP$ query $\overline{q}(s,t,\overline{C})$. $\overline{C}={C_1,...,C_{n-1}}$ is a set of maximum cost bounds. $\forall C_i\in \mathbb{R}^+$, $\overline{q}(s,t,\overline{C})$ returns a path $p$ with the minimum $w(p)$ while guaranteeing that each $c_i(p) \leq C_i$. 
%\end{definition}
%
%\begin{definition}[Multi-dimensional Path Dominance]
%	\label{def:Multi-Dominance}
%	Given two paths $p_1$ and $p_2$ with the same OD, $p_1$ dominates $p_2$ iff $w(p_1) \leq w(p_2)$ and $c_i(p_1) \leq c_i(p_2),\forall i\in[1,n-1]$, and at least one of them is the strictly smaller relation.
%\end{definition}
%
%\begin{definition}[Multi-Skyline Path]
%	\label{def:Multi-SkylinePath}
%	Given any two paths $p_1$ and $p_2$ with the same OD, they are skyline paths if they cannot dominate each other. 
%\end{definition}
%#########################################

%Challenges of extending F2Hop
As the road network structure dictates the hierarchical structure we built, with the increasing of criteria in a road network, the structure of its tree decomposition will be changeless. However, the skyline path validation will become complex....

Also, the number of skyline paths in each label will increase dramatically, especially, in large scale networks.....


%analysing complex of multi-path domination test
%\begin{theorem}
%	\label{the:2-n skyline}
%We treat two path $p_1$ and $p_2$ are the same, if $w(p_1)=w(p_2)$ and $c_i(p_1)=c_i(p_2),\forall i\in[1,n-1]$. Thereby, if a path $p$ is a skyline path in a two dimensional space, it must be a skyline path in n dimensions. 
%\end{theorem}
%\begin{proof}

%\end{proof}
%In terms of \ref{the:2-n skyline}, we can identify a Multi-skyline path, if it can not be dominated in a two-dimensional space. However,  

%analysing number of skyline paths



\subsection{Multi-Dimensional Constraint Skyline Path Concatenation}

Theorem \ref{theorem:GreedySkyline} efficiently reduces the complexity of skyline path validation in 2D road networks. This is because the cost of 2D skyline paths is natural ranking if we sort them with weight-increasing order. In algorithm \ref{Algorithm:GreedyConcatenation}, when a new path $p_i^j$ is concatenated, its weight must be not less than all the skyline paths in $P_s$. Thus, we only need to compare the cost of $p_i^j$ with the cost of the ranked last path in $P_s$, which has the minimum cost. However, this skyline validation method will be not feasible when each path has multiple costs, as we can not guarantee the ordering of costs for a weight-sorting Multi-skyline path set. For example, in Table \ref{table:EG_skylines} has five skyline paths within 4-dimensions. Each cost is out-of-order, even though we sort them by weigh-increasing order. To reduce the comparison number of skyline validation in paths with multiple costs, we provide the following theorem:


\begin{theorem}
\label{theorem:MultiGreedySkyline}
In $n$-dimensional graph, suppose the concatenated paths are coming in the weight-increasing order. We have $k$ skyline paths and a new path $p_{k+1}$ comes with weight larger than $w_k$. $\forall c_i \in \overline{C}$, $i\leq n$, we rank $k+1$ paths in cost-increasing order and obtain the rank of $p_{k+1}$, which is denoted as $r_i(k+1)$. $\exists o \in [1,n)$ such that $r_o(k+1)$ is minimum compared with arbitrary $r_i(k+1)$. The corresponding criterion $c_o$ is named as distinct criterion. Suppose $m$ concatenated skyline paths, $m \leq k$, have higher or equal ranking than $r_o(k+1)$ on $c_o$. If all the $m$ paths cannot dominate $p_{k+1}$, then $p_{k+1}$ must be a skyline path. 
\end{theorem} 

\begin{proof}
We divide the $k$ skyline paths into two set $S_1$ and $S_2$. $S_1$ contains the $m$ skyline paths that have higher or equal ranking than $p_{k+1}$ on dimension $c_o$. $S_2$ contains the remaining skyline paths.  Compared with all the paths in $S_2$, $p_{k+1}$ has largest value on dimension $c_o$ and highest value on dimension $w$. Thereby, $p_{k+1}$ is a skyline path in set $S_2$. As $p_{k+1}$ has larger weight than the $k$ skyline paths, $p_{k+1}$ can not dominated each path in $S_1$. According to definition \ref{def:Multi-SkylinePath}, if no one path in $S_1$ can dominate $p_{k+1}$, it must be a skyline paths in $S_1$. Due to $p_{k+1}$ is a skyline path in both $S_1$ and $S_2$, it is a skyline path in the current concatenated path set. Also, we have proved that $p_{k+1}$ cannot be dominated by latter coming paths in Theorem \ref{theorem:GreedySkyline}. $p_{k+1}$ thus must be a final skyline path.
\end{proof}

For example in Table \ref{table:EG_skylines}, we have a set of skyline paths ${p_1, p_2, p_3, p_4, p_5}$. On each dimension, we rank the paths with increasing order, which is shown in Figure \ref{fig:MultiSkylineValidation}. Suppose we have the next concatenated path $p_6={8, 5, 8, 9}$. As $p_6$ has greater weight than the five paths, it must be ranked last on dimension $w$. Then, we find the ranks of $p_6$ on other dimensions, which are highlighted by red color. The distinct criterion is $c_2$. We need to identify whether $p_6$ can be dominated by $p_3$ or $p_5$. As $p_6$ cannot be dominated, $p_6$ is a skyline path.

However, in Theorem \ref{theorem:MultiGreedySkyline}, if the next concatenated path $p_{k+1}$ has the same weight with $p_k$, we need to do skyline validation between $p_{k+1}$ and each path that has the same weight with it. If $p_{k+1}$ is dominated, we concatenate next path. If $p_{k+1}$ can dominate any paths having the same weight with it, we remove the dominated paths from the concatenated set. Afterwards, we use Theorem \ref{theorem:MultiGreedySkyline} to further do the skyline validation for $p_{k+1}$. For example, suppose we change $p_6$ to ${6,5,8,9}$. It has the same weight with $p_5$. We compare $p_5$ and $p_6$, as they can not dominate each other, we further check the highest rank of $p_6$ as the same as the previous discussion. 

The efficiency of the extending algorithm is depended on the number of the paths having higher or equal ranking than the new coming path $p_{k+1}$ on distinct criterion. If $p_{k+1}$ ranks too low on distinct criterion, we may compare a large amount of skyline paths in real cases, which is still time consuming. Thus, we provide a pruning technique for the algorithm. The theorem is shown as follows.

\begin{theorem}
\label{the: MultiGreedyPruning}
In $n$-dimensional graph, suppose the concatenated paths are coming in the weight-increasing order. We have $k$ skyline paths and a new path $p_{k+1}$ comes with weight larger than $w_k$. We rank $k+1$ paths as the same as Theorem \ref{theorem:MultiGreedySkyline}. Compute the number of paths that has lower ranking than $p_{k+1}$ on at least one criterion. If the number less than $k$, $p_{k+1}$ is not a skyline path.
\end{theorem}

\begin{proof}
 We proof it by contraction. Suppose $p_{k+1}$ is a skyline path and there are $k-1$ skyline paths having lower ranking than $p_{k+1}$ on at least one criterion. As $p_{k+1}$ has the larger weight than these $k$ paths. We only need to consider the rankings on the criteria of costs. Except $p_{k+1}$, $k$ paths are considered in the rankings. Thereby, it must has at least one skyline path $p_i$, $\forall i \leq k$, having higher or equal ranking than $p_{k+1}$ on all the criteria of costs. According to definition \ref{def:Multi-Dominance}, $p_i$ can dominate $p_{k+1}$. Since the assumption is false, Theorem \ref{the: MultiGreedyPruning} is true.
\end{proof}



\begin{table}[]
\centering
\caption{An example of skyline paths}
\label{table:EG_skylines}
\scriptsize
%\scalebox{1.1}{
\begin{tabular}{|l|l|l|l|l|}
\hline
$P_c$ & $w$ & $c_1$ & $c_2$ & $c_3$ \\ \hline
$p_1$ & 2   & 4     & 10    & 2     \\ \hline
$p_2$ & 2   & 4     & 9     & 3     \\ \hline
$p_3$ & 3   & 7     & 7     & 10    \\ \hline
$p_4$ & 5   & 3     & 9     & 3     \\ \hline
$p_5$ & 6   & 6     & 8     & 4     \\ \hline
\end{tabular}
%}
\end{table}

\begin{figure}[ht]
    \centering
    \includegraphics[scale=0.25]{MultiGreedy.jpg}
    \caption{Next Skyline Path Validation in Multi-dimensions}
    \label{fig:MultiSkylineValidation}
\end{figure}
%rectangle 
%How to concatenate skylines in multi-dimensions. 
%Why it is efficient.
%\subsection{Pruning on Multi-Dimensional Skyline Path Concatenation}
%How to extend rectangle-base pruning
%running example


==> Preliminary.tex <==
\section{Preliminary}
\label{sec:Preliminary}

\subsection{Problem Definition}
\label{subsec:Preliminary_PD}
%As discussed above, we focus our discussions on directed weighted large-scale road network. 
A road network is a graph $G(V, E)$, where $V$ is a set of vertices representing intersections and $E\subseteq V\times V$ is a set of edges representing road segments. Each edge $e \in E$ has two criteria: weight $w(e)$ and cost $c(e)$.  A path $p$ from the source $s \in V$ to the target $t \in V$ is a sequence of consecutive vertices $p$=$\left<s=v_0,v_1,\dots,v_k=t\right>$=$\mycolor{\left<e_0,e_1,\dots,e_{k-1}\right>}$, where \mycolor{$e_i$=}$(v_i,v_{i+1})\in E, \forall i\in[0,k-1]$. Each path $p$ has a weight $w(p)$=$\sum_{e \in p}w(e)$ and a cost $c(p)$=$\sum_{e \in p}c(e)$. We assume the graph unweighted while it is easy to extend our techniques to the directed ones. Then we define the \textit{CSP	} query below:

\begin{definition}[CSP Query]
\label{def:CSP}
Given a graph $G$, a source $s$, a destination $t$, and a maximum cost bound $C\in \mathbb{R}^+$, a \textit{CSP} query $q(s,t,C)$ returns a path with the minimum $w(p)$ while guaranteeing that $c(p) \leq C$. 
\end{definition}

As analyzed in Section \ref{sec:Introduction}, it is quite slow to answer a \textit{CSP} query by online search. Therefore, in this paper, we resort to index-based method and study the following problem: 
\begin{definition}[Index-based CSP Query Processing]
\label{def:PD}
%Given a static undirected weighted graph $G(V, E)$, construct a hop-based index $L$ that given any \textit{CSP} query $q(s,t,c)$, it could answer $q$ efficiently only with $L$.
Given a graph $G$, we aim to construct a hop-based index $L$ that can efficiently answer any \textit{CSP} query $q(s,t,C)$ only with $L$, \mycolor{which stored in a lookup table and can avoid the online searching in road networks.}
\end{definition} 

Unlike the index for the shortest path queries which only needs to store the shortest distance from one vertex to another, the \textit{CSP} index needs to cover all the possible constraints $C$. In addition, we observe that the \textit{CSP} paths are essentially a subset of the \textit{Skyline} paths, which is introduced as follows.
% Therefore, we first introduce the skyline path as follows.

%There are three essential concepts in solving CSP, which are dominance relationship, skyline, and 2 hop labeling. 

\subsection{Skyline Path}
\label{subsec:Preliminary_Skyline}
Like the \textit{dominance} relation of the skyline query in the 2D space \cite{papadias2003optimal}, we first define the \textit{dominance} relation between any two paths with the same source and destination:
\begin{definition}[Path Dominance]
\label{def:dominance}
Given two paths $p_1$ and $p_2$ with the same $s$ and $t$, $p_1$ dominates $p_2$ iff $w(p_1) < w(p_2)$ and $c(p_1) \leq c(p_2)$, or $w(p_1) \leq w(p_2)$ and $c(p_1) < c(p_2)$. 
\end{definition}

\begin{figure}[ht]
    \centering
    \includegraphics[scale=0.22]{example_road_network.pdf}
    \caption{An example of Skyline Path. Edge labels are $(w(e), c(e))$.}
    \label{fig:ExampleGraph}
\end{figure}

%For example in Figure \ref{fig:ExampleGraph}, $p_1$=$\left<v_5, v_4, v_9\right>$ has $w(p_1)=4$ and $c(p_1)=3$, while $p_2$=$\left<v_5, v_8, v_9\right>$ has $w(p_2)=4$ and $c(p_2)=5$. Since $w(p_1)=w(p_2)$ while $c(p_1)<c(p_2)$, $p_1$ dominates $p_2$.

\begin{definition}[Skyline Path]
Given any two paths $p_1$ and $p_2$ with the same $s$ and $t$, $p_1$ and $p_2$ are skyline paths if they cannot dominate each other. %namely they satisfy either of the following two conditions: $(i)$ $w(p_1) \leq w(p_2)$ and $c(p_1) \geq c(p_2)$; or $(ii)$ $w(p_1) \geq w(p_2)$ and $c(p_1) \leq c(p_2)$. 
\end{definition}

In this paper, \mycolor{we use $P(s,t)$ to denote the set of skyline paths from $s$ to $t$. we denote a path $p$ as a skyline path $\overline{p}$ if it is in a skyline path set}. Consider the example in Figure \ref{fig:ExampleGraph}. We enumerate four paths from $v_5$ to $v_9$:
\begin{enumerate}
    \item $p_1 = \left<v_5, v_4, v_9\right>$, $w(p_1)=4$, $c(p_1)=3$
    \item $p_2 = \left<v_5, v_8, v_9\right>$, $w(p_2)=4$, $c(p_2)=5$
    \item $p_3 = \left<v_5, v_4, v_8, v_9\right>$, $w(p_3)=3$, $c(p_3)=6$
    \item $p_4 = \left<v_5, v_8, v_4, v_9\right>$, $w(p_3)=7$, $c(p_3)=6$
\end{enumerate}
According to the definition, we can identify that $p_2$ is dominated by $p_1$, and $p_4$ is dominated by the other three paths. Hence, $p_2$ and $p_4$ are not skyline paths. Meanwhile, as $p_1$ and $p_3$ cannot dominate each other, we obtain two skyline paths from $v_5$ to $v_9$: $P(v_5,v_9)=\mycolor{\{\overline{p}_1,\overline{p}_3\}}$. Next we prove that skyline paths are essential for building any \textit{CSP} index:

\begin{theorem}
\label{the:Skyline}
The skyline paths between any two vertices are complete and minimal for all the possible \textit{CSP} queries.
\end{theorem}
\begin{proof}
We first prove the completeness. Suppose the skyline paths from $s$ to $t$ are \mycolor{$\{\overline{p}_1$, $\dots$, $\overline{p}_k\}$} and they are sorted in the cost-increasing order. Therefore, the cost space is divided into $k+1$ intervals: \mycolor{$[0,c(\overline{p}_1)),[c(\overline{p}_1),c(\overline{p}_2)),\dots, [c(\overline{p}_k),\infty)$}. Then $\forall C\in \mathbb{R}^+$, we can find an $i$ such that $\mycolor{c(\overline{p}_i)}\leq C$ and $\mycolor{c(\overline{p}_{i+1})}> C$. Then it is guaranteed that $\mycolor{\overline{p}_i}$ is a \textit{CSP} result because all the paths with costs smaller than $\mycolor{c(\overline{p}_i)}$ have larger weights than $\mycolor{w(\overline{p}_i)}$, and all the paths with weights smaller than $\mycolor{w(\overline{p}_i)}$ have larger costs than the constraint $C$. When $C<\mycolor{c(\overline{p}_1)}$, no path between $s$ and $t$ satisfies the constraint; when $C>\mycolor{c(\overline{p}_k)}$, $\mycolor{\overline{p}_k}$ is the \textit{CSP} result.

Next we prove this skyline path set is minimal. Suppose we remove any skyline path $\overline{p}_i$ from the skyline result set. Then for \textit{CSP} queries whose constraint is within the range $[c(\overline{p}_i),c(\overline{p}_{i+1})]$, its result would be $\overline{p}_{i-1}$. However, the correct result should be $\overline{p}_i$ as analyzed above. Hence, no skyline path can be removed and the set is minimal.
\end{proof}

In summary, building an index for \textit{CSP} query is equivalent to building the index for skyline path query.
%Hence, building an index for skyline path query is equivalent to the \textit{CSP} query.

\subsection{2-Hop Labeling}
\label{subsec:Preliminary_2Hop}
\textit{2-hop labeling} is an index method that does not involve any search during query answering. It answers the shortest distance query by table lookup and addition. Specifically, $\forall u \in V$, we assign a label set $L(u)={\{v,w(v,u)\}}$ to store the minimum weights between a set of \textit{hop vertices} $v$ to $u$. To answer a query $q(s,t)$, we first determine the intermediate hop set $H=L(s) \cap L(t)$. Then we can find the minimum weight via the hop set: $min_{h \in H}{\{w(s,h)+w(h,t)\}}$. In this work, we extend the 2-hop labeling to support \textit{CSP} path because it can avoid any search during query processing.



==> SkylineQuery.tex <==
\section{Extension to Skyline Query}



%\subsection{Index Construction Using Skyline Preserved Graph}

%\subsection{Label with Distance and Cost Skyline}
